Learning a Static Bug Finder from Data

We present an alternative approach to creating static bug finders. Instead of relying on human expertise, we utilize deep neural networks to train static analyzers directly from data. In particular, we frame the problem of bug finding as a classification task and train a classifier to differentiate the buggy from non-buggy programs using Graph Neural Network (GNN). Crucially, we propose a novel interval-based propagation mechanism that leads to a significantly more efficient, accurate and scalable generalization of GNN. We have realized our approach into a framework, NeurSA, and extensively evaluated it. In a cross-project prediction task, three neural bug detectors we instantiate from NeurSA are effective in catching null pointer dereference, array index out of bound and class cast bugs in unseen code. We compare NeurSA against several static analyzers (e.g. Facebook Infer and Pinpoint) on a set of null pointer dereference bugs. Results show that NeurSA is more precise in catching the real bugs and suppressing the spurious warnings. We also apply NeurSA to several popular Java projects on GitHub and discover 50 new bugs, among which 9 have been fixed, and 3 have been confirmed.

==> GGNN_paper-(submission)/Sections/Abstract.tex <==
% !TeX root = ../ggnn.tex


\begin{abstract}\label{sec:Abstract}

% Static analysis is an effective technique to catch bugs early when they are cheap to fix. Recent advances in program reasoning theory have led to increasing adoption of static analyzers in software engineering practice. Despite the significant progress, the room for improvement remains. In this paper, 

We present an alternative approach to creating static bug finders. 
Instead of relying on human expertise, we utilize deep neural networks
to train static analyzers directly from data. In particular, we frame the problem of bug finding as a classification task and train a classifier to differentiate the buggy from non-buggy programs using Graph Neural Network (GNN). Crucially, we propose a novel interval-based propagation mechanism that leads to a significantly more efficient, accurate and scalable generalization of GNN. 

We have realized our approach into a framework, \tool, and extensively evaluated it. In a cross-project prediction task, three neural bug detectors we instantiate from \tool are effective in catching null pointer dereference, array index out of bound and class cast bugs in unseen code. 
We compare \tool against several static analyzers (\eg Facebook Infer and Pinpoint) on a set of null pointer dereference bugs. Results show that \tool is more precise in catching the real bugs and suppressing the spurious warnings. We also apply \tool to several popular Java projects on GitHub and discover 50 new bugs, among which 9 have been fixed, and 3 have been confirmed.

% We are in active discussion with Visa Inc for possible adoption of \tool in their software development cycle. Due to the effectiveness and generality, we expect \tool to be helpful in improving the quality of their code base.  
\end{abstract}


==> GGNN_paper-(submission)/Sections/Append.tex <==
\subsection{Irreducible Graph }

Figure \ref{fig:irredGraph} shows examples of graphs that can not be reduced to a single node.

\begin{figure}[htb!]
\centering
  \includegraphics[width=.25\linewidth]{Figures/non-reduce.pdf}
  \caption{Examples of irreducible graph.}
  \label{fig:irredGraph}
\end{figure}


\subsection{Examples of Array Index Out of Bound bugs and Class Cast Exceptions}

Figure \ref{fig:CCEExamples} and \ref{fig:AIOOBExamples} show examples of the array index out of bound and class casting bugs.
Note that even though there are lots of these kinds of bugs, the pattern of them are less than null pointer dereference bugs.


\begin{figure*}
\begin{subfigure}[htb!]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Casting PC to ChildClass raises CCE.
public void manipulate(ParentClass PC) {
    ChildClass CC = (ChildClass) PC;
}
    
public void foo() {
    ParentClass PC = new ParentClass();
    manipulate(PC);
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:CCEa} A typical pattern of CCE.}
\end{subfigure}

\begin{subfigure}[b]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Extracted from bugs-dot-jar_LOG4J2-104
static {
    ...
    // url.returnLines() returns objects not in XML format
    props.loadFromXML(url.returnLines());
    ...
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:CCEb} CCE caused by different class.}
\end{subfigure}


\begin{subfigure}[b]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Extracted from bugs-dot-jar_CAMEL-9672
public Object getManagedObjectForProcessor(CamelContext context, 
                                        Processor processor,
                                        ProcessorDefinition<?> definition, 
                                        Route route) {     
    ...
    } else if (target instanceof FilterProcessor) {
        // FilterDefinition is so precise that it results in CCE
        // The repair patch changes it to its parent class ExpressionNode.
        answer = new ManagedFilter(context, (FilterProcessor) target,
        (FilterDefinition) definition);
    ...
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:CCEc} CCE caused by class inherent.}
\end{subfigure}


\begin{subfigure}[b]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Extracted from eclipse.jdt.ui-096ab8f
private ITypeBinding getDestinationBinding() throws JavaModelException {
    ...
    // None of the two class cast operations are safe.
    return (ITypeBinding)((SimpleName)node).resolveBinding();
    // Fixed codes
    if (!(node instanceof SimpleName)) return null;
    IBinding binding= ((SimpleName)node).resolveBinding();
    if (!(binding instanceof ITypeBinding)) return null;
    return (ITypeBinding)binding;
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:CCEd} CCE caused by multiple class cast operations.}
\end{subfigure}
\caption{Illustrative examples of the CCE bugs.}
\label{fig:CCEExamples}
\end{figure*}


\begin{figure*}[t]
%\centering
\begin{subfigure}[b]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Extracted from eclipse.platform.ui-fa4aec8
public void restoreState(IDialogSettings dialogSettings) {
    ...
    priorities[i] = Integer.parseInt(priority);
    ...
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:array1} A typical pattern of AIOE.}
\end{subfigure}


\begin{subfigure}[b]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Extracted from bugs-dot-jar_LOG4J2-811
public void logMessage(final String fqcn, final Level level, 
    final Marker marker, final Messagemsg,
    final Throwable throwable) {
    ...
    // the length of params can be zero.
    if (... && params != null && params[params.length - 1] instanceof Throwable) {
        t = (Throwable) params[params.length - 1];
    } 
    ...
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:array2} AIOE caused by zero length array.}
\end{subfigure}


\begin{subfigure}[b]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Extracted from tomcat-3f4a241
public void addFilterMapBefore(FilterMap filterMap) {
    ...
    // The 4-th argument should be filterMaps.length - (filterMapInsertPoint + 1)
    System.arraycopy(filterMaps, filterMapInsertPoint, results,
    filterMaps.length - filterMapInsertPoint + 1,
    ...
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:array3} AIOE caused by miscalculate starting position in destination array.}
\end{subfigure}

\caption{Illustrative examples of AIOE.}
\label{fig:AIOOBExamples}
\end{figure*}

\clearpage

\subsection{Other Pertinent Information of Evaluated Projects}

Table \ref{tab:numOfBugs} shows the number of bugs and buggy methods in our evaluated projects. The number outside (inside) of the parenthesis is the number of bugs (buggy methods). Note that developer may fix multiple methods for a single bug so the number of buggy method and bugs may differ.

\begin{table*}[htbp!]
\centering
\small
\caption{Number of bugs of evaluated projects}
\begin{tabular}{c|ccc}
\hline
  \multirow{2}{*}{\tabincell{c}{Projects}} &  \multicolumn{3}{c}{Number of bugs (buggy methods)} \\
\cline{2-4}
& \tabincell{c}{NPE} & \tabincell{c}{AIOE} & \tabincell{c}{CCE} \\\hline
Lang &  5 (7) & 3 (5) & 1 (2)  \\\hline
Closure & 2 (18) & 0 (0) & 0 (0)  \\\hline
Chart & 4 (17) & 1 (7) & 0 (0)  \\\hline
Mockito & 7 (14) & 2 (5)  & 5 (23)  \\\hline
Math & 10 (16)  & 8 (17) & 2  (3) \\\hline
Accumulo & 5 (6)  & 0 (0) & 0 (0)  \\\hline
Camel & 8 (17) & 1 (1) & 1 (1)  \\\hline
Flink & 6 (13) & 0 (0) & 0 (0)  \\\hline
Jackrabbit-oak & 7 (23) & 1 (1) & 1 (1)  \\\hline
Log4j2 & 16 (29) & 1 (1) & 1  (2) \\\hline
Maven & 3 (6) & 0 (0) & 0 (0)  \\\hline
Wicket & 6 (7) & 1 (1) & 3 (8)  \\\hline
Birt & 165 (678) & 19 (129) & 39 (154)  \\\hline
JDT UI & 332  (897) & 39 (63) &  47 (156) \\\hline
SWT & 105  (276) & 40 (136) & 7  (26)  \\\hline
Platform UI & 389  (920) & 27 (72) & 60  (194) \\\hline
Aspectj & 72  (151) & 9 (14) &  9  (19) \\\hline
Tomcat & 44  (111) & 6  (18)& 12  (28) \\\hline
\hline
Total & 1186 (3206) & 143 (470) & 188 (617)  \\\hline
\end{tabular}
\label{tab:numOfBugs}
\end{table*}









\ignore{

\begin{table*}[!t]
\centering
\small
\caption{Projects used in the evaluation.}
\begin{tabular}{c|c|c|ccc}
\hline
 \multirow{2}{*}{Dataset} & \multirow{2}{*}{Projects} & \multirow{2}{*}{Description}&  \multicolumn{3}{c}{\#Methods} \\
\cline{4-6}
& & &\tabincell{c}{NPE} & \tabincell{c}{Array} & \tabincell{c}{\tabincell{c}{CCE}} \\\hline
\multirow{13}{*}{Test} &Lang & Java lang library & 486 & 225 & 174  \\\cline{2-6}
&Closure & A JavaScript checker and optimizer. & 46 & 0 & 0  \\\cline{2-6}
&Chart & Java chart library & 504 & 20 & 0  \\\cline{2-6}
&Mockito & Mocking framework for unit tests & 209 & 22 & 94  \\\cline{2-6}
&Math & Mathematics and statistics components & 188 & 284 & 31  \\\cline{2-6} % 121+67, 139+145, 31
&Accumulo & Key/value store & 69 & 0 & 0  \\\cline{2-6}
&Camel & Enterprise integration framework & 653 & 98 & 12  \\\cline{2-6}
&Flink & System for data analytics in clusters & 141 & 0 & 0  \\\cline{2-6}
&Jackrabbit-oak & hierarchical content repository & 289 & 34 & 24  \\\cline{2-6}
&Log4j2 & Logging library for Java & 187 & 9 & 2  \\\cline{2-6}
&Maven & Project management and comprehension tool & 50 & 0 & 0  \\\cline{2-6}
&Wicket & Web application framework & 98 & 42 & 30  \\\hline
\hline
\multicolumn{3}{r|}{Total}& 2920 (173) & 734 (38) & 365 (40)  \\\hline % (num) is the number of buggy methods
\hline
\multirow{6}{*}{Training}&Birt & Data visualizations platform & 1356 & 258 & 308  \\\cline{2-6}
&JDT UI & User interface for the Java IDE & 1794 & 126 & 312 \\\cline{2-6}
&SWT & Eclipse Platform project repository & 552 & 272 & 52  \\\cline{2-6}
&Platform UI & User interface and help components of Eclipse & 1840 & 144 & 388  \\\cline{2-6}
&AspectJ & An aspect-oriented programming extension & 302 & 28 &  38 \\\cline{2-6}
&Tomcat & Web server and servlet container & 222 & 36 & 56  \\\hline
\hline
\multicolumn{3}{r|}{Total}& 6066 (3033) & 864 (432) & 1154(577)  \\\hline
\end{tabular}
\label{tab:methodres}
\end{table*}
}



==> GGNN_paper-(submission)/Sections/Approach.tex <==
% !TeX root = ../ggnn.tex

\section{Framework}\label{sec:AD}
This section presents \tool, a framework for creating various kinds of neural bug detectors. 
% In particular, we address two challenges: how to obtain sufficient training data and how to train a model that can precisely detect the presence of a bug.

\subsection{Overview of \tool}
\label{subsec:over}

\begin{figure}
\centering
  \includegraphics[width=0.95\linewidth]{Figures/Framework.png}
  \caption{\tool's Workflow.}
  \label{fig:framework}
\end{figure}

Figure \ref{fig:framework} depicts the overview of \tool. We split \tool's workflow into four parts and describe each one below.
%It consists of four parts.

\begin{enumerate}[label*=(\arabic*)]
    \item \textbf{Collecting Data:} We extract programs from the codebases of real-world projects. We obtain bug labels by cross-referencing bug reports and the commit history of the same project. 
    
    \item \textbf{Representing Programs Using Graphs:} We construct the control flow graph for each method. To facilitate \tool to pinpoint a bug in a method, %    is constructed to a method-level control flow graph (CFG).
    we break each node denoting a basic block into multiple nodes each of which represents a non-control statement. We also stitch the control flow graphs of caller and callee to aid inter-procedural analysis. 
    
    
    %In order to avoid merging statements with different semantics, each node in the graph is a statement, instead of a basic block. 
    %To the best of our knowledge, real-world methods can be very large. Therefore, to reduce the communication burden, each graph is partitioned into several intervals. The compact representation of method-level CFG is called method-level interval graph. Two kinds of edges are introduced to represent edges in intra-interval and inter-interval nodes. Nodes are represented as a list of syntax tokens.
    
    \item \textbf{Training Neural Bug Detectors:} We train neural bug detectors using graph neural networks. In particular, we propose a novel interval-based propagation mechanism that significantly enhances the capacity of GNN in learning programming patterns. 
    % address the generalization issues of GGNN on large graphs. The idea is to only perform propagation among nodes within the same interval. By moving from a lower order interval graph to a higher order interval graph, we implicitly expand the propagation to include more nodes in a graph, and therefore moving the propagation gradually towards the global level. To recover the embeddings of each node in the first order graph, we split an interval of higher order graph back to a multitude of nodes in the lower order graph until arriving at the original control flow graph. The process will be repeated until the model converges. Our intuition is to divide the propagation into two modes: local and global, between which a transition is realized to find the sweet spot. 
    %when a graph and its representations of nodes $\mathcal{M}$ are available, we perform the training process. The information propagation on interval graphs consists of three steps. First, for nodes inside each interval, we perform the classic information propagation. Then, when intra-interval propagation is finished, we conduct inter-interval propagation. The representation of each interval is computed by summing up the representations of all the nodes inside the interval. Finally, the representation of each node inside an interval is computed by averaging the representation of this interval. The combination of the three steps is an information propagation for the whole graph. We repeat it for $L$ times and take the node representation as final node representation.

    \item \textbf{Bug Detection:} Finally, we detect bugs in unseen code using the model we have trained.

\end{enumerate}

\subsection{Data Generation}
\label{subsec:data}
We use bug databases proposed by the prior works~\cite{just2014defects4j,saha2018bugs,tomassi2019bugswarm,ye2014learning} to generate our dataset. All databases provide a rich set of meta-information on each bug they contain (\eg detailed bug descriptions, links to actual commits of bug fixes, projects bug reports, \etc). We rely on such information to extract buggy methods and identify bug types. For example, given a bug description "\textit{Fixing Bugzilla\#2206...}", we search in the bug reports using the id \textit{\#2206} to retrieve the details of the bug, against which we match pre-defined keywords to determine the type of the bug. Next, we refer to the code commit to find out bug locations, specifically, we consider the lines that are modified by this commit to be buggy and the rest to be clean. We acknowledge the location of a bug and its fix may not be precisely the same thing. However, given the quality and maturity of the codebases we work with, our assumptions are reasonable. After extracting a buggy method, we choose from the same project several syntactically closest correct methods \wrt the tree edit distance between their abstract syntax trees.
 
% \ke{Given bug type information to correlate to intro} We extract methods from real world project corpus. To collect buggy code, we look for commits of bug fixes. For example, if a commit is described to fix a bug, then the lines that are modified will be considered as buggy whereas the rest are considered to be clean. We acknowledge the location of a bug and its fix may not be precisely the same thing. However, given the quality and maturity of the codebases we work with, our assumptions are reasonable. To classify the types of bugs, we cross-reference the bug reports and commit history of the same project. For example, given the format of a commit message "\textit{Fixing Bugzilla\#2206...}", we search in the bug reports using the id \textit{\#2206} to retrieve the details of the bug, against which we match pre-defined keywords to determine its type. To create a balanced dataset, for each buggy method we collect, we choose a syntactically closest correct method \wrt the tree edit distance between their abstract syntax trees.

\subsection{Representing Programs with Graphs}

We represent each method using its control flow graph. Besides, we split a graph node representing a basic block into a number of nodes, each of which represents a single statement. This variation enables the localization of bugs at the level of lines. To further enhance the expressiveness of our graph representation, we take the following measures: (1) we incorporate a new type of edges to represent the data dependency among variables. Specifically, we connect nodes with data dependency edges if the statements they represent exhibit a dependency relationship. Note that data dependency edges do not contribute to partitioning graphs into intervals. They only facilitate the local propagation within each interval. (2) we also add variable types into the mix. Given a variable $var$, we consider not only its actual type $\tau(var)$ but also all the supertypes of $\tau(var)$, denoted by $\tau^*(var) = \bigcup_{i=1}^{i=n} \tau^i(var)$, where $\tau^i(var) = \{\tau | \bigcup_{\omega \in \tau^{i-1}(var)} \omega$ implements $\tau\}$ with a base case $\tau^1(v) = \{\tau| \tau(var)$ implements type $\tau\}$. $\tau^n(var)$ signals the most general type (\eg \texttt{Object} in Java).

Due to the static nature of each non-control statement, we resort to recurrent neural networks---suitable for modeling sequentially data---to learn the initialization for each node in the graph. In particular, we treat a statement as a sequence of tokens. After each token is embedded into a numerical vector (similar to word embeddings~\cite{mikolov2013efficient}), we feed the entire token sequence into the network and extract its final hidden state as the initial node embedding. 

% If a method invokes other methods inside its body, 
We stitch the graphs of all callers (\ie methods invoking the target method) and callees (\ie methods invoked by the target method) to that of each target method to support inter-procedural analysis. In particular, we connect the node of method invocation inside of the caller to that of the entry point inside of the callee. Node labels obtained for each graph will be kept on the merged graph for neural bug detectors to predict. Worth mentioning our graph representation is independent of the type of the bug detector we train. In other words, a graph only presents the semantic representation of a program, it's the responsibility of a bug detector to learn the patterns \wrt the type of bugs it's interested in.

\subsection{Training and Testing Neural Bug Detectors}
Given the method representations we derived, we train a classifier using GNN with IBPM. In particular, different types of bug detectors will be trained and applied separately to catch bugs in the unseen code. Internally, each neural bug detector is trained in two steps. First, we train a feed-forward neural network~\cite{svozil1997introduction} on top of method embeddings computed from GNN (\ie aggregation of the node embeddings) to predict if a method is buggy or not. If it is, we will use the same network to predict the buggy lines. Our rationale is graph as a whole provides stronger signals for models to determine the correctness of a method. Correct methods will be refrained from further predictions, resulted in fewer false warnings to be emitted. On the other hand, if a method is indeed predicted to be buggy, our model will then pick the top $N$ statements according to their probabilities of being buggy. The benefit of this prediction mode is to provide flexibility for developers to tune their analysis toward either producing less false warnings or identifying more bugs. 

% In general, we initialize a node based on the Abstract Syntax Tree (AST) or token sequence of the statement it denotes. To enhance the expressiveness of the programs features, we also incorporate variable type information. Given a variable $var$, we consider not only its actual type $\tau(var)$ but also all the supertypes of $\tau(var)$, denoted by $\tau^*(var)$ \st $\tau^*(var) = \bigcup_{i=1}^{i=n} \tau^i(var)$, where $\tau^i(var) = \{\tau | \bigcup_{\omega \in \tau^{i-1}(var)} \omega$ implements $\tau\}$ with a base case $\tau^1(v) = \{\tau| \tau(var)$ implements type $\tau\}$. Based on the above-mentioned information, we present three choices for node initialization:



%Therefore, we leverage variable type information, 
%current type $\tau(v)$ and supertypes of $\tau(v)$ are encoded into the corresponding vector.
%To achieve this, we map a variable's type $\tau(v)$ to the set of its all supertypes, \ie, $\tau^1(v) = \{\tau: \tau(v)$ implements type $\tau\}, \tau^2(v) = \{\tau: \forall \tau(v_i) \in \tau^1(v), \tau(v_i)$ implements type $\tau\}, ..., \tau^n(v) = \{\tau: \forall \tau(v_i) \in \tau^{(n-1)}(v), \tau(v_i)$ implements type $\tau\}, \tau^*(v) = \bigcup_{i=1}^{i=n} \tau^i(v)$. The iteration finishes when there is no more new type. $\tau^*(v) = \{\tau: \tau(v)$ implements type $\tau\} \cup \{\tau(v)\}$.



% \paragraph{\textbf{Characteristic Vectors}}
% Given a statement denoted by a node in the graph, we first extract its Abstract Syntax Tree (AST). According to the definition of characteristic vectors~\cite{4222572}, we then count the number of occurrences for each type of the AST node (\eg for loop structure, if-else statement, assignment statement) and aggregate them into a vector in any pre-defined order. Finally we use the vector as an initial representation of the node. To keep the number of dimensions manageable, we consider all the variable types to be identical.
%To further enhance the expressiveness of this encoding, we leverage variable type information. 

%\begin{definition}{($q$-Level Atomic Tree Patterns)}
%\label{def:pat}	
%A $q$-level atomic pattern is a 
%complete binary tree of height $q$. Given a 
%label set $L$, including the empty label 
%$\epsilon$, there are at most $\vert L \vert^{2^q-1}$ 
%distinct $q$-level atomic patterns.
%\end{definition}

%\begin{definition}{($q$-Level Characteristic Vector)}	
%\label{def:cv}	
%	Given a tree $T$, its $q$-level 
%	characteristic vector is 
%	$\langle b_{1},  ...., b_{\vert L \vert^{2^q-1}} \rangle$, where $b_{i}$ 
%	is the number of occurrences of the $i$-th $q$-level 
%	atomic pattern in $T$.
%\end{definition}

% \paragraph{\textbf{RNN-Based Encoding}}
% As an alternative, we rely on Recurrent Neural Networks (RNNs) to initialize a node. In particular, we treat a statement as a sequence of tokens. After each token is embedded into a numerical vector (similar to word embeddings~\cite{mikolov2013efficient}), we feed the entire token sequence into a RNN and extract its final hidden state for node initialization. Note that we take some special measures to increase the precision of our encoding. First, whenever a token of a variable type occurs in the sequence, we automatically inject all of its supertypes into the token seqeunce before the actual type. Second, all variable tokens will receive the same embedding before being sent to the RNN as the inputs. In other words, we represent a variable primarily with its type information.

% \paragraph{\textbf{Transformer-Based Encoding}}
% We also utilize Transformer~\cite{vaswani2017attention}, arguably the state-of-the-art deep model in neural machine translation, to initialize a node. Similar to the RNN-based encoding, we use token sequence to represent a statement. However, instead of using RNN to process the sequence, we compute an attention weight for each token \wrt the other tokens in the sequence. In the end we compute the weighted sum of all tokens as the initialization vector. Similar to the RNN-Based encoding, we also take into account the type information to represent a variable. 





%In CFG, each node is a basic block, which is a linear sequence of program instructions having one entry point (the first instruction executed) and one exit point (the last instruction executed). 
%In order to avoid merging statements having different semantics, each node in our graph is a statement, which means that a basic block in CFG is split into several nodes.
%For convenience, we refer this kind of graph as method-level CFG, which is also denoted as $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{M})$.

%Based on the method-level CFG, we perform the partition according to Algorithm \ref{alg:intervals}.
%It splits a graph into intervals such that the complexity of a graph is reduced.
%Recall that $\mathcal{S}^i$ is the i-th order of graph and intervals are denoted as $I^i(h)$.
%Nodes inside an interval are denoted as $v^i_j \in I^i(h)$. 
%When $i$ is 1, then $v^1_j = v_j \in \mathcal{V}$.
% this is useless, but it is more representative for the CFG-based method we used to compare.
%We define two kinds of edges, representing relationship inside an interval and relationship between intervals, separately.

%\subsubsection{Node Representation}

%Each node in our graph is a statement of the corresponding line, we introduce AST-based vector representation for each statement.

%For each node, we use $\mu_v$ to represent the initial node representation.
%$\mu_v$ is represented in form of $\mu_v=\{NI_1, NI_2, ..., NI_j\}$ where $NI_i, i \in \{1,...,j\}$ is the node index when traversing the abstract syntax tree (AST) of the node $v$.
%$j$ depends on the length of the AST, which means that it is a variant number instead of a fixed number.
%Given a predefined dictionary, node index is the the unique identification of a AST node, including terminals (\ie, syntax tokens) and non-terminals (\ie, syntax nodes) in the programming language's grammar.
%Same kind of AST nodes share the same node ID.

%As far as we know, nodes index in a AST is too simple to capture semantics of a method.
%Therefore, we leverage variable type information, 
%current type $\tau(v)$ and supertypes of $\tau(v)$ are encoded into the corresponding vector.
%To achieve this, we map a variable's type $\tau(v)$ to the set of its all supertypes, \ie, $\tau^1(v) = \{\tau: \tau(v)$ implements type $\tau\}, \tau^2(v) = \{\tau: \forall \tau(v_i) \in \tau^1(v), \tau(v_i)$ implements type $\tau\}, ..., \tau^n(v) = \{\tau: \forall \tau(v_i) \in \tau^{(n-1)}(v), \tau(v_i)$ implements type $\tau\}, \tau^*(v) = \bigcup_{i=1}^{i=n} \tau^i(v)$. 
%The iteration finishes when there is no more new type.
%$\tau^*(v) = \{\tau: \tau(v)$ implements type $\tau\} \cup \{\tau(v)\}$.
%We can see that $\tau^*(v)$ is a collection of types. 
%We still leverage a commonly used predefined dictionary to map different types. 
%If a type is not in the dictionary, we additionally define $\tau_{unk}$ for all unknown types.
%To represent them as a vector, we traverse $\tau^*(v)$ from bottom to top (\ie, from $\tau^1(v)$ to $\tau^n(v)$) and append them to the vector in order.
%Finally, we merge type information and the AST based representation, so that each variable is represented by its type information, which is a dynamic way of encoding various variables.

%The assumption behind our representation is that leveraging AST information and type information is enough.
%However, representing tokens as as integer may not be sufficient to capture complex semantics of real world programs.
%To extend the ability of our representation, we additionally design four kinds of node representations.

%\textbf{Naive node representation: } The first design uses a fixed size of vector $\mathit{Vec}$ to represent a statement.
%The size of a vector is the number of predefined tokens.
%For each $TK_i$ in a statement, we increment the occurrence of the token.
%In other words, formula $Vec[dict(TK_i)] += 1$ shows the same mechanism. and $dict(TK_i)$ represents extracting the index of $TK_i$.

%The last three kinds depend on the $\mu_v$, whose size is variant and depends on the complexity of a statement.

%\textbf{LSTM-based representation: } It uses long short-term memory (LSTM) \cite{hochreiter1997long} to learn an embedding vector for each token.


%\textbf{Transformer-based representation: } It imports the encoder component in the transformer \cite{vaswani2017attention}.
%The intuition is that we regard a statement as a mutation of natural languages.
%Similar to natural languages, semantics of a statement depends on the whole context instead of processing them separately. 
%Transformer is a state-of-the-art network that shows a successful applications in language translation.

%\textbf{TransLSTM representation: } it combines the two methods so that we leverage LSTM to learn an embedding vector for each element learned by Transformer.

% \subsection{Training Neural Bug Detectors}
% % \begin{figure}[H]
% % \begin{subfigure}[t]{0.45\textwidth}
% % \centering
% %   \includegraphics[width=0.95\linewidth]{Figures/propagation-forward.pdf}
% %   \caption{Transition from low-order to high-order graph.}
% %   \label{fig:propagation-forward}
% % \end{subfigure}\hfill
% % \begin{subfigure}[t]{0.45\textwidth}
% % \centering
% %   \includegraphics[width=0.95\linewidth]{Figures/propagation-backward.pdf}
% %   \caption{Transition from high-order to low-order graph.}
% %   \label{fig:propagation-backward}
% % \end{subfigure}
% % \caption{Example of interval graph propagation.}
% % \label{fig:propagation}
% % \end{figure}

% Given the method representations we derived, we train a classifier using GNN with IBPM. 
% notice as the size of a graph increases, GGNN drops its accuracy, indicating its inadequacy in addressing the scalability challenge. Fundamentally, the cause of decrease in GGNN's accuracy lies in its propagation model. Specifically when a graph has large diameter, information has to be propagated over long distance, therefore, message exchange between nodes that are far apart in a graph becomes difficult. To overcome the scalability issues, we propose a novel interval-based propagation model that scales the generalization of GGNN to large graphs. Our insight is to use intervals to regulate how information is propagated on a graph. In particular, nodes are only allowed to communicate with their peers within the same interval. By transitioning the propagation on lower-order graphs to higher-order graphs (and \vv), we enable a sufficient message exchange among all nodes in a graph. Below we use the graph in Figure~\ref{fig:interval} to describe in details how the propagation works. 


% Starting with first order graph $\mathcal{S}^1$ (\ie initial control flow graph), since nodes are only allowed to exchange with their peers within the same interval, propagation will only take place in $I^{1}(3)$ (node 3, 4, 5 and 6) and $I^{1}(7)$ (node 7 and 8). The message exchange is conducted the same way as before (\ie Equation~\ref{equ:mes1} and~\ref{equ:mes2}). After repeating the propagation for a few steps, we move the propagation to the second order graph $\mathcal{S}^2$. Since we create two new nodes (\ie node 9 and 10) on $\mathcal{S}^2$ denoting $I^{1}(3)$ and $I^{1}(7)$ on $\mathcal{S}^1$, we sum the embeddings of nodes within $I^{1}(3)$ and $I^{1}(7)$ to be the initial representation for node 9 and 10 on $\mathcal{S}^2$. The following equation defines the initialization for nodes that are created when transitioning to higher-order graphs.

% \begin{equation}
% \mu^{(l)}_{I^{i+1}(h)} = \sum_{\mathclap{v \in I^{i+1}(h)}} \mu^{(l)}_{v}
% \end{equation}

% Similar to the propagation on $\mathcal{S}^1$, propagation on $\mathcal{S}^2$ takes place in $I^{2}(2)$ (node 2, 9 and 10) while node 1 is still isolated. Note that as propagation occurs within $I^{2}(2)$ on $\mathcal{S}^2$, all nodes except node 1 on $\mathcal{S}^1$ are communicating, with node 9 and 10 (on $\mathcal{S}^2$) being the proxy of node 3-6 and node 7 and 8 (on $\mathcal{S}^1$) respectively. This is where our new propagation model is advantageous over the existing one. As the propagation moves towards the global mode, the amount of data traffic is still manageable because many nodes only communicate through their proxies without being present in the graph to overload the propagation. When arriving at $\mathcal{S}^3$, we enable the propagation among all nodes in the graph directly or indirectly. Figure~\ref{fig:propagation-forward} illustrates the process.

% Now to recover the node embeddings on $\mathcal{S}^1$, we move the propagation back from $\mathcal{S}^3$ to $\mathcal{S}^1$ (Figure~\ref{fig:propagation-backward}). The idea is to reemphasize local propagation among nodes within an interval after their exposure to the global view of the graph. To initialize nodes within an interval on a lower order graph that are split from a single node on a higher order graph, we perform the following:
% \begin{equation}
% \forall m \in I^{i+1}(h), I^{i}(m) = \frac{\mu^{(l)}_{I^{i+1}(h)}}{|I^{i+1}(h)|}
% \end{equation}

% The process of transitioning between lower order graph and higher order graph is repeated until the model converges. 

% There are also many alternative designs~\cite{kipf2016semi,hamilton2017inductive,liao2018graph} relying on graph partitioning to scale graph neural networks. Compared with those works, our interval based propagation enjoys several conceptual advantages. First, since partition problems in graph
% theory are typically NP-hard, those works look for heuristic to approximate in practice. Second, given the graph partitions, they need to manually design how to alternate between the two propagation modes (\ie local and global). In contrast, by transitioning from lower order graph to higher order graph (and \vv), our propagation model mixed the two modes naturally and seamlessly. Third, our propagation model makes use of the special constructs in programs, which none of the related works considered. Specifically, intervals can be regarded as a representation of loop constructs, especially those that consist of many nodes, therefore by attending to a loop construct in a propagation model, GGNN can extract deeper and more precise semantic program features that other works can not. 


% %Given a list of interval sets $\{\mathcal{S}^i | i \in \{1,...,n\}\}$ where $n$ is the maximum order graph (\eg, $n$ is 4 in Fig. \ref{fig:interval}).
% %We perform the information propagation for intervals inside $\mathcal{S}^i$ as follows:

% %\begin{equation}
% %\mu^{(l)}_{I^{i+1}(h)} = \sum_{\mathclap{v \in I^{i+1}(h)}} \mu^{(l)}_{v}
% %\end{equation}

% %This equation sums all node representation $\mu^{(l)}_{v}$ in $I^{i+1}(h)$ to form a new representation for $\mu^{(l)}_{I^{i+1}(h)}$.
% %The boundary case is that when $i$ is 0, then $I^{i}(h)$ is the graph nodes in $\mathcal{V}$, \ie, $I^{0}(h) = h$.
% %Note that this formula propagates information from $\mathcal{S}^1$ to $\mathcal{S}^n$.
% %In order to do it in reversed order, we introduce the following formula:

% %\begin{equation}
% %\forall m \in I^{i+1}(h), I^{i}(m) = \frac{\mu^{(l)}_{I^{i+1}(h)}}{|I^{i+1}(h)|}
% %\end{equation}

% %It means that an interval propagates its representation to its nodes by averaging the representation.
% %In this way, we can propagate information from $\mathcal{S}^n$ to $\mathcal{S}^1$.

% %The above two formulas propagate node information between intervals. 
% %For information propagation inside an interval, we leverage traditional GGNN to do the propagation.

% By repeating the interval-based propagation model for $L$ steps, we sum the final embeddings of all nodes in the graph to represent a method.

% \subsection{Bug Detection}
% Given the embedding vector of a method, We use a Feed Forward Neural Network (FFNN)~\cite{svozil1997introduction} to predict if the method is buggy. When a method is predicted to be buggy, we continue to predict the lines on which a bug resides. Given a node embedding $\mu_i^L$, which represents a single line in the method, we use another FFNN to predict if a line is buggy. 
%To inject flexibility into the prediction at the level of lines, we use another hyperparamter as the threshold to determine the presence of a bug.

%to locate the buggy line.
%Similarly, we use $\mu_i^L$ to represent node $i$ and use another FFNN to compute its value.
%Then we sort the values and regard the top-N values (\ie, nodes) as buggy.



%After training our graph neural networks for $L$ steps, there is $\mu_i^L$ for each node in $\mathcal{V}$.
%We sum all $\mu_i^L$ in a method and the result is denoted as final representation for a method.
%Then, we use a feed forward neural network (FFNN) \cite{svozil1997introduction} to transform the vector into a value, using it to identify whether the method is buggy.

%When a method is buggy, then we try to locate the buggy line.
%Similarly, we use $\mu_i^L$ to represent node $i$ and use another FFNN to compute its value.
%Then we sort the values and regard the top-N values (\ie, nodes) as buggy.


==> GGNN_paper-(submission)/Sections/Conclusion.tex <==
% !TeX root = ../NeurSA.tex

\section{Conclusion}\label{sec:conclusion}
% Although static analysis in bug finding has been an active research area for decades, it still face important challenges (\eg precision, scalability and user-friendliness) to be widely adopted in practice. 

% We have realized our approach in a framework, \tool, which in principle can create any neural bug detector given a sufficient amount of training data.
% Three neural bug detectors we instantiate from \tool are highly effective in catching null pointer dereferencing, array index out of bound and class casting bugs. Compared to several static analysis tools, our neural bug detector displayed a superior performance. Our neural bug detectors have also caught new bugs in XXXXX on GitHub, which we have reported to the developers. 


% In this paper, we present \tool, a framework for creating neural bug detectors. Specifically, we leverage the power of GNN to train a model for classifying buggy code from non-buggy code. We also propose an interval-based propagation model to improve the capacity of GNN in learning program properties. Through our extensive evaluation, \tool displays a superior performance over the prior works in catching semantic bugs. Moreover, when deployed in the wild, \tool also manages to catch many bugs in several highly-rated and actively maintained projects on GitHub. For future work, we will further evaluate and improve \tool so that it can be readily deployed as a bug checker. More importantly, we will apply IBPM-Based GNN to other program analysis tasks as we believe the methodology offers a general, and powerful technique for learning semantic program embeddings.

In this paper, we present \tool, a framework for creating neural bug detectors based on GNN. We also propose an interval-based propagation model to improve the capacity of GNN in learning program properties. Our evaluation shows that \tool is effective in catching semantic bugs; it outperforms several flagship static analyzers in catching null pointer dereference bugs; and even finds new bugs in many highly-rated and actively maintained projects on GitHub. For future work, we will apply the IBPM-Based GNN to other program analysis tasks as we believe our approach offers a general, and powerful framework for learning effective program analyzers.





% and is even capable of finding bugs in several highly-rated and actively maintained projects on GitHub. For future work, we will further evaluate and improve \tool so that it can be readily deployed as a bug checker. More importantly, we will apply IBPM-Based GNN to other program analysis tasks as we believe the methodology offers a general, and powerful framework for learning semantic program embeddings.


==> GGNN_paper-(submission)/Sections/Discussion.tex <==
% !TeX root = ../ggnn.tex

\section{Limitation}\label{sec:discussion}
% This section discusses the limitation of \tool, and several other related subject matters.

% \subsection{Limitation}
We also discovered several issues that prevented \tool from being more effective. One, in particular, is the scalability. \tool is notably less accurate when handling larger programs despite the contribution IBPM makes to the underlying GNN. Naturally, steady advances in deep learning research would keep pushing the limit of model capacity. As a result, solutions in the specific application domains would continue to get better. In addition, we conjecture that better program representation that enables deep learning models to fulfill their potential may exist and worth exploring. Most importantly, we believe fundamental research aiming to explain why GNN can learn to analyze programs is necessary. Without a deeper understanding of GNNs, IBPM's results will be hard to improve upon.

% Even though IBPM significantly improves GNN's scalability, \tool tends to mishandle large programs. Steady advances in the deep learning community would keep pushing the limit of model capacity. As a result, solutions in the specific application domains would continue to get better. In addition, we conjecture that better program representation that enables deep learning models to fulfill their potential may exist and worth exploring. Most importantly, we believe fundamental research aiming to explain why GNN can learn to analyze programs is necessary. Specifically, how is the message-passing protocol, a seemingly effective technique on a general-purpose graph structure, even a sensible approach for any graph representation of a program? Answers to those questions help to diagnose the cause of GNN's shortcomings and stimulate future research. 

\tool is also limited by the availability of high-quality, large-scale datasets. Even with the synthetic buggy code injected into our dataset, it is not nearly at the same scale as other machine learning datasets (\eg ImageNet~\cite{russakovsky2015imagenet}). Considering the size and complexity of programs, it is fair to argue dataset of programs should be even larger for sufficiently training a quality model. 
% The difficulty though is the tremendous human effort that is needed to assemble such a dataset even with the abundant, freely accessible repositories of source code. Because automating this process involves other manual work such as identifying buggy code snippets, analyzing their root causes, collecting the corresponding fixes, \etc Examples like BugSwarm~\cite{tomassi2019bugswarm} have made great strides, however, we have found it to be significantly more noisy than defect4j and bugs.jar, two manually analyzed datasets.
% in our experiments. 

When applying \tool to catch bugs in the wild, we find \tool could have been a more useful bug-finding tool if it can provide justification to the developers as to why a particular code snippet is predicted to be buggy. We believe this issue can be promptly addressed by incorporating the ideas from a long line of works in the explainability of machine learning models~\cite{guidotti2019survey}. At the very least, \tool can highlight the regions of programs that have the most influence on its predictions, a technique researchers developed to explain why an image is predicted in a certain category.

% \subsection{Dealing with Noise}
% % \ignore{\gfj{As discussed in \cite{kim2011dealing}, recent studies have discovered that data so collected contain noises because current defect collection practices are based on optional bug fix keywords or bug report links in change logs. Automatically collected defect data based on the change logs could include noises.}}

% Recent studies~\cite{kim2011dealing} have discovered that the datasets used for training bug detectors can be noisy. We discuss two potential sources that could introduce noise in our datasets. 

% First, bugs types can be mislabeled (\eg null pointer dereference can be labeled as an array index out of bound). As explained in Section~\ref{subsec:over}, we determine the type of a bug by matching key words in the bug report. Even though the correctness can not be guaranteed, it is fair to disregard mislabeling as a serious issue. Because the nature of the three types of bugs we deal with is very different. Unless developer made a mistake in describing the bug in the report, the way we determine a bug type should be reliable. 

% Second, identifying a buggy method based upon the code patches is unsound. It is entirely possible for developers to commit quick hack around instead of fixes that address the root cause of the bug. However, since our datasets are well-studied in the literature, noise caused by imprecise fixes should be minimal. For the manually checked bugs, 79 in total, we only tweaked one bug location, which signals the quality of our datasets.

% % To confirm our hypothesis, we randomly pick 100 bugs in our datasets for manual inspection, and we find that all of them have not only the correct labels of bug types but also the correct locations in the method. 

% % \ignore{
% % \wyc{To further avoid noisy data, we use defects4j and bugs.jar as the ground truth (\ie, testing dataset) because they are widely used datasets. 
% % In contrast, the training dataset extends the dataset provided by \citet{ye2014learning}, which might be more noise and thus is not suitable to be the ground truth.}

% % We found that there is only one exception.
% % The case is that the code snippet contains a comment about NPE bug, which is identified as an NPE bug in \tool.
% % From the result we can claim that the noise in our datasets is small enough to be used in evaluation.}

% Finally, even though the noise is inevitable, our neural bug detectors beat the baseline on a level playing field.

% % \ignore{It is an unsound way and thus may miss related bugs.
% % However, it barely collects wrong bugs because if a bug report mentions some exception such as \textit{NullPointerException}, it probabily related to the null pointer bug.
% % The second kind is from imprecise patch analysis, \ie, identification of buggy methods and buggy lines.
% % There would be many incorrect/redundant buggy methods if we did not ignore some buggy irrelevant operations, new blank lines in a method for example.}

% % \subsection{Data Sufficiency}


% % \begin{figure}[htb!]
% % \captionsetup{justification=centering}
% % \begin{subfigure}{.4\textwidth}
% % \centering
% %   \includegraphics[width=\linewidth]{Figures/dataSizePerf.png}
% %   \caption{F1 score on NPE bugs.}
% %   \label{fig:dataSizePerfNPE}
% % \end{subfigure}
% % \par\bigskip
% % \begin{subfigure}{.4\textwidth}
% % \centering
% %   \includegraphics[width=\linewidth]{Figures/dataSizePerfArray.png}
% %   \caption{F1 score on AIOE bugs.}
% %   \label{fig:dataSizePerfArray}
% % \end{subfigure}
% % \par\bigskip
% % \begin{subfigure}{.4\textwidth}
% % \centering
% %   \includegraphics[width=\linewidth]{Figures/dataSizePerfCCE.png}
% %   \caption{F1 score on CCE bugs.}
% %   \label{fig:dataSizePerfCCE}
% % \end{subfigure}
% % \caption{How F1 varies as training data increase.}
% % \label{fig:dataSizePerf}  
% % \end{figure}

% % In this experiment, we examine the sufficiency of our training data. Specifically, starting from 10\% of the original training data, we gradually increase the percentage to investigate the performance trend for the three sets of neural bug detectors built by \tool and two other baselines. The testing data is kept intact for this experiment.
% % %\wyc{WY: updated to the three bug dataset instead of one}
% % %We measure the data sufficiency for all the three kinds of datasets we used.
% % %TODO: add results.
% % %The result in Fig. \ref{fig:dataSizePerf} shows the line chart of F1 score in different percentage of our dataset.
% % Figure~\ref{fig:dataSizePerf} shows how the F1 scores change as the percentage of the original training data increases. 
% % %is $N$ and Y-axis is the F1 score.
% % %$N$ ranges from 10 to 100, denoting that we use 10\% to 100\% of dataset for training.
% % Figure~\ref{fig:dataSizePerfNPE} shows the three competing models in catching null pointer dereference bugs. Three models show similar convergence. That is when reaching 80\% all three models show little improvements onward. Even at 50\%, their performances do not change by a big margin. 
% % %In fact, the performance becomes close to each other when there is more than 50\% of dataset.
% % Compared to the two baselines, the model built based on \tool requires less training data to converge. Overall, we conclude our data set is sufficient for training detectors of null pointer dereference bugs.
% % %Therefore, the number of bugs is enough for our evaluation.

% % %Note that it is the F1 score on NPE dataset, which is the largest dataset among the three bug datasets we used.
% % %The other two datasets include 14.4\% and 22.4\% of NPE dataset.

% % Figure~\ref{fig:dataSizePerfArray} and~\ref{fig:dataSizePerfCCE} shows 
% % the performance trend of the other two classes of bug detectors. Compared to the null pointer dereference bug detectors, all array index out of bound bug detectors display a smoother convergence, indicating the lower complexity in learning the semantic patterns of array index out of bound bugs. Similarly, class casting bugs detectors also seem to require less amount of training data to generalize compared to the null pointer dereference bugs. According to our manual inspection, the reason is that the patterns of null pointer dereference bugs are significantly more diverse than those of the other two bug types. To some degree, it also explains null pointer dereference bugs are harder to prevent, which tend to occur more frequently than other types of bugs in software development. 
% % % We list several examples of null pointer dereference bugs in Figure~\ref{fig:NPEs} we encountered in our dataset. 

% % Overall, we demonstrate in this experiment, the training data for all three sets of bug detectors are sufficient. Bug detectors instantiated from \tool tend to converge early with higher precision.
% % \ignore{
% % The bug in Figure~\ref{fig:npe1} is caused by calling a null pointer because \texttt{context.getManager()} may return $\mathit{NULL}$.
% % Fig. \ref{fig:npe2} misses an additional check to avoid \texttt{null == null} while Fig. \ref{fig:npe3} introduces an NPE by splitting empty data.
% % Fig. \ref{fig:npe4} shows an NPE caused by insufficient checks because \texttt{failureDetector} itself can be $\mathit{NULL}$.
% % Therefore, we should check \texttt{failureDetector} first and then check whether \texttt{failureDetector.get()} is success.}





% % \ignore{
% % The performance of the two datasets is similar to the NPE dataset,
% % the reason is that different kinds of bugs require various training data.
% % For example, the pattern in class cast exception is more clear because almost every buggy lines have type cast operations.
% % Similarly, array index out of bound exception has a pattern in the form of $array[index]$, which is also more clear comparing to null pointer dereference bugs.
% % However, the pattern of NPE bug is various and depends on how to use a pointer.
% % This is also the reason why the number of NPE bugs is significantly larger than the other two.
% % For instance, examples in Fig. \ref{fig:NPEs} are found when we inspect the NPE dataset.
% % The bug in Fig. \ref{fig:npe1} is caused by calling a null pointer because \texttt{context.getManager()} may return $\mathit{NULL}$.
% % Fig. \ref{fig:npe2} misses an additional check to avoid \texttt{null == null} while Fig. \ref{fig:npe3} introduces an NPE by splitting empty data.
% % Fig. \ref{fig:npe4} shows an NPE caused by insufficient checks because \texttt{failureDetector} itself can be $\mathit{NULL}$.
% % Therefore, we should check \texttt{failureDetector} first and then check whether \texttt{failureDetector.get()} is success.}




% % \begin{figure*}[htbp!]
% % %\centering
% % \ignore{
% % \begin{subfigure}[b]{1\textwidth}
% % \begin{mdframed}[roundcorner=5pt]
% % \scriptsize
% % \begin{lstlisting}[language=C++,showstringspaces=false]
% % ...
% % scriptContext.getContext().setApplicationClassLoader(
% %     getApplicationClassLoader());
% % ...
% % \end{lstlisting}
% % \vspace*{-4pt}
% % \end{mdframed}
% % \caption{\label{fig:npe1} NPE caused by calling a null pointer.}
% % \end{subfigure}
% % }



% % \begin{subfigure}[b]{1\textwidth}
% % \begin{mdframed}[roundcorner=5pt]
% % \scriptsize
% % \begin{lstlisting}[language=C++,showstringspaces=false]
% % // Extracted from tomcat-e14afee
% % public void list(HttpServletRequest request,
% %                 HttpServletResponse response,
% %                 String message) throws IOException {
% %     ...               
% %     // context.getManager() may return null.
% %     args[11] = new Integer(context.getManager().getMaxInactiveInterval()/60);
% %     ...
% % }
% % \end{lstlisting}
% % \vspace*{-4pt}
% % \end{mdframed}
% % \caption{\label{fig:npe1} NPE caused by missing check. }
% % \end{subfigure}


% % \begin{subfigure}[b]{1\textwidth}
% % \begin{mdframed}[roundcorner=5pt]
% % \scriptsize
% % \begin{lstlisting}[language=C++,showstringspaces=false]
% % // Extracted from bugs-dot-jar_FLINK-1167
% % public void setNextPartialSolution(OptimizerNode nextPartialSolution,
% %                                 OptimizerNodeterminationCriterion) {
% %     ...
% %     if (nextWorkset == worksetNode) {
% %         PactConnection noOpConn = new PactConnection(nextWorkset, noop);
% %         ...
% %     }
% %     ...
% % }
% % \end{lstlisting}
% % \vspace*{-4pt}
% % \end{mdframed}
% % \caption{\label{fig:npe2} NPE caused by comparing two $\mathit{NULL}$s.}
% % \end{subfigure}


% % \begin{subfigure}[b]{1\textwidth}
% % \begin{mdframed}[roundcorner=5pt]
% % \scriptsize
% % \begin{lstlisting}[language=C++,showstringspaces=false]
% % // Extracted from bugs-dot-jar_FLINK-1922
% % public InputSplit getNextInputSplit() {
% %     ...
% %     byte[] serializedData = nextInputSplit.splitData();
% %     deserializeObject(serializedData);
% %     ...
% % }
% % \end{lstlisting}
% % \vspace*{-4pt}
% % \end{mdframed}
% % \caption{\label{fig:npe3} NPE caused by splitting empty data of Byte class. }
% % \end{subfigure}




% % \begin{subfigure}[b]{1\textwidth}
% % \begin{mdframed}[roundcorner=5pt]
% % \scriptsize
% % \begin{lstlisting}[language=C++,showstringspaces=false]
% % // Extracted from tomcat-eb9f94e
% % protected void sendPing() {
% %     ...
% %     // Variable failureDetector itself can be null. 
% %     if (failureDetector.get() != null) {
% %         ...
% %     }
% %     ...
% % }
% % \end{lstlisting}
% % \vspace*{-4pt}
% % \end{mdframed}
% % \caption{\label{fig:npe4} NPE caused by insufficient check that misses the object. }
% % \end{subfigure}


% % \begin{subfigure}[b]{1\textwidth}
% % \begin{mdframed}[roundcorner=5pt]
% % \scriptsize
% % \begin{lstlisting}[language=C++,showstringspaces=false]
% % // Extracted from eclipse.platform.ui-6102a2f
% % private boolean isStatusLine(Control ctrl) {
% %     ...
% %     // element.getElementId() can also return null.
% %     if (element != null
% %         && element.getElementId().equals("org.eclipse.ui.StatusLine"))
% %         return true;
% %     return false;
% % }
% % \end{lstlisting}
% % \vspace*{-4pt}
% % \end{mdframed}
% % \caption{\label{fig:npe5} NPE caused by insufficient check that misses the return value of a method. }
% % \end{subfigure}

% % \caption{Illustrative examples of a variety of the NPE bugs.}
% % \label{fig:NPEs}
% % \end{figure*}



% \subsection{Dataset Selection}
% We pick datasets that are widely studied in the literature~\cite{just2014defects4j,saha2018bugs,ye2014learning}. Given their generality and representativeness, we believe \tool's performance is likely to transfer to many other projects. 
% % \ignore{The examined projects in this work have a large variance
% % in average buggy rates. We have tried our best to make our dataset general and representative. However, it is still possible that these projects are not generalizable enough to represent all software projects. Given projects that are not included in the 18 projects, our proposed approach might generate better or worse results. \tool is only evaluated on open source Java projects. Its performance on closed source software and projects written in other languages is unknown.}

% \subsection{Bug Selection}
% %The examined bugs in this work are highly depend on the number of bug reports in the dataset.
% We have analyzed all kinds of Java runtime exceptions in our dataset, and show their distributions in Figure~\ref{fig:numOfBugs}. We chose null pointer dereference, array index out of bound and class casting bugs to create neural bug detectors because they are among the highest occurrence of bugs in the codebases. We did not use illegal argument exceptions despite having enough data. The reason is vast majority of the bugs can be caught by a simple type checker on the argument of the caller and the parameter of the callee. Other bugs like out of assertion error are short of data for building bug detectors despite their important roles in ensuring software quality. 

% % \ignore{even though it is important to detect whether an assertion can be violated or not.
% % There are many bugs that are also as important as NPE bugs, but the number of bugs are only tens, such as stack overflow bugs.}

% \begin{figure}
% \centering
%   \includegraphics[width=\linewidth]{Figures/numOfBugs.pdf}
%   \caption{Bug distributions of our dataset.}
%   \label{fig:numOfBugs}
% \end{figure}

% \subsection{Generalizing to Other Programming Languages}
% \tool is a general framework across different programming languages. In particular, generalizing to another language only requires a new extractor that constructs the graph representation for programs in the new language, the rest of the workflow is language-agnostic.
% % \subsection{Limitation}
% % We pick datasets that are widely studied in the literature~\cite{just2014defects4j,saha2018bugs,ye2014learning}. Given their generality and representativeness, we believe \tool's performance is likely to transfer to many other projects. 

==> GGNN_paper-(submission)/Sections/Evaluation.tex <==
% % !TeX root = ../ggnn.tex
% \section{Evaluation}\label{sec:evaluation}
% This section presents an extensive evaluation of the three neural bug detectors we instantiate from \tool. First, we evaluate the performance of each neural bug detector. Next, we highlight the improved model capacity IBPM attributes to. Finally, we show how our neural bug detector fares against several static analysis tools in catching null pointer dereference bugs, followed by a summary of applying \tool to catch bugs in the wild.

% % Finally, we describe XXX bugs caught by our neural bug detector in XXXX Java projects. %on GitHub.
% % compare the bug detectors built based on \tool against those based on an existing AST-based GNN. Next, we highlight the improved generalization of GNN IBPM attributes. Besides, we also show how our neural bug detector fares against several static analysis tools in catching null pointer dereference bugs. Finally, we describe XXX new bugs discovered by our neural bug detector in XXXX popular Java projects on GitHub. 


% % \begin{table*}[!tbp]
% % \caption{Projects used in the evaluation.}
% % % \adjustbox{max width=1.5\paperwidth}{
% % \centering
% % \small
% % \begin{tabular}{c|c|c|c|ccc}
% % \hline
% %  \multirow{2}{*}{Dataset} & \multirow{2}{*}{Projects} & \multirow{2}{*}{Description}& \multirow{2}{*}{Size (KLoC)}&  \multicolumn{3}{c}{\# of Bugs} \\
% % \cline{5-7}
% % & & & &\tabincell{c}{NPE} & \tabincell{c}{AIOE} & \tabincell{c}{\tabincell{c}{CCE}} \\\hline
% % \multirow{13}{*}{Test} &Lang & Java lang library &50 & 7 & 5 & 2  \\\cline{2-7}
% % &Closure & A JavaScript checker and optimizer. &260 & 18 & 0 & 0  \\\cline{2-7}
% % &Chart & Java chart library &149 & 17 & 7 & 0  \\\cline{2-7}
% % &Mockito & Mocking framework for unit tests &45 & 14 & 5 & 23  \\\cline{2-7}
% % &Math & Mathematics and statistics components &165 & 16 & 17 & 3  \\\cline{2-7}
% % &Accumulo & Key/value store &194 & 6 & 0 & 0  \\\cline{2-7}
% % &Camel & Enterprise integration framework &560 & 17 & 1 & 1  \\\cline{2-7}
% % &Flink & System for data analytics in clusters &258 & 13 & 0 & 0  \\\cline{2-7}
% % &Jackrabbit-oak & hierarchical content repository &337 & 23 & 1 & 1  \\\cline{2-7}
% % &Log4j2 & Logging library for Java &70 & 29 & 1 & 2  \\\cline{2-7}
% % &Maven & Project management and comprehension tool & 62 & 6 & 0 & 0  \\\cline{2-7}
% % &Wicket & Web application framework &206 & 7 & 1 & 8  \\\cline{2-7}
% % &from BugSwarm & 61 projects on GitHub & 5191 & 156 & 20 & 3  \\\hline
% % \hline
% % \multicolumn{4}{r|}{Total}& 271 & 58 & 41  \\\hline % (num) is the number of buggy methods
% % \hline
% % \multirow{6}{*}{Training}&Birt & Data visualizations platform &1093 & 678 & 129 & 154  \\\cline{2-7}
% % &JDT UI & User interface for the Java IDE & 508 & 897 & 63 & 156 \\\cline{2-7}
% % &SWT & Eclipse Platform project repository & 460 & 276 & 136 & 26  \\\cline{2-7}
% % &Platform UI & User interface and help components of Eclipse & 595 & 920 & 72 & 194  \\\cline{2-7}
% % &AspectJ & An aspect-oriented programming extension &289 & 151 & 14 &  19 \\\cline{2-7}
% % &Tomcat & Web server and servlet container &222 & 111 & 18 & 28  \\\hline
% % \hline
% % \multicolumn{4}{r|}{Total}& 3033 & 432 & 577  \\\hline
% % \end{tabular}
% % % }
% % \label{tab:methodres}
% % \end{table*}


% \subsection{Implementation}\label{subsec:impl}
% Due to the popularity and availability of Java datasets, we target semantic bugs in Java programs. For a different language, \tool only requires a front-end analyzer that extracts the control flow graphs for programs in the new language, the rest of the workflow is language-agnostic. We construct the control flow and interval graphs using Spoon~\cite{pawlak:hal-01169705}, an open-source library for analyzing Java source code.  To efficiently choose correct methods to pair with each buggy method, we run DECKARD~\cite{4222572}, a clone detection tool adopting an approximation of the shortest tree edit distance algorithm to identify similar code snippets. 

% We realize our IBPM-based GNN based on GGNN's implementation~\cite{li2015gated}. All neural bug detectors are implemented in Tensorflow. All RNNs built in the model have 1 recurrent layer with 100 hidden units. Each token in the vocabulary is embedded into a 100-dimensional vector. We experimented with other model configurations (\eg more recurrent layers, hidden units, \etc) and did not obtain better results. We use random initialization for weight initialization. We train the neural bug detectors using the Adam optimizer~\cite{kingma2014adam}. All experiments are performed on a 3.7GHz i7-8700K machine with 32GB RAM and NVIDIA GTX 1080 GPU.


% % \subsection{Metrics}
% % Since we deal with largely unbalanced dataset (\ie the amount of correct code is significantly larger than that of the buggy code), we forgo the accuracy metric. Instead we opt for Precision, Recall, and F1 Score, metrics are commonly used in defect prediction literature~\cite{wang2016automatically,pradel2018deepbugs}.

% % \begin{equation*}
% % \mathit{Precision} =  \dfrac{\mathit{TP}}{\mathit{TP} + \mathit{FP}}
% % \end{equation*}

% % \begin{equation*}
% %  \mathit{Recall} =  \dfrac{\mathit{TP}}{\mathit{TP} + \mathit{FN}}
% % \end{equation*}

% % \begin{equation*}
% %  \mathit{F1} =  \dfrac{2 \times \mathit{Precision} \times \mathit{Recall}}{\mathit{Precision} +\mathit{Recall}}
% % \end{equation*}

% % TP, FP, FN stand for true positive, false positive, and false negative respectively. True positive is the number of predicted buggy lines that are truly buggy, while false positive is the number of predicted buggy lines that are not buggy. False negative records the number of buggy lines that are predicted as clean. A higher precision suggests relatively lower number of false warnings while high recall indicates relatively lower number of missed bugs. F1 takes both precision and recall into consideration. 
% % The reason we add the prefix of "Top-" is

% % after a method is predicted to be buggy our model ranks the statements according to their probabilities of being buggy, 
% %the manual inspection on a certain amount of predicted defective methods find more defects, while an increase in recall can reveal more
% %defects given a project. F1 takes both precision and recall into consideration.

% %To evaluate the performance of defect prediction at the line-level, we use the same three metrics for top-N prediction results. By top-N predictions, we mean considering the top N lines to be buggy ranked by the predicted probabilities, which also implies that the rest of the lines are predicted to be correct. In line-level prediction, TP, FP, FN, TN narrow down the prediction granularity to the level of lines. For example, true positive is the number of predicted defective lines that are truly defective.
 
% %means that the correct line gets to be in the top-N probabilities for it to count as ``correct''.

% % \begin{equation}
% % \label{equ:topn}
% % \text{Top-N Recall} =  \dfrac{TP_N}{TP_N + FN_N}
% % \end{equation}

% % We introduce another metric, top-N recall, dedicated to the prediction at the level of lines. Top-N refers to considering the top N lines to be buggy ranked by the predicted probabilities in a buggy method. Given the top-N predictions, we compute the recall as the only metric of line-level prediction. Our intuition is to favour predictions that capture all bugs in a method. Even it emits a high rate of false warnings, the issue should not be considered as serious since N is a small number. On the contrary, low recall would seriously hurts the usability of a bug finder. As a method is already predicted to be buggy, low recall provides little extra information for developer to pinpoint a bug.


% %Note that recall in top-N is the same as top-N accuracy, thus we use recall instead of top-N accuracy. The reason is that each method has only one buggy line according to our setup, and it can be true positive or false negative. The condition is similar in top-N accuracy because whether method is either buggy or clean depends on whether the buggy line is correctly predicted.

% %Even though the total number of bugs for them are 1186, 160 and 188 separately, the total number of buggy methods are 2085, 301 and 466.
% %The reason is that developers may add patches for more than one method,
% %which are all regarded as buggy.
% %Therefore, the number of buggy methods are more than the number of bugs.

% %Note that we classify all projects into two datasets.
% %The first 12 projects are in the testing dataset and the last 6 projects are in the training dataset.
% %The evaluation is focus on the cross-project defect prediction, which is more important and has more practical impact than within-project defect prediction.


% \begin{table*}[h]
% \caption{Details about our dataset. NPE, AIE, and CCE stand for null pointer dereference, array index out of bound and class cast exceptions respectively. Numbers in parenthesis records the number of synthetic bugs we created for AIE and CCE.}
% \adjustbox{max width=.8\paperwidth}{
% \centering
% \small
% \begin{tabular}{c|c|c|c|ccc}
% \hline
%  \multirow{2}{*}{Dataset} & \multirow{2}{*}{Projects} & \multirow{2}{*}{Description}& \multirow{2}{*}{Size (KLoC)}&  \multicolumn{3}{c}{Number of Buggy Methods} \\
% \cline{5-7}
% & & & &\tabincell{c}{NPE} & \tabincell{c}{AIE} & \tabincell{c}{\tabincell{c}{CCE}} \\\hline
% \multirow{13}{*}{Test} &Lang & Java lang library &50 & 7 & 5 & 2  \\\cline{2-7}
% &Closure & A JavaScript checker and optimizer. &260 & 18 & 0 & 0  \\\cline{2-7}
% &Chart & Java chart library &149 & 17 & 7 & 0  \\\cline{2-7}
% &Mockito & Mocking framework for unit tests &45 & 14 & 5 & 23  \\\cline{2-7}
% &Math & Mathematics and statistics components &165 & 16 & 17 & 3  \\\cline{2-7}
% &Accumulo & Key/value store &194 & 6 & 0 & 0  \\\cline{2-7}
% &Camel & Enterprise integration framework &560 & 17 & 1 & 1  \\\cline{2-7}
% &Flink & System for data analytics in clusters &258 & 13 & 0 & 0  \\\cline{2-7}
% &Jackrabbit-oak & hierarchical content repository &337 & 23 & 1 & 1  \\\cline{2-7}
% &Log4j2 & Logging library for Java &70 & 29 & 1 & 2  \\\cline{2-7}
% &Maven & Project management and comprehension tool & 62 & 6 & 0 & 0  \\\cline{2-7}
% &Wicket & Web application framework &206 & 7 & 1 & 8  \\\cline{2-7}
% &Birt & Data visualizations platform &1,093 & 678 & 129 & 154  \\\hline
% \hline
% \multicolumn{4}{r|}{Number of Buggy Methods in Total for Test}& 793 & 167 & 192  \\ % (num) is the number of buggy methods
% \multicolumn{4}{r|}{Number of Methods in Total for Test}& 3,000 & 600 & 800  \\\hline % (num) is the number of buggy methods
% \hline
% \multirow{6}{*}{Training}
% &JDT UI & User interface for the Java IDE & 508 & 897 & 63 & 156 \\\cline{2-7}
% &SWT & Eclipse Platform project repository & 460 & 276 & 136 & 26  \\\cline{2-7}
% &Platform UI & User interface and help components of Eclipse & 595 & 920 & 72 & 194  \\\cline{2-7}
% &AspectJ & An aspect-oriented programming extension &289 & 151 & 14 &  19 \\\cline{2-7}
% &Tomcat & Web server and servlet container &222 & 111 & 18 & 28  \\\cline{2-7}
% &from BugSwarm & 61 projects on GitHub & 5,191 & 156 & 20 & 3 \\\cline{2-7}
% &from BugSwarm & 250 projects on GitHub & 19,874 & (0) & (2,356) & (1,998) \\\hline
% \hline
% % \multicolumn{4}{r|}{Total}& 2,511 & 323 & 426  \\\hline
% \multicolumn{4}{r|}{Number of Buggy Methods in Total for Training}& 2,511 & 2,679 & 2,424  \\
% \multicolumn{4}{r|}{Number of Methods in Total for Training}& 10,000 & 10,000 & 10,000  \\\hline
% \end{tabular}
% }
% \label{tab:stas}
% \end{table*}


% \subsection{Experiment Setup}
% We assemble a dataset according to the procedure described in Section~\ref{subsec:data}. Table~\ref{tab:stas} shows the details: the projects from which we extract the code snippet, a brief description of their functionality, size of their codebase, and the number of buggy methods we extract from each project. We maintain approximately a 3:1 ratio between the correct and buggy methods across each bug type within each project. 1,000 methods are randomly picked out of the training set for the validation purpose. To enrich the set of AIE (Array Index Out of Bound Exception) and CCE (Class Cast Exception) bugs, we create synthetic buggy examples based on a collection of highly-rated and actively maintained projects from BugSwarm~\cite{tomassi2019bugswarm}. In particular, we first randomly select methods that contain either array access or class cast operations, and then strip away the bound or type checks. The number in parenthesis depicts how many buggy examples we synthesized for AIE and CCE. Note that all synthetic bugs are used for the training purpose only, and all bugs in the test set are real. We also make certain clean methods that are paired with synthetic buggy examples are other methods rather than their original version (\ie with the bound or type checks). We evaluate \tool on a standard classification task, that is, predicting each line in a test method to be buggy or not. Since we deal with a largely unbalanced dataset, we forgo the accuracy metric and opt for Precision, Recall, and F1 Score, metrics are commonly used in defect prediction~\cite{wang2016automatically,pradel2018deepbugs}.

% As a baseline, we select standard GGNN~\cite{li2015gated,allamanis2017learning}, a predominate deep learning model in the domain of programming. In particular, we re-implemented the program encoding scheme proposed by~\citet{allamanis2017learning}, a graph representation built of top of an abstract syntax tree with additional edges denoting variable types, data, control dependencies, \etc


% % \begin{table}[!t]
% % \centering
% % \normalsize
% % \caption{Dataset statistics. NPE, AIE and CCE stand for null pointer deference, array index out of bound and class cast exceptions respectively.}
% % \adjustbox{max width=\columnwidth}{\begin{tabular}{c|ccc|ccc}
% % \hline
% %  \multirow{2}{*}{\tabincell{c}{Dataset}} & \multicolumn{3}{c|}{\# of Buggy Methods} & \multicolumn{3}{c}{\# of Clean Methods}\\
% % \cline{2-7}
% %          & NPE & AIE & CCE & for NPE & for AIE & for CCE  \\\hline
% % Training & 3033 & 432 & 577 & 3033 & 432 & 577    \\\hline
% % Test & 271 & 58 & 41 & 271 & 58 & 41    \\\hline

% % \end{tabular}}
% % \label{tab:stas}
% % \end{table}

% % \begin{table}[!t]
% % \centering
% % \normalsize
% % \caption{Dataset statistics. NPE, AIE and CCE stand for null pointer deference, array index out of bound and class cast exceptions respectively.}
% % \adjustbox{max width=\columnwidth}{\begin{tabular}{c|ccc|c}
% % \hline
% %  \multirow{2}{*}{\tabincell{c}{Dataset}} & \multicolumn{3}{c|}{\# of Buggy Methods} & \multirow{2}{*}{\tabincell{c}{\# of Clean Methods}}\\
% % \cline{2-4}
% %          & NPE & AIE & CCE &   \\\hline
% % Training & 3033 & 432 & 577 & 4000    \\\hline
% % Test & 271 & 58 & 41 & 400    \\\hline

% % \end{tabular}}
% % \label{tab:stas}
% % \end{table}



% % We use defect4j~\cite{just2014defects4j}, bugs.jar~\cite{saha2018bugs}, BugSwarm~\cite{tomassi2019bugswarm} and the other by~\citet{ye2014learning}, which are all real-world, publicly accessible datasets, for our evaluation. We select projects that contain at least one bug of null pointer dereference, array index out of bound or class cast in their codebases.

% % As mentioned previously, we obtain the labels for each buggy method and their lines by cross-referencing the commit history and bug reports. Specifically, we search for commits that are considered to be bug fixes, and infer the type of the bug by referencing the bug reports. Methods and lines that are modified by commits of bug fixes are labeled buggy. Finally, we pick a correct method that is syntactically similar to pair with the buggy method. 

% %unified these datasets with the following steps:
% %(1) Locate a bug description for each bug by string matching;
% %(2) Locate a commit that repairs each bug;
% %(3) Label buggy methods if they are inside the modification by a patch;
% %(4) Label clean methods whose complexity are similar to the buggy methods.

% % Table~\ref{tab:methodres} depicts all selected projects including a brief description of their functionality. The first column shows if a project is used in the training or test set, and the last three columns denote the number of bugs it contains for each type. We also provide the size of the codebase for each project.
% % % are the number of total methods for each of the three bug types. Numbers in parenthesis are the number of buggy methods. For the actual number of bugs and buggy methods in each project\footnote{Developers may fix multiple methods for a single bug so the number of buggy methods and bugs may not be identical.}, we invite readers to refer to the supplemental material for the details. 
% % Our evaluation focuses on the cross-project defect prediction, which resembles the real usage scenarios of \tool better than within-project defect prediction.


% % \begin{table*}[!tbp]
% % \caption{Projects used in the evaluation.}
% % \adjustbox{max width=\textwidth}{
% % \centering
% % \small
% % \begin{tabular}{c|c|c|ccc}
% % \hline
% %  \multirow{2}{*}{Dataset} & \multirow{2}{*}{Projects} & \multirow{2}{*}{Description}&  \multicolumn{3}{c}{\#Methods} \\
% % \cline{4-6}
% % & & &\tabincell{c}{NPE} & \tabincell{c}{AIOE} & \tabincell{c}{\tabincell{c}{CCE}} \\\hline
% % \multirow{13}{*}{Test} &Lang & Java lang library & 115 & 46 & 75  \\\cline{2-6}
% % &Closure & A JavaScript checker and optimizer. & 11 & 0 & 0  \\\cline{2-6}
% % &Chart & Java chart library & 120 & 5 & 0  \\\cline{2-6}
% % &Mockito & Mocking framework for unit tests & 49 & 6 & 42  \\\cline{2-6}
% % &Math & Mathematics and statistics components & 44 & 59 & 14  \\\cline{2-6} % 121+67, 139+145, 31
% % &Accumulo & Key/value store & 16 & 0 & 0  \\\cline{2-6}
% % &Camel & Enterprise integration framework & 155 & 20 & 6  \\\cline{2-6}
% % &Flink & System for data analytics in clusters & 33 & 0 & 0  \\\cline{2-6}
% % &Jackrabbit-oak & hierarchical content repository & 68 & 7 & 12  \\\cline{2-6}
% % &Log4j2 & Logging library for Java & 44 & 2 & 1  \\\cline{2-6}
% % &Maven & Project management and comprehension tool & 12 & 0 & 0  \\\cline{2-6}
% % &Wicket & Web application framework & 23 & 8 & 16  \\\hline
% % \hline
% % \multicolumn{3}{r|}{Total}& 690 (173) & 153 (38) & 166 (40)  \\\hline % (num) is the number of buggy methods
% % \hline
% % \multirow{6}{*}{Training}&Birt & Data visualizations platform & 1356 & 258 & 308  \\\cline{2-6}
% % &JDT UI & User interface for the Java IDE & 1794 & 126 & 312 \\\cline{2-6}
% % &SWT & Eclipse Platform project repository & 552 & 272 & 52  \\\cline{2-6}
% % &Platform UI & User interface and help components of Eclipse & 1840 & 144 & 388  \\\cline{2-6}
% % &AspectJ & An aspect-oriented programming extension & 302 & 28 &  38 \\\cline{2-6}
% % &Tomcat & Web server and servlet container & 222 & 36 & 56  \\\hline
% % \hline
% % \multicolumn{3}{r|}{Total}& 6066 (3033) & 864 (432) & 1154(577)  \\\hline
% % \end{tabular}}
% % \label{tab:methodres}
% % \end{table*}

% % \subsection{Baselines}
% % %To gain a better understanding of the performance of our neural bug detectors, 
% % We compare \tool against the standard GGNN~\cite{li2015gated,allamanis2017learning}, a predominate deep learning model in the domain of programming. In particular, we re-implemented the program encoding scheme proposed by~\citet{allamanis2017learning}, a graph representation built of top of the AST with additional edges denoting variable types, data, control flow dependencies, \etc
% % For convenience, we refer the first baseline as AST method and the second as CFG method. 

% % proposed in while the second one uses a control flow graph-based program encoding. In both methodologies, we feed the program graphs to a standard GGNN built with the existing propagation model. 

% % \ignore{
% % To evaluate the performance of our method in defect
% % prediction, we compare interval graphs with traditional graphs and compare CFG-based representations with AST-based representations~\cite{allamanis2017learning}. 
% % Our first baseline is CFG-based representation without introducing intervals.
% % Except for the interval representation and node representation, other setups are the same as \tool.
% % For a fair comparison, our second baseline of graph representation is based on AST that without taking control flow into consideration. 
% % }


% %Moreover, The second baseline is a re-implementation of AST-based program representation \cite{allamanis2017learning}, which additionally adds data flow edges in the graph constructed from AST and leverages variable type information. The graph in AST is a tree, with an additional kind of edge that connects leaf nodes from one side to another side.



% % \subsection{Compare Node Initializations}
% % We compare the three encoding schemes for node initialization: characteristic vectors, RNN-based encoding and transformer-based encoding. We show the performance of each encoding at both method-level and line-level predictions.

% % Table \ref{tab:alter} presents the method-level prediction results of the three encoding schemes in precision, recall and F1. Figure~\ref{fig:alterComp} shows the average of all three metrics across all bug types for each encoding. We find that GGNN exhibits a decent performance in all node initialization schemes. 
% % %The reason is that the representations and information propagation enable \tool to reason about semantic similarities between syntactically different methods, which allows it to learn and predict bugs across similar methods. 
% % In particular, RNN-based encoding has the highest recall and F1 score in all three bug types (\ie on average higher than characteristic vectors and transformer-based encoding by 12.9\% and 12.0\% respectively), indicating it's the most precise encoding scheme for node initialization.
% % %best representation among the three methods.
% % %For example, the average improvement of F1 introduced by RNN-based encoding is 10.3\% and 3.3\% for characteristic vectors and transformer-based encoding.

% % As for the line-level predictions, we depict the average top-N recall across all bug types for each encoding scheme in Figure~\ref{fig:alterCompLine}. The characteristic vectors based encoding again falls behind whereas the RNN-based encoding shows a slight advantage over transformer-based encoding. The reason is that characteristic vectors do not capture as precise a representation of a statement as the other two. As for the transformer, we find their capabilities do not transfer to the programming field. We suspect this is caused by the fundamental difference between program language and natural language.

% % Based on the comparison among the three encoding schemes for node initialization, we choose the RNN-based encoding as \tool's default configuration, in which we compare \tool against the 
% % two baselines in the remaining experiments.

% % \ignore{
% % conthis one for the remaining evaluation, including the performance of \tool between AST method and CFG method and the requirement about the number of bugs in the dataset.


% % at both method- and line-level predictions, 



% % The result shows that RNN-based encoding shows the best performance among the three alternative representations.
% % Therefore, we choose this one for the remaining evaluation, including the performance of \tool between AST method and CFG method and the requirement about the number of bugs in the dataset.









% % the results are depicted in Figure~\ref{fig:alterCompLine} with the average F1 score between the three representations.
% % The characteristic vectors embedding is still the worst one among the three while the RNN-based encoding shows a slightly benefit than transformer-based encoding.

% % The reason is that characteristic vectors are not expressive enough to capture semantic features of methods.
% % As for the transformer, it demonstrates that syntax of methods is different from the natural language \cite{vaswani2017attention}, leading to the different performance between RNN-based encoding and transformer-based encoding.

% % The result shows that RNN-based encoding shows the best performance among the three alternative representations.
% % Therefore, we choose this one for the remaining evaluation, including the performance of \tool between AST method and CFG method and the requirement about the number of bugs in the dataset.
% % }

% % \begin{figure}[h]
% % \begin{subfigure}[t]{0.47\textwidth}
% % \centering
% %   \includegraphics[width=0.95\linewidth]{Figures/alterComp.pdf}
% %   \caption{Compare the average precision, recall and F1 for different node initialization schemes.}
% %   \label{fig:alterComp}
% % \end{subfigure}\hfill
% % \begin{subfigure}[t]{0.47\textwidth}
% % \centering
% %   \includegraphics[width=0.95\linewidth]{Figures/alterCompLine.png}
% %   \caption{Average top-N recall of different node initialization schemes.}
% %   \label{fig:alterCompLine}
% % \end{subfigure}
% % \caption{Comparison among the different node initialization schemes using average across all bug types.}
% % \label{fig:alterPerf}
% % \end{figure}


% % \begin{table*}[!t]
% % \centering
% % \small
% % \caption{Compare the different encoding for node intialization.}
% % \begin{tabular}{c|ccc|ccc|ccc}
% % \hline
% % \multirow{2}{*}{\tabincell{c}{Node \\Representations}} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{AIOE} & \multicolumn{3}{c}{CCE}\\
% % \cline{2-10}
% % & Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall & F1 \\\hline
% % \tabincell{c}{Characteristic\\vectors}&  26.6 & 64.0 & 37.6 & 40.1 & 82.1 & 53.9 & 27.9 & 52.4 & 36.4   \\\hline
% % \tabincell{c}{RNN-based\\encoding } & \textbf{30.3} & \textbf{72.1} & \textbf{42.6} & \textbf{44.7} & \textbf{85.7} & \textbf{58.7} & \textbf{41.9} & \textbf{81.0} & \textbf{55.3} \\\hline
% % \tabincell{c}{Transformer-based\\encoding } & 29.0 & 68.5 & 40.8 & 44.6 & 82.1 & 57.8 & 38.7 & 66.7 & 49.0  \\\hline 

% % \end{tabular}
% % \label{tab:alter}
% % \end{table*}




% % the method-level prediction. The highest precision, recall and F1 for each bug type is highlighted in bold. In general, \tool is better than AST method and CFG method in most metrics, particularly, \tool is far more accurate in dealing with null pointer dereference and array index out of bound bugs (\ie by more than 10\% in F1 score). Furthermore, we find out \tool beats the two baselines by even bigger margin in F1 score on the top 10\% largest graphs (\ie 73.5\% by \tool vs. 29.3\% by CFG vs. 38.9\% by AST ), indicating the interval-based propagation model indeed improves the scalability of GGNN for generalizing on larger graphs. Figure~\ref{fig:largeGraph} shows how the F1 score changes for each methodology across the graph size. 

% %For example, for array index out of bound bug, the F1 score is 58.7\%, while the F1 is 43.2\% with the first baseline of AST-based representation, and the F1 is 39.5\% with the CFG method.

% % Figure~\ref{fig:perCmp} shows a bar graph charting the average performance across all bug types among the three methodologies. On average, \tool achieves 52.2\% in F1 score, while the AST and CFG method achieve 42.0\% and 40.8\% respectively. In terms of the average recall, \tool achieves 79.6\% while AST and CFG achieve 60.2\% and 62.3\% respectively. Our results demonstrate at the method-level prediction, \tool outperforms the baselines in both recall and F1 significantly.


% %\ke{Yu this sentence is not clear to me: The results demonstrate that \tool on average outperforms the baselines by 20.8\% in F1 score and 29.9\% in recall among the 12 projects.} \wyc{WY: it means that \tool is 20.8\% better than AST and CFG method in F1 score and 29.9\% better than the two method in recall. The formula is $20.8\%=((F1_{\tool}-F1_{AST})/F1_{\tool} + (F1_{\tool}-F1_{CFG})/F1_{\tool})/2$}
   

% \begin{table*}
% \begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{Precision in predicting NPE.}
% \centering
% \adjustbox{max width=1\textwidth}{
% \begin{tabular}{c|c|c|c}
% \hline
%  \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
% Baseline (0) & 0.209 & 0.147 & 0.117 \\\hline
% Baseline (1) & \textit{0.285} & 0.166 & 0.131 \\\hline
% Baseline (2) & 0.218 & 0.138 & 0.101 \\\hline
% \tool (0) & 0.326 & 0.174 & 0.138 \\\hline
% \tool (1) & \textbf{0.351} & 0.167 & 0.130 \\\hline
% \tool (2) & 0.305 & 0.164 & 0.136 \\\hline
% \hline
% Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.351} - \textit{0.285} = 0.066} \\\hline
% \end{tabular}}
% \label{tab:preNPE}
% \end{minipage}
% \begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{Recall in predicting NPE.}
% \centering
% \adjustbox{max width=1\textwidth}{
% \begin{tabular}{c|c|c|c}
% \hline
%  \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
% Baseline (0) & 0.243 & 0.373 & \textit{0.450} \\\hline
% Baseline (1) & 0.171 & 0.252 & 0.302 \\\hline
% Baseline (2) & 0.210 & 0.337 & 0.375 \\\hline
% \tool (0) & 0.282 & 0.374 & 0.447 \\\hline
% \tool (1) & 0.329 & 0.431 & \textbf{0.507} \\\hline
% \tool (2) & 0.304 & 0.402 & 0.500 \\\hline
% \hline
% Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.507} - \textit{0.450} = 0.057} \\\hline
% \end{tabular}}
% \label{tab:reNPE}
% \end{minipage}
% \begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{F1 score in predicting NPE.}
% \centering
% \adjustbox{max width=1\textwidth}{
% \begin{tabular}{c|c|c|c}
% \hline
%  \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
% Baseline (0) & \textit{0.224} & 0.211 & 0.186 \\\hline
% Baseline (1) & 0.214 & 0.201 & 0.183 \\\hline
% Baseline (2) & 0.214 & 0.196 & 0.159 \\\hline
% \tool (0) & 0.303 & 0.238 & 0.211 \\\hline
% \tool (1) & \textbf{0.339} & 0.241 & 0.207 \\\hline
% \tool (2) & 0.304 & 0.233 & 0.214 \\\hline
% \hline
% Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.339} - \textit{0.224} = 0.115} \\\hline
% \end{tabular}}
% \label{tab:f1NPE}
% \end{minipage}

% \par\bigskip

% \begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{Precision in predicting AIE.}
% \centering
% \adjustbox{max width=1\textwidth}{
% \begin{tabular}{c|c|c|c}
% \hline
%  \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
% Baseline (0) & \textit{0.286} & 0.124 & 0.106 \\\hline
% Baseline (1) & 0.218 & 0.112 & 0.095 \\\hline
% Baseline (2) & 0.215 & 0.134 & 0.088 \\\hline
% \tool (0) & 0.269 & 0.159 & 0.113 \\\hline
% \tool (1) & 0.308 & 0.134 & 0.097 \\\hline
% \tool (2) & \textbf{0.362} & 0.131 & 0.110 \\\hline
% \hline
% Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.362} - \textit{0.286} = 0.076} \\\hline
% \end{tabular}}
% \label{tab:preAI}
% \end{minipage}\hfill
% \begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{Recall in predicting AIE}
% \centering
% \adjustbox{max width=1\textwidth}{
% \begin{tabular}{c|c|c|c}
% \hline
%  \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
% Baseline (0) & 0.231 & 0.266 & \textit{0.355} \\\hline
% Baseline (1) & 0.165 & 0.225 & 0.300 \\\hline
% Baseline (2) & 0.180 & 0.288 & 0.306 \\\hline
% \tool (0) & 0.284 & 0.425 & 0.470 \\\hline
% \tool (1) & 0.291 & 0.358 & 0.403 \\\hline
% \tool (2) & 0.333 & 0.378 & \textbf{0.489} \\\hline
% \hline
% Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.489} - \textit{0.355} = 0.134} \\\hline
% \end{tabular}}
% \label{tab:reAI}
% \end{minipage}\hfill
% \begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{F1 score in predicting AIE.}
% \centering
% \adjustbox{max width=1\textwidth}{
% \begin{tabular}{c|c|c|c}
% \hline
%  \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
% Baseline (0) & \textit{0.256} & 0.169 & 0.163 \\\hline
% Baseline (1) & 0.188 & 0.149 & 0.145 \\\hline
% Baseline (2) & 0.196 & 0.183 & 0.136 \\\hline
% \tool (0) & 0.276 & 0.232 & 0.182 \\\hline
% \tool (1) & 0.299 & 0.195 & 0.157 \\\hline
% \tool (2) & \textbf{0.347} & 0.195 & 0.179 \\\hline
% \hline
% Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.347} - \textit{0.256} = 0.091} \\\hline
% \end{tabular}}
% \label{tab:f1AI}
% \end{minipage}\hfill

% \par\bigskip

% \begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{Precision in predicting CCE.}
% \centering
% \adjustbox{max width=1\textwidth}{
% \begin{tabular}{c|c|c|c}
% \hline
%  \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
% Baseline (0) & 0.345 & 0.165 & 0.169 \\\hline
% Baseline (1) & 0.328 & 0.180 & 0.135 \\\hline
% Baseline (2) & \textit{0.352} & 0.198 & 0.173 \\\hline
% \tool (0) & 0.362 & 0.220 & 0.170 \\\hline
% \tool (1) & \textbf{0.438} & 0.244 & 0.199 \\\hline
% \tool (2) & \textbf{0.438} & 0.252 & 0.193 \\\hline
% \hline
% Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.438} - \textit{0.387} = 0.051} \\\hline
% \end{tabular}}
% \label{tab:preCC}
% \end{minipage}\hfill
% \begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{Recall in predicting CCE.}
% \centering
% \adjustbox{max width=1\textwidth}{
% \begin{tabular}{c|c|c|c}
% \hline
%  \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
% Baseline (0) & 0.270 & 0.319 & 0.467 \\\hline
% Baseline (1) & 0.319 & 0.369 & 0.393 \\\hline
% Baseline (2) & 0.291 & 0.371 & \textit{0.503} \\\hline
% \tool (0) & 0.286 & 0.443 & 0.495 \\\hline
% \tool (1) & 0.292 & 0.413 & 0.486 \\\hline
% \tool (2) & 0.384 & 0.561 & \textbf{0.620} \\\hline
% \hline
% Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.620} - \textit{0.503} = 0.117} \\\hline
% \end{tabular}}
% \label{tab:reCC}
% \end{minipage}\hfill
% \begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{F1 score in predicting CCE.}
% \centering
% \adjustbox{max width=1\textwidth}{
% \begin{tabular}{c|c|c|c}
% \hline
%  \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
% Baseline (0) & 0.303 & 0.217 & 0.249 \\\hline
% Baseline (1) & \textit{0.323} & 0.242 & 0.201 \\\hline
% Baseline (2) & 0.319 & 0.258 & 0.257 \\\hline
% \tool (0) & 0.320 & 0.294 & 0.254 \\\hline
% \tool (1) & 0.350 & 0.307 & 0.282 \\\hline
% \tool (2) & \textbf{0.409} & 0.348 & 0.295 \\\hline
% \hline
% Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.409} - \textit{0.323} = 0.086} \\\hline
% \end{tabular}}
% \label{tab:f1CC}
% \end{minipage}\hfill
% \end{table*}

% \ignore{
% \begin{table*}
% \begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{Precision in predicting all bugs.}
% \centering
% \adjustbox{max width=1\textwidth}{
% \begin{tabular}{c|c|c|c}
% \hline
%  \tabincell{c}{\#Interval} & Top-1 & Top-3 & Top-5  \\\hline
% 1-2 & 51.1/40.2 & 29.7/23.2 & 24.0/18.1 \\\hline
% 3-4 & 10.0/23.1 & 8.9/12.3 & 8.7/9.2 \\\hline
% 5-6 & 4.3/0.0 & 2.9/6.0 & 1.7/4.8 \\\hline
% >6 & 8.3/0.0 & 2.8/0.0 & 3.3/0.7 \\\hline
% \end{tabular}}
% \label{tab:cfgpre}
% \end{minipage}
% \begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{Recall in predicting all bugs.}
% \centering
% \adjustbox{max width=1\textwidth}{
% \begin{tabular}{c|c|c|c}
% \hline
%  \tabincell{c}{\#Interval} & Top-1 & Top-3 & Top-5  \\\hline
% 1-2 & 30.2/37.1 & 40.4/49.9 & 46.7/55.9 \\\hline
% 3-4 & 9.7/21.4 & 25.8/34.3 & 41.9/42.9 \\\hline
% 5-6 & 4.5/0.0 & 9.1/26.0 & 9.1/34.6 \\\hline
% >6 & 8.3/0.0 & 8.3/0.0 & 16.7/3.3 \\\hline
% \end{tabular}}
% \label{tab:cfgre}
% \end{minipage}
% \begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{F1 score in predicting all bugs.}
% \centering
% \adjustbox{max width=1\textwidth}{
% \begin{tabular}{c|c|c|c}
% \hline
%  \tabincell{c}{\#Interval} & Top-1 & Top-3 & Top-5  \\\hline
% 1-2 & 37.9/38.6 & 34.2/31.7 & 31.7/27.4 \\\hline
% 3-4 & 9.8/22.2 & 13.2/18.1 & 14.4/15.2 \\\hline
% 5-6 & 4.4/NA & 4.4/9.7 & 2.9/8.4 \\\hline
% >6 & 8.3/NA & 4.2/NA & 5.6/1.1 \\\hline
% \end{tabular}}
% \label{tab:cfgf1}
% \end{minipage}

% \par\bigskip

% \end{table*}
% }


% \subsection{Performance Measurement}
% We build two sets of neural bug detectors based on \tool and the baseline. Each set includes three models, each of which deals with null pointer dereference, array index out of bound and class casting bugs respectively. 

% \paragraph{Evaluating models using proposal metrics} Table~\ref{tab:preNPE}--\ref{tab:f1CC} depicts the precision, recall, and F1 for all neural bug detectors. We set out to examine the impact of the depth of inlining on the performance of each bug detector. In particular, each row in a table shows the result of a neural bug detector that is trained either using the baseline model or \tool. The number in parenthesis is the depth of inlining. Specifically, 0 means no inlining, 1 inlines all methods that are invoking or invoked by the target methods, and 2 further inlines all callers and callees of each method that is inlined by 1. Exceeding the depth of 2 has costly consequences. First, most data points will have to be filtered out for overflowing the GPU memory. Moreover, a significant portion of the remaining ones would also have to be placed in a batch on its own, resulted in a dramatic increase in training time. Methods in the test set are inlined as deep as those in the training set to maintain a consistent distribution across the entire dataset. We also make certain each buggy method is only inlined once to prevent a potential date duplicate issue. Columns in each table correspond to three prediction modes in which \tool picks 1, 3 or 5 statements to be buggy after a method is predicted to be buggy.

% Overall, \tool consistently outperforms the baseline across all bug types using all proposed metrics. In particular, \tool beats the baseline by around 10\% across all bugs types in F1 score. 
% % For null pointer dereference, \tool achieves far better results in all three metrics across all prediction configurations. For array index out of bound and class cast exceptions, \tool is still considerably better than the baseline despite performing marginally worse on occasion. 
% Regarding the impact of the depth of inlining, we find that increasing the depth mostly but not always leads to improved performance of either \tool or the baseline. The reason is, on one hand, models will benefit from a more complete program representation thanks to the inlining. On the other hand, exceedingly large graphs hinders the generalization of GNN, resulted in degraded performance of the neural bug detectors. 

% % \begin{table*}[!t]
% % \centering
% % \small
% % \caption{Method-level prediction results.}
% % \begin{tabular}{c|ccc|ccc|ccc}
% % \hline
% %  \multirow{2}{*}{\tabincell{c}{Methods}} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{AIOE} & \multicolumn{3}{c}{CCE} \\
% % \cline{2-10}
% % & Precision & Recall & F1 & Precision & Recall & F1  & Precision & Recall & F1  \\\hline
% % AST & 24.0 & 52.3 & 32.3 & 34.8 & 57.1 & 43.2 & 38.3 & 71.4 & 49.8  \\\hline
% % CFG & 24.2 & 55.9 & 33.8 & 28.5 & 64.3 & 39.5 & 38.7 & 66.7 & 49.0  \\\hline
% % \hline
% % \tool & \textbf{30.3} & \textbf{72.1} & \textbf{42.6} & \textbf{44.7} & \textbf{85.7} & \textbf{58.7} & \textbf{41.9} & \textbf{81.0} & \textbf{55.3} \\\hline

% % \end{tabular}
% % \label{tab:metRes}
% % \end{table*}



% % \begin{figure}
% % \centering
% % \begin{minipage}{.45\textwidth}
% %   \centering
% %   \includegraphics[width=.95\linewidth]{Figures/perCmp.pdf}
% %   \captionof{figure}{Average precision, recall and F1 for method-level prediction.}
% %   \label{fig:perCmp}
% % \end{minipage}\hfill
% % \begin{minipage}{.45\textwidth}
% %   \centering
% %   \includegraphics[width=.95\linewidth]{Figures/largeGraph.png}
% %   \captionof{figure}{F1 score of each methodology in top N\% largest graphs.}
% %   \label{fig:largeGraph}
% % \end{minipage}
% % \end{figure}



% % \begin{table}

% % 	\begin{minipage}{.55\textwidth}
% % 		\caption{Top-N recall for line-level prediction.}
% % 		\centering
% % 		\adjustbox{max width=1\textwidth}{

% % 		\begin{tabular}{c|c|c|c|c|c}
% % \hline
% %  \tabincell{c}{Methods} & Top-N & NPE & AIOE & CCE & Avg. \\\hline
% % \multirow{5}{*}{AST} & Top-1 & 37.8 & 28.6 & \textbf{66.7} & \textbf{44.4} \\\cline{2-6}
% % & Top-3 & 55.0 & 35.7 & 66.7 & 52.5 \\\cline{2-6}
% % & Top-5 & 64.0 & 39.3 & \textbf{81.0} & 61.4 \\\cline{2-6}
% % & Top-7 & 72.1 & 42.9 & \textbf{85.7} & 66.9 \\\cline{2-6}
% % & Top-10 & 80.2 & 64.3 & \textbf{95.2} & 79.9 \\\hline
% % \multirow{5}{*}{CFG} & Top-1 & \textbf{47.7} & 32.1 & 52.4 & 44.1 \\\cline{2-6}
% % & Top-3 & 55.9 & 46.4 & 66.7 & 56.3\\\cline{2-6}
% % & Top-5 & 61.3 & 46.4 & 76.2 & 61.3 \\\cline{2-6}
% % & Top-7 & 67.6 & 57.1 & 76.2 & 67.0 \\\cline{2-6}
% % & Top-10 & 79.3 & 64.3 & \textbf{95.2} & 79.6 \\\hline
% % \hline
% % \multirow{5}{*}{\tool} & Top-1 & 44.1 & \textbf{35.7} & 47.6 & 42.5 \\\cline{2-6}
% % & Top-3 & \textbf{57.7} & \textbf{50.0} & \textbf{71.4} & \textbf{59.7} \\\cline{2-6}
% % & Top-5 & \textbf{67.6} & \textbf{71.4} & \textbf{81.0} & \textbf{73.3} \\\cline{2-6}
% % & Top-7 & \textbf{73.0} & \textbf{75.0} & 81.0 & \textbf{76.3} \\\cline{2-6}
% % & Top-10 & \textbf{82.0} & \textbf{75.0} & \textbf{95.2} & \textbf{84.1} \\\hline
% % \end{tabular}}
% % \label{tab:lineres}
% % 	\end{minipage}\hfill
% % 		\begin{minipage}{.43\textwidth}
% % 		\centering
% % 		\includegraphics[width=1\linewidth ]{Figures/largeGraphLine.png}
% % 		\captionof{figure}{Top-3 recall in top N\% largest graphs at line-level prediction.}
% %         \label{fig:largeGraphLine}
% % 	\end{minipage}
% % \end{table}

% % \ke{line-level below}
% % To completely separate the line-level prediction with the method-level 
% % prediction, we train all neural bug detectors from buggy methods only. In other words, the job of line-level predictors is to locate the bugs in a known buggy method. 
% %To evaluate the line-level performance, we only keep buggy methods for training and testing.
% %Therefore, all data for training and testing are buggy methods with analyzed buggy lines.
% %In this way, we can have a more clear performance without affected by method-level prediction results.
% % Table \ref{tab:lineres} presents the top-N recall of the line-level prediction results. We choose N to be 1, 3, 5, 7, and 10 for 
% % multiple prediction configurations. As before, we highlight the highest top-N recall for each methodology across all bug types. Overall, \tool outperforms the baslines in most metrics. Specifically, for array index out of bound bugs, \tool yields significantly better models than AST and CFG methods in each top-N configuration. However, the improvement \tool made over the baselines is not as significant as that in method-level prediction, especially in dealing with class cast bugs where AST method outperforms \tool in certain configurations. The last column shows average top-N recall performance among all three bug types. \tool achieves almost 60\% in top-3 and more than 70\% in top-5 recall, which is still notably better than the two other methodologies. Figure~\ref{fig:largeGraphLine} depicts the top-3 recall across the graph size. Similar to the method-level prediction, \tool shows bigger improvement over the baselines on the top 10\% largest graphs. 

% % \ignore{
% % As the results show, \tool is over-perform than AST method and CFG method in many cases.
% % For example, for all the three metrics in array index out of bound bugs, \tool beats the two baselines with overwhelming performance.
% % The average improvement in the top-N accuracy is 30.1\% and 18.0\% for AST method and CFG method when predicting the array index out of bound bug. 
% % However, the performance of \tool in line-level prediction is not as good as method-level prediction results.
% % AST method is beatable in some cases, such as predicting CCE bugs.
% % %The performance is better for AST method.
% % The last column shows average performance among the three kinds of bugs.
% % The overall performance shows that \tool is better than the two baselines with around 8.3\% improvement.


% % \textit{Top-N} in the second column represents that we regard \textit{N} predictions as buggy. The N we choose is 1, 3, 5, 7, and 10.
% % A row with top-N means that precision, recall and F1 are evaluated when predicting \textit{N} lines as buggy and remaining lines as clean.
% % In this table, we highlight the highest precision, recall and F1 of the three methods.
% % We can see from the table that all metrics are the same in top-1. 
% % The reason is that if a method has $N$ statements, we only predict one statement as buggy.
% % If the prediction is wrong, then both FP and FN are increased by 1, which means that FP is the same as FN. 

% % As the results show, \tool is over-perform than AST method and CFG method in many cases.
% % For example, for all the three metrics in array index out of bound bugs, \tool beats the two baselines with overwhelming performance.
% % The average improvement in the top-N accuracy is 30.1\% and 18.0\% for AST method and CFG method when predicting the array index out of bound bug. 
% % However, the performance of \tool in line-level prediction is not as good as method-level prediction results.
% % AST method is beatable in some cases, such as predicting CCE bugs.
% % %The performance is better for AST method.
% % The last column shows average performance among the three kinds of bugs.
% % The overall performance shows that \tool is better than the two baselines with around 8.3\% improvement.}


% % \ignore{
% % From the method-level and line-level evaluation, we can find that \tool is over-perform than two baselines in method-level performance and \tool is comparable to AST method in line-level prediction.
% % Additionally, note that the line-level evaluation is only focus on buggy method, which means that the combination of method-level and line-level prediction of our method is better than the two baselines.
% % }

% % Through our extensive evaluations of \tool in both method- and line-level predictions, we conclude that \tool's neural bug detectors are more precise in capturing the semantic buggy patterns than the two other methodologies. Compared to the CFG method, the superior performance \tool displays is entirely due to the interval-based propagation model, which demonstrates a better generalization of GGNN. As for AST methods, \tool uses a more semantic and principle graph representation to facilitate GGNN for learning deeper and more complicated semantic features.

% \paragraph{Investigating models scalability}
% We divide the entire test set into ten subsets, each of which consists of graphs of similar size. We then investigate how models perform on each subset starting from the smallest to the largest graphs. We fix the depth of inlining to be 2, which provides the largest variation among all graphs in terms of the size. Figure~\ref{fig:scaf} depicts the F1 score for \tool and the baseline under top-3 prediction mode (top-1 and top-5 yield similar results which we left to the supplemental material). Initially, \tool achieves slightly better results on the subset of small graphs; later as the size of graphs increases, \tool is significantly more resilient with its prediction than the baseline. Overall, we conclude bug detectors built out of \tool are more scalable.

% \begin{figure*}
% \begin{minipage}{.33\textwidth}
% % \captionsetup{skip=1pt}
% % \caption{Precision in predicting NPE.}
% \centering
% \begin{tikzpicture}[scale=0.92]
%   \begin{axis}[
%     xmax=10,xmin=1,
%     ymin=0,ymax=0.7,
%     xlabel=\emph{N-th Set (Ranked by Size of Graphs)},ylabel=\emph{Top-3 F1 Score},
%     xtick={1,2,...,10},
%     ytick={0,0.1,0.20,...,0.7},
%     xticklabels={1,2,...,10},
%     % xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}\%},
%     ]
%      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(1, 0.481) (2, 0.385) (3, 0.288) (4, 0.256) (5, 0.236) (6, 0.163) (7, 0.156) (8, 0.127) (9, 0.070) (10, 0.027)};
%      \addplot coordinates{(1, 0.488) (2, 0.376) (3, 0.350) (4, 0.309) (5, 0.303) (6, 0.266) (7, 0.275) (8, 0.244) (9, 0.149) (10, 0.073)};   
%     \legend{\emph{Baseline},\emph{\tool}}
%     \end{axis}
%     \end{tikzpicture}
%      ~%
%     % %
%     \subcaption{}
% \label{fig:scaf}
% \end{minipage}
% \begin{minipage}{.33\textwidth}
% % \captionsetup{skip=1pt}
% % \caption{F1 score in predicting NPE.}
% \centering
% \begin{tikzpicture}[scale=0.92]
%   \begin{axis}[
%     xmax=120,xmin=0,
%       ymin=0,ymax=0.4,
%     xlabel=\emph{Training Time (Minutes)},ylabel=\emph{Average Test F1 for NPE},
%     % xtick={0,4,8,...,20},
%     xtick={0,30,60,90,120},
%     ytick={0,0.1,0.20,...,0.4},
%     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}},
%   ]
   
%     %  \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(0, 0.177) (7.5, 0.171) (15, 0.165) (22.5, 0.165) (30, 0.165) (37.5, 0.141) (45, 0.193) (52.5, 0.168) (60, 0.174) (67.5, 0.168) (75, 0.153) (82.5, 0.193) (90, 0.186) (97.5, 0.180) (105, 0.156) (112.5, 0.186) (120, 0.165) (127.5, 0.162) (135, 0.199) (142.5, 0.165) (150, 0.171)};
%     %  \addplot coordinates{(0, 0.245) (7.5, 0.253) (15, 0.270) (22.5, 0.291) (30, 0.304) (37.5, 0.279) (45, 0.287) (52.5, 0.300) (60, 0.291) (67.5, 0.291) (75, 0.283) (82.5, 0.274) (90, 0.296) (97.5, 0.274) (105, 0.287) (112.5, 0.287) (120, 0.287) (127.5, 0.287) (135, 0.291) (142.5, 0.287) (150, 0.283)};
%      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(0, 0.1)  (15, 0.123)  (30, 0.129) (45, 0.137)  (60, 0.169)  (75, 0.167)  (90, 0.174)  (105, 0.19)  (120, 0.191)  (135, 0.239)  (150, 0.24)};
%      \addplot coordinates{(0, 0.117)  (15, 0.185)  (30, 0.204)  (45, 0.232) (60, 0.252)  (75, 0.255)  (90, 0.255)  (105, 0.256)  (120, 0.255) (135, 0.412) (150, 0.41)};
%      \legend{\emph{Baseline}, \emph{\tool}}
%     \end{axis}
%     \end{tikzpicture}%
%     ~%
% \subcaption{}
% \label{fig:ttf}
% \end{minipage}
% \begin{minipage}{.33\textwidth}
% \vspace{4pt}
% % \captionsetup{skip=1pt}
% % \caption{Recall in predicting NPE.}
% \centering
% \begin{tikzpicture}[scale=0.92]
%   \begin{axis}[
%   % x tick label style={/pgf/number format/1000 sep=},
%     ymin=0,ymax=0.7,
%     xlabel=\emph{Number of First Order Intervals}, ylabel=\emph{Top-3 F1 Score},
%     xtick=data,
%     xticklabels={1,2,...,6,7+},
%     ybar,
%     bar width=6pt,
%     xtick pos=lower,ytick pos=left,
%     xtick style={draw=none},
%     xticklabel style={yshift=.75ex},
%     legend image code/.code={
%         \draw [#1] (0cm,-0.1cm) rectangle (0.2cm,0.25cm); },
%   ]

%   \addplot [black!30!white,fill=black!30!white] coordinates {
%   (1, 0.257) (2, 0.215) (3, 0.183) (4, 0.173) (5, 0.116) (6, 0.115) (7, 0.074)
%   };
%   \addplot [black!100!white,fill=black!100!white] coordinates {
%   (1, 0.352) (2, 0.288) (3, 0.259) (4, 0.291) (5, 0.102) (6, 0.159) (7, 0.107)
%   };
%   \legend{\emph{w/o IBPM},\emph{\tool}}
%   \end{axis}
% \end{tikzpicture}%
%     ~%
%     %
% \subcaption{}
% % \caption{ss}
% \label{fig:intf}
% \end{minipage}
% \caption{Experiment results.}
% \end{figure*}

% % \begin{figure*}
% % \centering
% %   \begin{tikzpicture}[scale=0.92]
% %   \begin{axis}[
% %     xmax=100,xmin=0,
% %       ymin=0,ymax=0.7,
% %     xlabel=\emph{Graph Size},ylabel=\emph{Top-1 F1 Score},
% %     xtick={0,20,40,...,100},
% %     ytick={0,0.1,0.20,...,0.7},
% %     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}\%},
% %   ]
   
% %      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(5, 0.547) (15, 0.435) (25, 0.209) (35, 0.281) (45, 0.294) (55, 0.209) (65, 0.175) (75, 0.194) (85, 0.080) (95, 0.035)};
% %      \addplot coordinates{(5, 0.443) (15, 0.357) (25, 0.285) (35, 0.459) (45, 0.487) (55, 0.353) (65, 0.297) (75, 0.416) (85, 0.201) (95, 0.112)};    
% %      \legend{\emph{Baseline}, \emph{\tool}}
% %     \end{axis}
% %     \end{tikzpicture}%
% %     ~%
% %     %
% %     \begin{tikzpicture}[scale=0.92]
% %   \begin{axis}[
% %     xmax=100,xmin=0,
% %     ymin=0,ymax=0.7,
% %     xlabel=\emph{Graph Size},ylabel=\emph{Top-3 F1 Score},
% %     xtick={0,20,40,...,100},
% %     ytick={0,0.1,0.20,...,0.7},
% %     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}\%},
% %     ]
% %      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(5, 0.481) (15, 0.385) (25, 0.288) (35, 0.256) (45, 0.256) (55, 0.163) (65, 0.156) (75, 0.127) (85, 0.070) (95, 0.027)};
% %      \addplot coordinates{(5, 0.388) (15, 0.294) (25, 0.350) (35, 0.309) (45, 0.303) (55, 0.266) (65, 0.275) (75, 0.244) (85, 0.149) (95, 0.073)};   
% %     \legend{\emph{Baseline},\emph{\tool}}
% %     \end{axis}
% %     \end{tikzpicture}%
% %     ~%
% %     %
% %      \begin{tikzpicture}[scale=0.92]
% %   \begin{axis}[
% %     xmax=100,xmin=0,
% %     ymin=0,ymax=0.7,
% %     xlabel=\emph{Graph Size},ylabel=\emph{Top-5 F1 Score},
% %     xtick={0,20,40,...,100},
% %     ytick={0,0.1,0.20,...,0.70},
% %     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}\%},
% %     ]
    
% %      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(5, 0.440) (15, 0.328) (25, 0.249) (35, 0.225) (45, 0.241) (55, 0.121) (65, 0.135) (75, 0.106) (85, 0.060) (95, 0.030)};
% %      \addplot coordinates{(5, 0.343) (15, 0.280) (25, 0.337) (35, 0.304) (45, 0.302) (55, 0.228) (65, 0.202) (75, 0.207) (85, 0.115) (95, 0.069)};   
% %      \legend{\emph{Baseline},\emph{\tool}}
% %      \end{axis} 
% %      \end{tikzpicture}
% %     \caption{Investigating the scalability of all models.}
% %     \label{fig:sca}
% % \end{figure*}

% \paragraph{Measuring training efficiency}
% Since all models make instantaneous predictions (\eg around 800 examples per second), we only measure the training speed of \tool and the baseline. Again, we fix the depth of inlining to be 2, which presents the biggest challenges in training efficiency. Figure~\ref{fig:ttf} shows the \textit{test} F1 score (average across top-1, 3 and 5 prediction modes) over training time for \tool and the baseline on null pointer dereference bugs (Other two bug types are much easier to train, and we left their results in the supplemental material). \tool's bug detector achieves results that are as 50\% as good as its final results under half an hour, and results that are as 95\% as good under 1 hour, while both being substantially higher than the best results of the baseline models. Our model achieves its best results around the 1 hour mark.



% % Table \ref{tab:lineres} presents the top-N recall of the line-level prediction results. We choose N to be 1, 3, 5, 7, and 10 for 
% % multiple prediction configurations. As before, we highlight the highest top-N recall for each methodology across all bug types. Overall, \tool outperforms the baslines in most metrics. Specifically, for array index out of bound bugs, \tool yields significantly better models than AST and CFG methods in each top-N configuration. However, the improvement \tool made over the baselines is not as significant as that in method-level prediction, especially in dealing with class cast bugs where AST method outperforms \tool in certain configurations. The last column shows average top-N recall performance among all three bug types. \tool achieves almost 60\% in top-3 and more than 70\% in top-5 recall, which is still notably better than the two other methodologies. Figure~\ref{fig:largeGraphLine} depicts the top-3 recall across the graph size. Similar to the method-level prediction, \tool shows bigger improvement over the baselines on the top 10\% largest graphs. 

% % \begin{table}[!t]
% % \centering
% % \normalsize
% % \caption{Training time.}
% % \adjustbox{max width=\columnwidth}{\begin{tabular}{c|ccc|ccc|ccc}
% % \hline
% %  \multirow{2}{*}{\tabincell{c}{Method//\#Inline}} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{AIOE} & \multicolumn{3}{c}{CCE}\\
% % \cline{2-10}
% %         & 0 & 1 & 2 & 0 & 1 & 2& 0 & 1 & 2  \\\hline
% % Baseline & 4 &	11.3 & 	37.8 & 0.9 &	1.9 &	6.4 & 0.7 &	1.9 &	7.5   \\\hline
% % CFG & 0.9 &	1.4 &	12 &  0.2 &	0.4 &	2.2 & 0.2 &	0.3 &	2.1   \\\hline
% % \hline
% % \tool & 20.7 &	39.3 &	51.7 & 4.5 &	8.1 &	10.2 & 4.3 &	7.8 &	9.4  \\\hline % FP should *3?

% % \end{tabular}}
% % \label{tab:sats}
% % \end{table}

% \subsection{Contribution of IBPM}
% We aim to precisely quantify IBPM's contribution to the learning capacity of the GNN. In particular, we re-implement \tool by replacing its IBPM with the standard propagation mechanism. In other words, we perform a head-to-head comparison between the two propagation mechanisms while the rest of the model architecture is held the same. Figure~\ref{fig:intf} shows how the test F1 scores of both configurations vary with the number of first order intervals in top-3 prediction mode (top-1 and top-5 yield similar results which we left to the supplemental material). For the same reason, the depth of inlining is fixed to be 2. Given the same number of the first order intervals, IBPM performs better than the standard propagation mechanism across the board. Apart from the apparent scalability advantage IBPM displays over the standard propagation mechanism, IBPM achieves better results even when the number of intervals is small, thanks to its exploitation of the program-specific graph characteristics.  



% \subsection{Further Evaluation of \tool}
% In general, static analyzers can be classified into two categories: soundy and unsound. The former refers to tools that are sound by design but make unsound choices for utility concerns, whereas the latter is often built out of pattern matching techniques that do not concern themselves with soundness. Intending to cover both flavors, we pick soundy tools: 
% Facebook Infer~\cite{calcagno2015moving,berdine2005smallfoot}, Pinpoint~\cite{shi2018pinpoint} and BugPicker, and another unsound tool: SpotBugs (the successor of FindBugs~\cite{Hovemeyer2004}).

% We emphasize that our work makes no claims of advancing the theory of sound static analysis, therefore this experiment solely focuses on studying the utility of each tool in practice. 
% We examine the performance of each checker in catching null pointer dereference bugs, which happen to be the only type of bugs all tools support.


% % This section compares \tool against traditional 
% % static analyzers. As a conceptual advantage, we re-emphasize 
% % that creating neural bug finders based on \tool does not require the substantial amount of human-expertise that is needed to build 
% % classical static analyzers. Sufficient amount of training data is 
% % all \tool needs. Besides, \tool also allows an easier extension to 
% % support new types of bugs compared to static analyzers. 

% % To compare the actual performance between \tool and static 
% % analyzers in catching real world, complex and semantic bugs, 
% % we pick Facebook Infer~\cite{calcagno2015moving}, arguably the state-of-the-art static analyzer supporting Java program language. 

% % We compare \tool against and Infer in catching null pointer dereference bugs, which happen to be the only type of bugs both \tool and Infer support.

% % Ideally, we would like to use all bugs in our test set for the experiment, however, doing so would require a substantial amount of manual work. As for each bug in the test set, we need to pull from the repository the right version of the source code at which the bug has a presence, and subsequently analyze the report produced by each static analysis tool. 

% To keep the engineering load manageable, we randomly pick 75 bugs out of seven projects from defect4j and bugs.jar, two most studied datasets in bug detection literature. Later we discover Infer does not have access to the build tools that are required to compile some of the projects in defect4j. Therefore, we show Infer's performance only on the projects it can compile. Those projects contain 58 bugs in total, namely Bug Set I.

% First, we manually verify the validity, and more importantly, the location for all 75 bugs in case any bug may trigger an exception at a different location than developers' fix. Next, we feed the entire codebase of each project for each checker to scan. A report that points to a buggy location will be counted as a true positive, otherwise, it's a false positive. We acknowledge that a static analysis tool could have caught a real bug that is mistakenly counted as a false positive since it falls out of the 75 bugs we collected, however, the exact same issue applies to \tool, which we regrettably ignore due to resource constraint. We use \tool with depth 2 of inlining trained in the previous experiment. It is configured to run the top-1 prediction mode. We choose the most precise analysis for Pinpoint to perform. We also manually fine-tune BugPicker (\eg increase the length of the call chain or reset the timeout), but obtain the same results. We do not manage to run any other configuration for Infer and SpotBugs rather than their default set up. 

% Table~\ref{tab:sats} depicts the results (a more detailed comparison is provided in the supplemental material). 
% Overall, we find (1) \tool achieves better precision and recall than any other evaluated tool; more importantly, (2) bugs that are found by competing tools are all caught by \tool. Besides, \tool detects another 11 bugs that are missed by the other tools.

% % shows the performance of each bug finder\footnote{We also provide the details of the comparison in the supplemental material.}, and we interpret and analyze the results below.


% % nitially, we collected all null pointer dereference bugs from all of our testing projects.
% % Later we excluded the bugs from some of the projects that other tools do not manage to compile. For example, Infer does not have access to the build tools that are required to compile the projects in defect4j.
% % \footnote{Some projects require build tools such as those provided by defects4j that Infer does not have access to.} 
% % In the end we have 58 null pointer dereference bugs from Lang, Math, Flink, Closure, Wicket and Mockito, against which we show the performance of each bug finder in Table~\ref{tab:sats}. Below we interpret and analyze the results we obtain.

% % \begin{itemize}%[leftmargin=*]
% %     \item Each column records the number of detected bugs (denoted by TP), missed bugs (denoted by FN) and false warnings (denoted by FP) for each tool on the two bug sets. Overall, \tool achieves better precision and recall than any other evaluated tool.
% %     % (we provide a breakdown for the performance of each checker on each project in the supplemental material)
% %     % \item We have manually verified the validity, and more importantly the location for each of the 79 bugs to prevent any tool from being unfairly disadvantaged. For example, if a developer's fix does not exactly correlate to the program location where exceptions are thrown, we will manually add another buggy label to the location in addition to the point of fix registered by developers.
    
% %     \item We use \tool with depth 2 of inlining trained in the previous experiment. It is configured to run top-1 prediction mode. We choose the most precise analysis for Pinpoint to perform. We also manually fine tune BugPicker (\eg increase the length of call chain or reset the timeout), but obtain no improvement. We do not manage to run any other configuration for Infer and SpotBugs rather than their default set up.
    
% %     \item All bugs that are found by Infer and Pinpoint are also caught by \tool. In addition, \tool detects another 13 bugs that are missed by Infer and Pinpoint.
    
% %     % \item In general, we found that unsound tools (\eg SpotBugs and BugPicker) produce less warnings but miss more bugs than soundy tools (\eg Infer and Pinpoint). \tool produces comparable amount of warnings to unsound tools, and catches far more bugs than any evaluated tool. 
    
% % \end{itemize}

% \begin{table}[!t]
% \centering
% \normalsize
% \caption{Results of the comparison. TP, FP, FN stand for true positives, false positives and false negatives respectively.}
% \adjustbox{max width=\columnwidth}{\begin{tabular}{c|ccc|ccc|cc}
% \hline
%  \multirow{2}{*}{\tabincell{c}{Tools}} & \multicolumn{3}{c|}{Bug Set I} & \multicolumn{3}{c|}{Remaining Set} & \multicolumn{2}{c}{Total}\\
% \cline{2-9}
%          & TP & FP & FN & TP & FP & FN  & Precision & Recall   \\\hline
% FB Infer & 4 & 1004 & 54 & NA & NA & NA & .004 & .069    \\\hline
% Pinpoint & 4 & 1524 & 54 & 3 & 1104 & 14 & .003 & .093   \\\hline
% SpotBugs & 0 & 107 & 58 & 1 & 26 & 16 & .007 & .013   \\\hline
% BugPicker & 0 & 79 & 58 & 0 & 0 & 17 & 0 & 0   \\\hline
% \hline
% \textbf{\tool} & \textbf{16} & \textbf{1655} & \textbf{42} & \textbf{5} & \textbf{521} & \textbf{12} & \textbf{.010} & \textbf{.280}  \\\hline %top-1
% % \textbf{\tool} & \textbf{22} & \textbf{4414} & \textbf{33} & \textbf{8} & \textbf{1579} & \textbf{13} & \textbf{.005} & \textbf{.379}  \\\hline %top-3
% %\textbf{\tool} & \textbf{25} & \textbf{136} & \textbf{33} & \textbf{6} & \textbf{34} & \textbf{11} & \textbf{.154} & \textbf{.413}  \\\hline % FP should *3?

% \end{tabular}}
% \label{tab:sats}
% \end{table}

% % On those projects, Infer reports 1008 null pointer dereference bugs in total. After manually verifying the reports according to the ground truth, we confirm that Infer detects only one of them. In comparison, \tool is able to detect 42 buggy methods with 138 warnings. With the top-3 prediction mode at the line-level, \tool achieves 71.4\% recall, in other words, by scanning three lines in each buggy method, developers are able to precisely locate 30 out of the 58 bugs.

% % Worth noting we only validate Infer's report according to the existing bugs, it is possible that Infer detects potentially unknown bugs. In other words, there might have been true bugs contained in the 1008 warnings reported by Infer. However, since \tool and Infer use the same ground truth, it is equally possible that other bugs reported by \tool may also be true positives.

% % Apart from the practical benefits \tool yields, we believe \tool also enjoys several conceptual advantages over the competing static analysis tools. First, given the framework \tool provides, creating a static bug finder can be simplified to solving a machine learning task. In comparison, traditional way of designing static analysis tools even the unsound ones requires substantial amount of human expertise. Besides, unlike the static analysis tools, model-based bug detectors can benefit from increasingly large datasets and powerful training regime, as a result, they will evolve and get better over time.

% %The result shows that \tool is comparable to Infer in detecting NPE bugs.
% %However, building a new bug detector in \tool does require expertise on static analysis or verification.
% %Developers only need to collect data for the new bug and define a reasonable representation for it, which is easier than writing a program analysis tool.

% We have also applied \tool to catch bugs in the wild, and obtained encouraging results. Configured with top-1 prediction mode and inline depth of 2 (we also tried 3 and 4 for smaller methods), \tool found 50 bugs (40 NPE and 10 AIE) in 17 projects that are among the most starred on GitHub. All bugs are manually verified and reported to developers, out of which 9 (7 NPE and 2 AIE) are fixed and 3 (all NPE) are confirmed (fixes pending). We provide the links of bug reports in the supplemental material. Our findings show that not only does \tool significantly improve the prior works, but more importantly, \tool can be an industry-strength tool for checking real-world Java projects.

% % demonstrates its potential of being a highly-effective and useful static bug finder for real-world Java projects.

% \subsection{Discussion on Limitation of \tool}
% In order to gain a deeper understanding of \tool's limitation, we mainly look into the bugs \tool missed in the prior experiment. We find that when bug patterns are not local, that is, the dereference is quite distant from where a null pointer is assigned, \tool tends to struggle, in particular, it even misclassifies the method to be clean most of the time. The reason is, as one can imagine, \tool's signal gets diluted when a scattered bug pattern is overwhelmed by the irrelevant statements. We plan to tackle this issue with both program analysis and machine learning techniques. For data pre-processing, program slicing~\cite{Weiser1981} seems to be a promising idea. Given the location of a potential null pointer dereference (due to the null assignment or non-initialization), we can filter out statements that fall out of the slice to localize a bug pattern. On the other hand, a larger, more diverse dataset that contains a variety of bug patterns should also help. Alternatively, we can also synthesize new programs by randomly adding dummy statements in between the assignment and dereference of null pointers for buggy methods, especially when the high-quality, large-scale public datasets are unavailable.

% Another issue we discovered is \tool is less accurate when handling large programs (\ie approximately 1,000 nodes in the graph) despite the contribution IBPM makes to the underlying GNN. We find several bugs \tool missed where the bug patterns are in fact local. We believe this is due to the fundamental limitation of GNN, which requires deeper insight and understanding of the models themselves, without which, IBPM's results will be hard to improve upon in a qualitative manner.

% We also briefly examine the false positives \tool emitted. For a few dozen we inspected, we find that the same issue causing \tool to miss bugs are also major sources of \tool's imprecision. In addition, \tool can be over-sensitive about the presence of null pointers, albeit we can not confirm they are never dereferenced.


% % When applying \tool to catch bugs in the wild, we find \tool could have been a more useful bug-finding tool if it can provide justification to the developers as to why a particular code snippet is predicted to be buggy. We believe this issue can be promptly addressed by incorporating the ideas from a long line of works in the explainability of machine learning models~\cite{guidotti2019survey}. At the very least, \tool can highlight the regions of programs that have the most influence on its predictions, a technique researchers developed to explain why an image is predicted in a certain category.

% % To evaluate the performance of \tool in detecting unknown bugs, we apply \tool on open-source projects. 
% % For bugs reported by \tool, we manually verify them and report them to developers.
% % In total, we report 193 bugs, 13 of them are confirmed, 7 of them are fixed and remainings are waiting for confirmation. 
% % Specifically, we report 107 NPE bugs and 86 AIE bugs in 23 projects. 11 NPE bugs and 2 AIE bugs are confirmed. 5 NPE bugs are fixed and 2 AIE bugs are fixed.
% % It is worth noting that some bugs can be grouped into one according to their root cause. For example, a method that returns null may have multiple call sites, which use the null value. AIE bugs can also be grouped in the similar way.
% % The number of reported bugs is the number of bugs without group.


% % \ignore{

% % The section aims at evaluating the precision of infer by detecting known bugs.
% % We evaluated infer on 25 projects with 58 known NPE bugs from the dataset we used.
% % Infer reports 1008 null pointer dereference bugs.
% % After manually verifying the reports and comparing them with the known bugs, we found that infer detects 1 of them.
% % In comparison, \tool is able to detect NPE bugs with 72.1\% recall.
% % \wyc{\tool detects 24 bugs base on top-3 prediction, which reports 282 warnings methods in total.
% % If we use top-5 prediction, then we are able to pinpoint 28 bugs.
% % }


% % It is worth noting that we only validate bugs related to known bugs, there is a chance that Infer detects unknown bugs among the 1008 bug reports.
% % In other words, other bugs reported by Infer may also be true positives.
% % However, both two tools use the same ground truth, which means that other bugs reported by \tool may also be true positives.

% % The result shows that \tool is comparable to Infer in detecting NPE bugs.
% % However, building a new bug detector in \tool does require expertise on static analysis or verification.
% % Developers only need to collect data for the new bug and define a reasonable representation for it, which is easier than writing a program analysis tool.
% %}

% % \ignore{
% % \subsection{Performance on top N\% largest graphs}

% % \begin{table*}[!t]
% % \centering
% % \small
% % \caption{F1 score on top N\% largest graphs}
% % \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% % \hline
% %  Bug types & \multicolumn{4}{c|}{\tool} & \multicolumn{4}{c|}{CFG} & \multicolumn{4}{c|}{AST} \\
% % \cline{2-13}
% % & 20\% & 30\% & 40\% & 50\%  &20\% & 30\% & 40\% & 50\%  & 20\% & 30\% & 40\% & 50\% \\\hline
% % NPE & 724 &  721 & 775 & 769 & 744 &  789 & 729 & 729 &  667 & 636 & 627 & 694  \\\hline
% % \end{tabular}
% % \label{tab:lineres}
% % \end{table*}



% % \begin{table*}[!t]
% % \centering
% % \small
% % \caption{Performance on line-level prediction}
% % \begin{tabular}{c|c|ccc|ccc|ccc}
% % \hline
% %  \multirow{2}{*}{\tabincell{c}{Methods}} & \multirow{2}{*}{Top-N} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{AIOE} & \multicolumn{3}{c}{CCE} \\
% % \cline{3-11}
% % &  & Precision & Recall & F1 & Precision & Recall & F1  & Precision & Recall & F1  \\\hline
% % \multirow{5}{*}{AST} & Top-1 & 37.8 & 37.8 & 37.8 & 28.6 & 28.6 & 28.6 & \textbf{66.7} & \textbf{66.7} & \textbf{66.7} \\\cline{2- 11}
% % & Top-3 & \textbf{22.3} & 55.0 & \textbf{31.7} & 12.7 & 35.7 & 18.7 & \textbf{26.4} & 66.7 & \textbf{37.8} \\\cline{2- 11}
% % & Top-5 & \textbf{16.9} & 64.0 & \textbf{26.8} & 8.7 & 39.3 & 14.2 & \textbf{22.4} & \textbf{81.0} & \textbf{35.1} \\\cline{2- 11}
% % & Top-7 & \textbf{14.7} & 72.1 & \textbf{24.4} & 6.9 & 42.9 & 11.9 & \textbf{19.4} & \textbf{85.7} & \textbf{31.6} \\\cline{2- 11}
% % & Top-10 & \textbf{13.0} & 80.2 & \textbf{22.3} & 7.7 & 64.3 & 13.7 & \textbf{18.5} & \textbf{95.2} & \textbf{31.0} \\\hline
% % \multirow{5}{*}{CFG} & Top-1 & \textbf{47.7} & \textbf{47.7} & \textbf{47.7} & 32.1 & 32.1 & 32.1 & 52.4 & 52.4 & 52.4 \\\cline{2- 11}
% % & Top-3 & 18.6 & 55.9 & 27.9 & 15.5 & 46.4 & 23.2 & 22.2 & 66.7 & 33.3 \\\cline{2- 11}
% % & Top-5 & 13.7 & 61.3 & 22.4 & 9.6 & 46.4 & 16.0 & 16.8 & 76.2 & 27.6 \\\cline{2- 11}
% % & Top-7 & 11.7 & 67.6 & 19.9 & 8.7 & 57.1 & 15.2 & 13.6 & 76.2 & 23.0 \\\cline{2- 11}
% % & Top-10 & 10.7 & 79.3 & 18.8 & 7.2 & 64.3 & 12.9 & 14.1 & \textbf{95.2} & 24.5 \\\hline
% % \hline
% % \multirow{5}{*}{\tool} & Top-1 & 44.1 & 44.1 & 44.1 & \textbf{35.7} & \textbf{35.7} & \textbf{35.7} & 47.6 & 47.6 & 47.6 \\\cline{2- 11}
% % & Top-3 & 19.2 & \textbf{57.7} & 28.8 & \textbf{16.7} & \textbf{50.0} & \textbf{25.0} & 23.8 & \textbf{71.4} & 35.7 \\\cline{2- 11}
% % & Top-5 & 15.1 & \textbf{67.6} & 24.7 & \textbf{14.8} & \textbf{71.4} & \textbf{24.5} & 17.9 & \textbf{81.0} & 29.3 \\\cline{2- 11}
% % & Top-7 & 12.6 & \textbf{73.0} & 21.5 & \textbf{11.5} & \textbf{75.0} & \textbf{19.9} & 14.4 & 81.0 & 24.5 \\\cline{2- 11}
% % & Top-10 & 11.0 & \textbf{82.0} & 19.5 & \textbf{8.4} & \textbf{75.0} & \textbf{15.1} & 14.1 & \textbf{95.2} & 24.5 \\\hline
% % \end{tabular}
% % \label{tab:lineresold}
% % \end{table*}


% % \begin{table*}[!t]
% % \caption{Top-N recall for line-level prediction.}
% % \centering
% % \small
% % \begin{tabular}{c|c|c|c|c|c}
% % \hline
% %  \tabincell{c}{Methods} & Top-N & NPE & AIOE & CCE & Avg. \\\hline
% % \multirow{5}{*}{AST} & Top-1 & 37.8 & 28.6 & \textbf{66.7} & \textbf{44.4} \\\cline{2-6}
% % & Top-3 & 55.0 & 35.7 & 66.7 & 52.5 \\\cline{2-6}
% % & Top-5 & 64.0 & 39.3 & \textbf{81.0} & 61.4 \\\cline{2-6}
% % & Top-7 & 72.1 & 42.9 & \textbf{85.7} & 66.9 \\\cline{2-6}
% % & Top-10 & 80.2 & 64.3 & \textbf{95.2} & 79.9 \\\hline
% % \multirow{5}{*}{CFG} & Top-1 & \textbf{47.7} & 32.1 & 52.4 & 44.1 \\\cline{2-6}
% % & Top-3 & 55.9 & 46.4 & 66.7 & 56.3\\\cline{2-6}
% % & Top-5 & 61.3 & 46.4 & 76.2 & 61.3 \\\cline{2-6}
% % & Top-7 & 67.6 & 57.1 & 76.2 & 67.0 \\\cline{2-6}
% % & Top-10 & 79.3 & 64.3 & \textbf{95.2} & 79.6 \\\hline
% % \hline
% % \multirow{5}{*}{\tool} & Top-1 & 44.1 & \textbf{35.7} & 47.6 & 42.5 \\\cline{2-6}
% % & Top-3 & \textbf{57.7} & \textbf{50.0} & \textbf{71.4} & \textbf{59.7} \\\cline{2-6}
% % & Top-5 & \textbf{67.6} & \textbf{71.4} & \textbf{81.0} & \textbf{73.3} \\\cline{2-6}
% % & Top-7 & \textbf{73.0} & \textbf{75.0} & 81.0 & \textbf{76.3} \\\cline{2-6}
% % & Top-10 & \textbf{82.0} & \textbf{75.0} & \textbf{95.2} & \textbf{84.1} \\\hline
% % \end{tabular}
% % \label{tab:lineres}
% % \end{table*}



% % \begin{figure}
% % \centering
% % \begin{minipage}{.45\textwidth}
% %   \centering
% %   \includegraphics[width=.95\linewidth]{Figures/perCmp.pdf}
% %   \captionof{figure}{Method-level prediction.}
% %   \label{fig:perCmp}
% % \end{minipage}%
% % \begin{minipage}{.45\textwidth}
% %   \centering
% %   \includegraphics[width=.95\linewidth]{Figures/linef1Comp.png}
% %   \captionof{figure}{Top-N recall of line-level prediction.}
% %   \label{fig:linef1Comp}
% % \end{minipage}
% % \end{figure}


% % \begin{table}
% % 	\begin{minipage}{.43\textwidth}
% % 		\centering
% % 		\includegraphics[width=1\linewidth ]{Figures/perCmp.pdf}
% % 		\captionof{figure}{Average precision, recall and F1 for method-level prediction.}
% %         \label{fig:perCmp}
% % 	\end{minipage}\hfill
% % 	\begin{minipage}{.55\textwidth}
% % 		\caption{Top-N recall for line-level prediction.}
% % 		\centering
% % 		\adjustbox{max width=1\textwidth}{

% % 		\begin{tabular}{c|c|c|c|c|c}
% % \hline
% %  \tabincell{c}{Methods} & Top-N & NPE & AIOE & CCE & Avg. \\\hline
% % \multirow{5}{*}{AST} & Top-1 & 37.8 & 28.6 & \textbf{66.7} & \textbf{44.4} \\\cline{2-6}
% % & Top-3 & 55.0 & 35.7 & 66.7 & 52.5 \\\cline{2-6}
% % & Top-5 & 64.0 & 39.3 & \textbf{81.0} & 61.4 \\\cline{2-6}
% % & Top-7 & 72.1 & 42.9 & \textbf{85.7} & 66.9 \\\cline{2-6}
% % & Top-10 & 80.2 & 64.3 & \textbf{95.2} & 79.9 \\\hline
% % \multirow{5}{*}{CFG} & Top-1 & \textbf{47.7} & 32.1 & 52.4 & 44.1 \\\cline{2-6}
% % & Top-3 & 55.9 & 46.4 & 66.7 & 56.3\\\cline{2-6}
% % & Top-5 & 61.3 & 46.4 & 76.2 & 61.3 \\\cline{2-6}
% % & Top-7 & 67.6 & 57.1 & 76.2 & 67.0 \\\cline{2-6}
% % & Top-10 & 79.3 & 64.3 & \textbf{95.2} & 79.6 \\\hline
% % \hline
% % \multirow{5}{*}{\tool} & Top-1 & 44.1 & \textbf{35.7} & 47.6 & 42.5 \\\cline{2-6}
% % & Top-3 & \textbf{57.7} & \textbf{50.0} & \textbf{71.4} & \textbf{59.7} \\\cline{2-6}
% % & Top-5 & \textbf{67.6} & \textbf{71.4} & \textbf{81.0} & \textbf{73.3} \\\cline{2-6}
% % & Top-7 & \textbf{73.0} & \textbf{75.0} & 81.0 & \textbf{76.3} \\\cline{2-6}
% % & Top-10 & \textbf{82.0} & \textbf{75.0} & \textbf{95.2} & \textbf{84.1} \\\hline
% % \end{tabular}}
% % \label{tab:lineres}
% % 	\end{minipage}
% % \end{table}


% % }

% \ignore{

% \begin{figure*}
% \centering
% \begin{tikzpicture}[scale=0.92]
%   \begin{axis}[
%   % x tick label style={/pgf/number format/1000 sep=},
%     ymin=0,ymax=0.7,
%     xlabel=\emph{Number of First Order Intervals}, ylabel=\emph{Top-1 F1 Score},
%     xtick=data,
%     xticklabels={1,2,...,6,7+},
%     ybar,
%     bar width=6pt,
%     legend image code/.code={
%         \draw [#1] (0cm,-0.1cm) rectangle (0.2cm,0.25cm); },
%   ]

%   \addplot [black!30!white,fill=black!30!white] coordinates {
%   (1, 0.297) (2, 0.220) (3, 0.202) (4, 0.213) (5, 0.058) (6, 0.095) (7, 0.044) 
%   };
%   \addplot [black!100!white,fill=black!100!white] coordinates {
%   (1, 0.358) (2, 0.310) (3, 0.233) (4, 0.397) (5, 0.076) (6, 0.154) (7, 0.213)
%   };
%   \legend{\emph{w/o IBPM},\emph{\tool}}
%   \end{axis}
% \end{tikzpicture}%
%     ~%
%     %
% \begin{tikzpicture}[scale=0.92]
%   \begin{axis}[
%   % x tick label style={/pgf/number format/1000 sep=},
%     ymin=0,ymax=0.7,
%     xlabel=\emph{Number of First Order Intervals}, ylabel=\emph{Top-3 F1 Score},
%     xtick=data,
%     xticklabels={1,2,...,6,7+},
%     ybar,
%     bar width=6pt,
%     legend image code/.code={
%         \draw [#1] (0cm,-0.1cm) rectangle (0.2cm,0.25cm); },
%   ]

%   \addplot [black!30!white,fill=black!30!white] coordinates {
%   (1, 0.257) (2, 0.215) (3, 0.183) (4, 0.173) (5, 0.116) (6, 0.115) (7, 0.074) 
%   };
%   \addplot [black!100!white,fill=black!100!white] coordinates {
%   (1, 0.352) (2, 0.288) (3, 0.259) (4, 0.291) (5, 0.102) (6, 0.159) (7, 0.107)
%   };
%   \legend{\emph{w/o IBPM},\emph{\tool}}
%   \end{axis}
% \end{tikzpicture}%
%     ~%
%     %
% \begin{tikzpicture}[scale=0.92]
%   \begin{axis}[
%   % x tick label style={/pgf/number format/1000 sep=},
%     ymin=0,ymax=0.7,
%     xlabel=\emph{Number of First Order Intervals}, ylabel=\emph{Top-5 F1 Score},
%     xtick={1,2,...,7},
%     xticklabels={1,2,...,6,7+},
%     ybar,
%     bar width=6pt,
%     legend image code/.code={
%         \draw [#1] (0cm,-0.1cm) rectangle (0.2cm,0.25cm); },
%   ]

%   \addplot [black!30!white,fill=black!30!white] coordinates {
%   (1, 0.215) (2, 0.182) (3, 0.136) (4, 0.138) (5, 0.090) (6, 0.114) (7, 0.048) 
%   };
%   \addplot [black!100!white,fill=black!100!white] coordinates {
%   (1, 0.326) (2, 0.269) (3, 0.228) (4, 0.219) (5, 0.099) (6, 0.163) (7, 0.071)
%   };
%   \legend{\emph{w/o IBPM},\emph{\tool}}
%   \end{axis}
% \end{tikzpicture}
%     \caption{Comparing IBPM against the standard propagation. \wyc{(11+ represent graphs with more than 11 intervals.)}}
%     \label{fig:pm}
     
% \end{figure*}


% % \begin{figure*}
% % \centering
% %   \begin{tikzpicture}[scale=0.92]
% %   \begin{axis}[
% %     xmax=20,xmin=0,
% %       ymin=0,ymax=0.7,
% %     xlabel=\emph{Training Time (Minutes)},ylabel=\emph{F1 Score for NPE},
% %     xtick={0,4,8,...,20},
% %     ytick={0,0.1,0.20,...,0.7},
% %     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}},
% %   ]
   
% %      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(0, 0.177) (1, 0.171) (2, 0.165) (3, 0.165) (4, 0.165) (5, 0.141) (6, 0.193) (7, 0.168) (8, 0.174) (9, 0.168) (10, 0.153) (11, 0.193) (12, 0.186) (13, 0.180) (14, 0.156) (15, 0.186) (16, 0.165) (17, 0.162) (18, 0.199) (19, 0.165) (20, 0.171)};
% %      \addplot coordinates{(0, 0.245) (1, 0.253) (2, 0.270) (3, 0.291) (4, 0.304) (5, 0.279) (6, 0.287) (7, 0.300) (8, 0.291) (9, 0.291) (10, 0.283) (11, 0.274) (12, 0.296) (13, 0.274) (14, 0.287) (15, 0.287) (16, 0.287) (17, 0.287) (18, 0.291) (19, 0.287) (20, 0.283)};    
% %      \legend{\emph{Baseline}, \emph{\tool}}
% %     \end{axis}
% %     \end{tikzpicture}%
% %     ~%
% %     %
% %     \begin{tikzpicture}[scale=0.92]
% %   \begin{axis}[
% %     xmax=7,xmin=0,
% %     ymin=0,ymax=0.7,
% %     xlabel=\emph{Training Time (Minutes)},ylabel=\emph{F1 Score for AIOE},
% %     xtick={0,1,2,...,7},
% %     ytick={0,0.1,0.20,...,0.7},
% %     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}},
% %     ]
% %      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{ (0, 0.176) (1, 0.196) (2, 0.098) (3, 0.157) (4, 0.196) (5, 0.176) (6, 0.137) (7, 0.157) (8, 0.118) (9, 0.137) (10, 0.157) (11, 0.157) (12, 0.157) (13, 0.098)};
% %      \addplot coordinates{ (0, 0.256) (1, 0.256) (2, 0.320) (3, 0.288) (4, 0.256) (5, 0.288) (6, 0.320) (7, 0.288)};   
% %     \legend{\emph{Baseline},\emph{\tool}}
% %     \end{axis}
% %     \end{tikzpicture}%
% %     ~%
% %     %
% %      \begin{tikzpicture}[scale=0.92]
% %   \begin{axis}[
% %     xmax=10,xmin=0,
% %     ymin=0,ymax=0.7,
% %     xlabel=\emph{Training Time (Minutes)},ylabel=\emph{F1 Score for CCE},
% %     xtick={0,1,2,...,10},
% %     ytick={0,0.1,0.20,...,0.70},
% %     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}},
% %     ]
% %      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{ (0, 0.319) (1, 0.223) (2, 0.191) (3, 0.223) (4, 0.287) (5, 0.255) (6, 0.255) (7, 0.191) (8, 0.255) (9, 0.319) (10, 0.191) (11, 0.191)};
% %      \addplot coordinates{(0, 0.223) (1, 0.260) (2, 0.335) (3, 0.335) (4, 0.297) (5, 0.335) (6, 0.409) (7, 0.372) (8, 0.372) (9, 0.297) (10, 0.335) (11, 0.372) (12, 0.260)};   
% %      \legend{\emph{Baseline},\emph{\tool}}
% %      \end{axis} 
% %      \end{tikzpicture}
% %     \caption{Training time.}
% %     \label{fig:tt}
     
% % \end{figure*}
% }



% !TeX root = ../ggnn.tex
\section{Evaluation}\label{sec:evaluation}
This section presents an extensive evaluation of the three neural bug detectors we instantiate from \tool. First, we evaluate the performance of each neural bug detector. Next, we highlight the improved model capacity IBPM attributes to. Finally, we show how our neural bug detector fares against several static analysis tools in catching null pointer dereference bugs, followed by a summary of applying \tool to catch bugs in the wild.

% Finally, we describe XXX bugs caught by our neural bug detector in XXXX Java projects. %on GitHub.
% compare the bug detectors built based on \tool against those based on an existing AST-based GNN. Next, we highlight the improved generalization of GNN IBPM attributes. Besides, we also show how our neural bug detector fares against several static analysis tools in catching null pointer dereference bugs. Finally, we describe XXX new bugs discovered by our neural bug detector in XXXX popular Java projects on GitHub. 


% \begin{table*}[!tbp]
% \caption{Projects used in the evaluation.}
% % \adjustbox{max width=1.5\paperwidth}{
% \centering
% \small
% \begin{tabular}{c|c|c|c|ccc}
% \hline
%  \multirow{2}{*}{Dataset} & \multirow{2}{*}{Projects} & \multirow{2}{*}{Description}& \multirow{2}{*}{Size (KLoC)}&  \multicolumn{3}{c}{\# of Bugs} \\
% \cline{5-7}
% & & & &\tabincell{c}{NPE} & \tabincell{c}{AIOE} & \tabincell{c}{\tabincell{c}{CCE}} \\\hline
% \multirow{13}{*}{Test} &Lang & Java lang library &50 & 7 & 5 & 2  \\\cline{2-7}
% &Closure & A JavaScript checker and optimizer. &260 & 18 & 0 & 0  \\\cline{2-7}
% &Chart & Java chart library &149 & 17 & 7 & 0  \\\cline{2-7}
% &Mockito & Mocking framework for unit tests &45 & 14 & 5 & 23  \\\cline{2-7}
% &Math & Mathematics and statistics components &165 & 16 & 17 & 3  \\\cline{2-7}
% &Accumulo & Key/value store &194 & 6 & 0 & 0  \\\cline{2-7}
% &Camel & Enterprise integration framework &560 & 17 & 1 & 1  \\\cline{2-7}
% &Flink & System for data analytics in clusters &258 & 13 & 0 & 0  \\\cline{2-7}
% &Jackrabbit-oak & hierarchical content repository &337 & 23 & 1 & 1  \\\cline{2-7}
% &Log4j2 & Logging library for Java &70 & 29 & 1 & 2  \\\cline{2-7}
% &Maven & Project management and comprehension tool & 62 & 6 & 0 & 0  \\\cline{2-7}
% &Wicket & Web application framework &206 & 7 & 1 & 8  \\\cline{2-7}
% &from BugSwarm & 61 projects on GitHub & 5191 & 156 & 20 & 3  \\\hline
% \hline
% \multicolumn{4}{r|}{Total}& 271 & 58 & 41  \\\hline % (num) is the number of buggy methods
% \hline
% \multirow{6}{*}{Training}&Birt & Data visualizations platform &1093 & 678 & 129 & 154  \\\cline{2-7}
% &JDT UI & User interface for the Java IDE & 508 & 897 & 63 & 156 \\\cline{2-7}
% &SWT & Eclipse Platform project repository & 460 & 276 & 136 & 26  \\\cline{2-7}
% &Platform UI & User interface and help components of Eclipse & 595 & 920 & 72 & 194  \\\cline{2-7}
% &AspectJ & An aspect-oriented programming extension &289 & 151 & 14 &  19 \\\cline{2-7}
% &Tomcat & Web server and servlet container &222 & 111 & 18 & 28  \\\hline
% \hline
% \multicolumn{4}{r|}{Total}& 3033 & 432 & 577  \\\hline
% \end{tabular}
% % }
% \label{tab:methodres}
% \end{table*}


\subsection{Implementation}\label{subsec:impl}
Due to the popularity and availability of Java datasets, we target semantic bugs in Java programs. For a different language, \tool only requires a front-end analyzer that extracts the control flow graphs for programs in the new language, the rest of the workflow is language-agnostic. We construct the control flow and interval graphs using Spoon~\cite{pawlak:hal-01169705}, an open-source library for analyzing Java source code.  To efficiently choose correct methods to pair with each buggy method, we run DECKARD~\cite{4222572}, a clone detection tool adopting an approximation of the shortest tree edit distance algorithm to identify similar code snippets. 

We realize our IBPM-based GNN based on GGNN's implementation~\cite{li2015gated}. All neural bug detectors are implemented in Tensorflow. All RNNs built in the model have 1 recurrent layer with 100 hidden units. Each token in the vocabulary is embedded into a 100-dimensional vector. We experimented with other model configurations (\eg more recurrent layers, hidden units, \etc) and did not obtain better results. We use random initialization for weight initialization. We train the neural bug detectors using the Adam optimizer~\cite{kingma2014adam}. All experiments are performed on a 3.7GHz i7-8700K machine with 32GB RAM and NVIDIA GTX 1080 GPU.


% \subsection{Metrics}
% Since we deal with largely unbalanced dataset (\ie the amount of correct code is significantly larger than that of the buggy code), we forgo the accuracy metric. Instead we opt for Precision, Recall, and F1 Score, metrics are commonly used in defect prediction literature~\cite{wang2016automatically,pradel2018deepbugs}.

% \begin{equation*}
% \mathit{Precision} =  \dfrac{\mathit{TP}}{\mathit{TP} + \mathit{FP}}
% \end{equation*}

% \begin{equation*}
%  \mathit{Recall} =  \dfrac{\mathit{TP}}{\mathit{TP} + \mathit{FN}}
% \end{equation*}

% \begin{equation*}
%  \mathit{F1} =  \dfrac{2 \times \mathit{Precision} \times \mathit{Recall}}{\mathit{Precision} +\mathit{Recall}}
% \end{equation*}

% TP, FP, FN stand for true positive, false positive, and false negative respectively. True positive is the number of predicted buggy lines that are truly buggy, while false positive is the number of predicted buggy lines that are not buggy. False negative records the number of buggy lines that are predicted as clean. A higher precision suggests relatively lower number of false warnings while high recall indicates relatively lower number of missed bugs. F1 takes both precision and recall into consideration. 
% The reason we add the prefix of "Top-" is

% after a method is predicted to be buggy our model ranks the statements according to their probabilities of being buggy, 
%the manual inspection on a certain amount of predicted defective methods find more defects, while an increase in recall can reveal more
%defects given a project. F1 takes both precision and recall into consideration.

%To evaluate the performance of defect prediction at the line-level, we use the same three metrics for top-N prediction results. By top-N predictions, we mean considering the top N lines to be buggy ranked by the predicted probabilities, which also implies that the rest of the lines are predicted to be correct. In line-level prediction, TP, FP, FN, TN narrow down the prediction granularity to the level of lines. For example, true positive is the number of predicted defective lines that are truly defective.
 
%means that the correct line gets to be in the top-N probabilities for it to count as ``correct''.

% \begin{equation}
% \label{equ:topn}
% \text{Top-N Recall} =  \dfrac{TP_N}{TP_N + FN_N}
% \end{equation}

% We introduce another metric, top-N recall, dedicated to the prediction at the level of lines. Top-N refers to considering the top N lines to be buggy ranked by the predicted probabilities in a buggy method. Given the top-N predictions, we compute the recall as the only metric of line-level prediction. Our intuition is to favour predictions that capture all bugs in a method. Even it emits a high rate of false warnings, the issue should not be considered as serious since N is a small number. On the contrary, low recall would seriously hurts the usability of a bug finder. As a method is already predicted to be buggy, low recall provides little extra information for developer to pinpoint a bug.


%Note that recall in top-N is the same as top-N accuracy, thus we use recall instead of top-N accuracy. The reason is that each method has only one buggy line according to our setup, and it can be true positive or false negative. The condition is similar in top-N accuracy because whether method is either buggy or clean depends on whether the buggy line is correctly predicted.

%Even though the total number of bugs for them are 1186, 160 and 188 separately, the total number of buggy methods are 2085, 301 and 466.
%The reason is that developers may add patches for more than one method,
%which are all regarded as buggy.
%Therefore, the number of buggy methods are more than the number of bugs.

%Note that we classify all projects into two datasets.
%The first 12 projects are in the testing dataset and the last 6 projects are in the training dataset.
%The evaluation is focus on the cross-project defect prediction, which is more important and has more practical impact than within-project defect prediction.


\begin{table*}[h]
\caption{Details about our dataset. NPE, AIE, and CCE stand for null pointer dereference, array index out of bound and class cast exceptions respectively. Numbers in parenthesis records the number of synthetic bugs we created for AIE and CCE.}
\adjustbox{max width=.8\paperwidth}{
\centering
\small
\begin{tabular}{c|c|c|c|ccc}
\hline
 \multirow{2}{*}{Dataset} & \multirow{2}{*}{Projects} & \multirow{2}{*}{Description}& \multirow{2}{*}{Size (KLoC)}&  \multicolumn{3}{c}{Number of Buggy Methods} \\
\cline{5-7}
& & & &\tabincell{c}{NPE} & \tabincell{c}{AIE} & \tabincell{c}{\tabincell{c}{CCE}} \\\hline
\multirow{13}{*}{Test} &Lang & Java lang library &50 & 7 & 5 & 2  \\\cline{2-7}
&Closure & A JavaScript checker and optimizer. &260 & 18 & 0 & 0  \\\cline{2-7}
&Chart & Java chart library &149 & 17 & 7 & 0  \\\cline{2-7}
&Mockito & Mocking framework for unit tests &45 & 14 & 5 & 23  \\\cline{2-7}
&Math & Mathematics and statistics components &165 & 16 & 17 & 3  \\\cline{2-7}
&Accumulo & Key/value store &194 & 6 & 0 & 0  \\\cline{2-7}
&Camel & Enterprise integration framework &560 & 17 & 1 & 1  \\\cline{2-7}
&Flink & System for data analytics in clusters &258 & 13 & 0 & 0  \\\cline{2-7}
&Jackrabbit-oak & hierarchical content repository &337 & 23 & 1 & 1  \\\cline{2-7}
&Log4j2 & Logging library for Java &70 & 29 & 1 & 2  \\\cline{2-7}
&Maven & Project management and comprehension tool & 62 & 6 & 0 & 0  \\\cline{2-7}
&Wicket & Web application framework &206 & 7 & 1 & 8  \\\cline{2-7}
&Birt & Data visualizations platform &1,093 & 678 & 129 & 154  \\\hline
\hline
\multicolumn{4}{r|}{Number of Buggy Methods in Total for Test}& 793 & 167 & 192  \\ % (num) is the number of buggy methods
\multicolumn{4}{r|}{Number of Methods in Total for Test}& 3,000 & 600 & 800  \\\hline % (num) is the number of buggy methods
\hline
\multirow{6}{*}{Training}
&JDT UI & User interface for the Java IDE & 508 & 897 & 63 & 156 \\\cline{2-7}
&SWT & Eclipse Platform project repository & 460 & 276 & 136 & 26  \\\cline{2-7}
&Platform UI & User interface and help components of Eclipse & 595 & 920 & 72 & 194  \\\cline{2-7}
&AspectJ & An aspect-oriented programming extension &289 & 151 & 14 &  19 \\\cline{2-7}
&Tomcat & Web server and servlet container &222 & 111 & 18 & 28  \\\cline{2-7}
&from BugSwarm & 61 projects on GitHub & 5,191 & 156 & 20 & 3 \\\cline{2-7}
&from BugSwarm & 250 projects on GitHub & 19,874 & (0) & (2,356) & (1,998) \\\hline
\hline
% \multicolumn{4}{r|}{Total}& 2,511 & 323 & 426  \\\hline
\multicolumn{4}{r|}{Number of Buggy Methods in Total for Training}& 2,511 & 2,679 & 2,424  \\
\multicolumn{4}{r|}{Number of Methods in Total for Training}& 10,000 & 10,000 & 10,000  \\\hline
\end{tabular}
}
\label{tab:stas}
\end{table*}


\subsection{Experiment Setup}
We assemble a dataset according to the procedure described in Section~\ref{subsec:data}.
% To create a dataset for our evaluation, we refer to defect4j~\cite{just2014defects4j}, bugs.jar~\cite{saha2018bugs}, BugSwarm~\cite{tomassi2019bugswarm} and the other by~\citet{ye2014learning}, four real-world, publicly accessible bug databases. All databases provide a rich set of information pertaining to each bug they contain (\eg commits made by developers that introduce or fix bugs, bug reports, \etc). We rely on such
% information to extract buggy methods and identify the bug type. We run DECKARD to collect clean methods in the same project from which a buggy method is extracted. 
Table~\ref{tab:stas} shows the details: the projects from which we extract the code snippet, a brief description of their functionality, size of their codebase, and the number of buggy methods we extract from each project. We maintain approximately 3:1 ratio between the correct and buggy methods across each bug type within each project.
To enrich the set of AIE (Array Index Out of Bound Exception) and CCE (Class Cast Exception) bugs, we create synthetic buggy examples based on a collection of highly-rated and actively maintained projects from BugSwarm~\cite{tomassi2019bugswarm}. In particular, we first randomly pick methods that contain either array access or class cast operations, and then strip away the bounds or type checks. The number in parenthesis depicts how many buggy examples we synthesized for AIE and CCE. Note that all synthetic bugs are used for the training purpose only, and all bugs in the test set are real. We also make certain clean methods that are paired with synthetic buggy examples are chosen from other methods rather than their original version (\ie with the bounds or type checks). We evaluate \tool on a standard classification task, that is, predicting each line in a method in the test set to be buggy or not. Since we deal with a largely unbalanced dataset, we forgo the accuracy metric and opt for Precision, Recall, and F1 Score, metrics are commonly used in defect prediction literature~\cite{wang2016automatically,pradel2018deepbugs}.

As a baseline, we select standard GGNN~\cite{li2015gated,allamanis2017learning}, a predominate deep learning model in the domain of programming. In particular, we re-implemented the program encoding scheme proposed by~\citet{allamanis2017learning}, a graph representation built of top of the AST with additional edges denoting variable types, data, control flow dependencies, \etc


% \begin{table}[!t]
% \centering
% \normalsize
% \caption{Dataset statistics. NPE, AIE and CCE stand for null pointer deference, array index out of bound and class cast exceptions respectively.}
% \adjustbox{max width=\columnwidth}{\begin{tabular}{c|ccc|ccc}
% \hline
%  \multirow{2}{*}{\tabincell{c}{Dataset}} & \multicolumn{3}{c|}{\# of Buggy Methods} & \multicolumn{3}{c}{\# of Clean Methods}\\
% \cline{2-7}
%          & NPE & AIE & CCE & for NPE & for AIE & for CCE  \\\hline
% Training & 3033 & 432 & 577 & 3033 & 432 & 577    \\\hline
% Test & 271 & 58 & 41 & 271 & 58 & 41    \\\hline

% \end{tabular}}
% \label{tab:stas}
% \end{table}

% \begin{table}[!t]
% \centering
% \normalsize
% \caption{Dataset statistics. NPE, AIE and CCE stand for null pointer deference, array index out of bound and class cast exceptions respectively.}
% \adjustbox{max width=\columnwidth}{\begin{tabular}{c|ccc|c}
% \hline
%  \multirow{2}{*}{\tabincell{c}{Dataset}} & \multicolumn{3}{c|}{\# of Buggy Methods} & \multirow{2}{*}{\tabincell{c}{\# of Clean Methods}}\\
% \cline{2-4}
%          & NPE & AIE & CCE &   \\\hline
% Training & 3033 & 432 & 577 & 4000    \\\hline
% Test & 271 & 58 & 41 & 400    \\\hline

% \end{tabular}}
% \label{tab:stas}
% \end{table}



% We use defect4j~\cite{just2014defects4j}, bugs.jar~\cite{saha2018bugs}, BugSwarm~\cite{tomassi2019bugswarm} and the other by~\citet{ye2014learning}, which are all real-world, publicly accessible datasets, for our evaluation. We select projects that contain at least one bug of null pointer dereference, array index out of bound or class cast in their codebases.

% As mentioned previously, we obtain the labels for each buggy method and their lines by cross-referencing the commit history and bug reports. Specifically, we search for commits that are considered to be bug fixes, and infer the type of the bug by referencing the bug reports. Methods and lines that are modified by commits of bug fixes are labeled buggy. Finally, we pick a correct method that is syntactically similar to pair with the buggy method. 

%unified these datasets with the following steps:
%(1) Locate a bug description for each bug by string matching;
%(2) Locate a commit that repairs each bug;
%(3) Label buggy methods if they are inside the modification by a patch;
%(4) Label clean methods whose complexity are similar to the buggy methods.

% Table~\ref{tab:methodres} depicts all selected projects including a brief description of their functionality. The first column shows if a project is used in the training or test set, and the last three columns denote the number of bugs it contains for each type. We also provide the size of the codebase for each project.
% % are the number of total methods for each of the three bug types. Numbers in parenthesis are the number of buggy methods. For the actual number of bugs and buggy methods in each project\footnote{Developers may fix multiple methods for a single bug so the number of buggy methods and bugs may not be identical.}, we invite readers to refer to the supplemental material for the details. 
% Our evaluation focuses on the cross-project defect prediction, which resembles the real usage scenarios of \tool better than within-project defect prediction.


% \begin{table*}[!tbp]
% \caption{Projects used in the evaluation.}
% \adjustbox{max width=\textwidth}{
% \centering
% \small
% \begin{tabular}{c|c|c|ccc}
% \hline
%  \multirow{2}{*}{Dataset} & \multirow{2}{*}{Projects} & \multirow{2}{*}{Description}&  \multicolumn{3}{c}{\#Methods} \\
% \cline{4-6}
% & & &\tabincell{c}{NPE} & \tabincell{c}{AIOE} & \tabincell{c}{\tabincell{c}{CCE}} \\\hline
% \multirow{13}{*}{Test} &Lang & Java lang library & 115 & 46 & 75  \\\cline{2-6}
% &Closure & A JavaScript checker and optimizer. & 11 & 0 & 0  \\\cline{2-6}
% &Chart & Java chart library & 120 & 5 & 0  \\\cline{2-6}
% &Mockito & Mocking framework for unit tests & 49 & 6 & 42  \\\cline{2-6}
% &Math & Mathematics and statistics components & 44 & 59 & 14  \\\cline{2-6} % 121+67, 139+145, 31
% &Accumulo & Key/value store & 16 & 0 & 0  \\\cline{2-6}
% &Camel & Enterprise integration framework & 155 & 20 & 6  \\\cline{2-6}
% &Flink & System for data analytics in clusters & 33 & 0 & 0  \\\cline{2-6}
% &Jackrabbit-oak & hierarchical content repository & 68 & 7 & 12  \\\cline{2-6}
% &Log4j2 & Logging library for Java & 44 & 2 & 1  \\\cline{2-6}
% &Maven & Project management and comprehension tool & 12 & 0 & 0  \\\cline{2-6}
% &Wicket & Web application framework & 23 & 8 & 16  \\\hline
% \hline
% \multicolumn{3}{r|}{Total}& 690 (173) & 153 (38) & 166 (40)  \\\hline % (num) is the number of buggy methods
% \hline
% \multirow{6}{*}{Training}&Birt & Data visualizations platform & 1356 & 258 & 308  \\\cline{2-6}
% &JDT UI & User interface for the Java IDE & 1794 & 126 & 312 \\\cline{2-6}
% &SWT & Eclipse Platform project repository & 552 & 272 & 52  \\\cline{2-6}
% &Platform UI & User interface and help components of Eclipse & 1840 & 144 & 388  \\\cline{2-6}
% &AspectJ & An aspect-oriented programming extension & 302 & 28 &  38 \\\cline{2-6}
% &Tomcat & Web server and servlet container & 222 & 36 & 56  \\\hline
% \hline
% \multicolumn{3}{r|}{Total}& 6066 (3033) & 864 (432) & 1154(577)  \\\hline
% \end{tabular}}
% \label{tab:methodres}
% \end{table*}

% \subsection{Baselines}
% %To gain a better understanding of the performance of our neural bug detectors, 
% We compare \tool against the standard GGNN~\cite{li2015gated,allamanis2017learning}, a predominate deep learning model in the domain of programming. In particular, we re-implemented the program encoding scheme proposed by~\citet{allamanis2017learning}, a graph representation built of top of the AST with additional edges denoting variable types, data, control flow dependencies, \etc
% For convenience, we refer the first baseline as AST method and the second as CFG method. 

% proposed in while the second one uses a control flow graph-based program encoding. In both methodologies, we feed the program graphs to a standard GGNN built with the existing propagation model. 

% \ignore{
% To evaluate the performance of our method in defect
% prediction, we compare interval graphs with traditional graphs and compare CFG-based representations with AST-based representations~\cite{allamanis2017learning}. 
% Our first baseline is CFG-based representation without introducing intervals.
% Except for the interval representation and node representation, other setups are the same as \tool.
% For a fair comparison, our second baseline of graph representation is based on AST that without taking control flow into consideration. 
% }


%Moreover, The second baseline is a re-implementation of AST-based program representation \cite{allamanis2017learning}, which additionally adds data flow edges in the graph constructed from AST and leverages variable type information. The graph in AST is a tree, with an additional kind of edge that connects leaf nodes from one side to another side.



% \subsection{Compare Node Initializations}
% We compare the three encoding schemes for node initialization: characteristic vectors, RNN-based encoding and transformer-based encoding. We show the performance of each encoding at both method-level and line-level predictions.

% Table \ref{tab:alter} presents the method-level prediction results of the three encoding schemes in precision, recall and F1. Figure~\ref{fig:alterComp} shows the average of all three metrics across all bug types for each encoding. We find that GGNN exhibits a decent performance in all node initialization schemes. 
% %The reason is that the representations and information propagation enable \tool to reason about semantic similarities between syntactically different methods, which allows it to learn and predict bugs across similar methods. 
% In particular, RNN-based encoding has the highest recall and F1 score in all three bug types (\ie on average higher than characteristic vectors and transformer-based encoding by 12.9\% and 12.0\% respectively), indicating it's the most precise encoding scheme for node initialization.
% %best representation among the three methods.
% %For example, the average improvement of F1 introduced by RNN-based encoding is 10.3\% and 3.3\% for characteristic vectors and transformer-based encoding.

% As for the line-level predictions, we depict the average top-N recall across all bug types for each encoding scheme in Figure~\ref{fig:alterCompLine}. The characteristic vectors based encoding again falls behind whereas the RNN-based encoding shows a slight advantage over transformer-based encoding. The reason is that characteristic vectors do not capture as precise a representation of a statement as the other two. As for the transformer, we find their capabilities do not transfer to the programming field. We suspect this is caused by the fundamental difference between program language and natural language.

% Based on the comparison among the three encoding schemes for node initialization, we choose the RNN-based encoding as \tool's default configuration, in which we compare \tool against the 
% two baselines in the remaining experiments.

% \ignore{
% conthis one for the remaining evaluation, including the performance of \tool between AST method and CFG method and the requirement about the number of bugs in the dataset.


% at both method- and line-level predictions, 



% The result shows that RNN-based encoding shows the best performance among the three alternative representations.
% Therefore, we choose this one for the remaining evaluation, including the performance of \tool between AST method and CFG method and the requirement about the number of bugs in the dataset.









% the results are depicted in Figure~\ref{fig:alterCompLine} with the average F1 score between the three representations.
% The characteristic vectors embedding is still the worst one among the three while the RNN-based encoding shows a slightly benefit than transformer-based encoding.

% The reason is that characteristic vectors are not expressive enough to capture semantic features of methods.
% As for the transformer, it demonstrates that syntax of methods is different from the natural language \cite{vaswani2017attention}, leading to the different performance between RNN-based encoding and transformer-based encoding.

% The result shows that RNN-based encoding shows the best performance among the three alternative representations.
% Therefore, we choose this one for the remaining evaluation, including the performance of \tool between AST method and CFG method and the requirement about the number of bugs in the dataset.
% }

% \begin{figure}[h]
% \begin{subfigure}[t]{0.47\textwidth}
% \centering
%   \includegraphics[width=0.95\linewidth]{Figures/alterComp.pdf}
%   \caption{Compare the average precision, recall and F1 for different node initialization schemes.}
%   \label{fig:alterComp}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.47\textwidth}
% \centering
%   \includegraphics[width=0.95\linewidth]{Figures/alterCompLine.png}
%   \caption{Average top-N recall of different node initialization schemes.}
%   \label{fig:alterCompLine}
% \end{subfigure}
% \caption{Comparison among the different node initialization schemes using average across all bug types.}
% \label{fig:alterPerf}
% \end{figure}


% \begin{table*}[!t]
% \centering
% \small
% \caption{Compare the different encoding for node intialization.}
% \begin{tabular}{c|ccc|ccc|ccc}
% \hline
% \multirow{2}{*}{\tabincell{c}{Node \\Representations}} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{AIOE} & \multicolumn{3}{c}{CCE}\\
% \cline{2-10}
% & Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall & F1 \\\hline
% \tabincell{c}{Characteristic\\vectors}&  26.6 & 64.0 & 37.6 & 40.1 & 82.1 & 53.9 & 27.9 & 52.4 & 36.4   \\\hline
% \tabincell{c}{RNN-based\\encoding } & \textbf{30.3} & \textbf{72.1} & \textbf{42.6} & \textbf{44.7} & \textbf{85.7} & \textbf{58.7} & \textbf{41.9} & \textbf{81.0} & \textbf{55.3} \\\hline
% \tabincell{c}{Transformer-based\\encoding } & 29.0 & 68.5 & 40.8 & 44.6 & 82.1 & 57.8 & 38.7 & 66.7 & 49.0  \\\hline 

% \end{tabular}
% \label{tab:alter}
% \end{table*}




% the method-level prediction. The highest precision, recall and F1 for each bug type is highlighted in bold. In general, \tool is better than AST method and CFG method in most metrics, particularly, \tool is far more accurate in dealing with null pointer dereference and array index out of bound bugs (\ie by more than 10\% in F1 score). Furthermore, we find out \tool beats the two baselines by even bigger margin in F1 score on the top 10\% largest graphs (\ie 73.5\% by \tool vs. 29.3\% by CFG vs. 38.9\% by AST ), indicating the interval-based propagation model indeed improves the scalability of GGNN for generalizing on larger graphs. Figure~\ref{fig:largeGraph} shows how the F1 score changes for each methodology across the graph size. 

%For example, for array index out of bound bug, the F1 score is 58.7\%, while the F1 is 43.2\% with the first baseline of AST-based representation, and the F1 is 39.5\% with the CFG method.

% Figure~\ref{fig:perCmp} shows a bar graph charting the average performance across all bug types among the three methodologies. On average, \tool achieves 52.2\% in F1 score, while the AST and CFG method achieve 42.0\% and 40.8\% respectively. In terms of the average recall, \tool achieves 79.6\% while AST and CFG achieve 60.2\% and 62.3\% respectively. Our results demonstrate at the method-level prediction, \tool outperforms the baselines in both recall and F1 significantly.


%\ke{Yu this sentence is not clear to me: The results demonstrate that \tool on average outperforms the baselines by 20.8\% in F1 score and 29.9\% in recall among the 12 projects.} \wyc{WY: it means that \tool is 20.8\% better than AST and CFG method in F1 score and 29.9\% better than the two method in recall. The formula is $20.8\%=((F1_{\tool}-F1_{AST})/F1_{\tool} + (F1_{\tool}-F1_{CFG})/F1_{\tool})/2$}
   

\begin{table*}
\begin{minipage}{.33\textwidth}
\captionsetup{skip=1pt}
\caption{Precision in predicting NPE.}
\centering
\adjustbox{max width=1\textwidth}{
\begin{tabular}{c|c|c|c}
\hline
 \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
Baseline (0) & 0.209 & 0.147 & 0.117 \\\hline
Baseline (1) & \textit{0.285} & 0.166 & 0.131 \\\hline
Baseline (2) & 0.218 & 0.138 & 0.101 \\\hline
\tool (0) & 0.326 & 0.174 & 0.138 \\\hline
\tool (1) & \textbf{0.351} & 0.167 & 0.130 \\\hline
\tool (2) & 0.305 & 0.164 & 0.136 \\\hline
\hline
Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.351} - \textit{0.285} = 0.066} \\\hline
\end{tabular}}
\label{tab:preNPE}
\end{minipage}
\begin{minipage}{.33\textwidth}
\captionsetup{skip=1pt}
\caption{Recall in predicting NPE.}
\centering
\adjustbox{max width=1\textwidth}{
\begin{tabular}{c|c|c|c}
\hline
 \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
Baseline (0) & 0.243 & 0.373 & \textit{0.450} \\\hline
Baseline (1) & 0.171 & 0.252 & 0.302 \\\hline
Baseline (2) & 0.210 & 0.337 & 0.375 \\\hline
\tool (0) & 0.282 & 0.374 & 0.447 \\\hline
\tool (1) & 0.329 & 0.431 & \textbf{0.507} \\\hline
\tool (2) & 0.304 & 0.402 & 0.500 \\\hline
\hline
Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.507} - \textit{0.450} = 0.057} \\\hline
\end{tabular}}
\label{tab:reNPE}
\end{minipage}
\begin{minipage}{.33\textwidth}
\captionsetup{skip=1pt}
\caption{F1 score in predicting NPE.}
\centering
\adjustbox{max width=1\textwidth}{
\begin{tabular}{c|c|c|c}
\hline
 \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
Baseline (0) & \textit{0.224} & 0.211 & 0.186 \\\hline
Baseline (1) & 0.214 & 0.201 & 0.183 \\\hline
Baseline (2) & 0.214 & 0.196 & 0.159 \\\hline
\tool (0) & 0.303 & 0.238 & 0.211 \\\hline
\tool (1) & \textbf{0.339} & 0.241 & 0.207 \\\hline
\tool (2) & 0.304 & 0.233 & 0.214 \\\hline
\hline
Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.339} - \textit{0.224} = 0.115} \\\hline
\end{tabular}}
\label{tab:f1NPE}
\end{minipage}

\par\bigskip

\begin{minipage}{.33\textwidth}
\captionsetup{skip=1pt}
\caption{Precision in predicting AIE.}
\centering
\adjustbox{max width=1\textwidth}{
\begin{tabular}{c|c|c|c}
\hline
 \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
Baseline (0) & \textit{0.286} & 0.124 & 0.106 \\\hline
Baseline (1) & 0.218 & 0.112 & 0.095 \\\hline
Baseline (2) & 0.215 & 0.134 & 0.088 \\\hline
\tool (0) & 0.269 & 0.159 & 0.113 \\\hline
\tool (1) & 0.308 & 0.134 & 0.097 \\\hline
\tool (2) & \textbf{0.362} & 0.131 & 0.110 \\\hline
\hline
Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.362} - \textit{0.286} = 0.076} \\\hline
\end{tabular}}
\label{tab:preAI}
\end{minipage}\hfill
\begin{minipage}{.33\textwidth}
\captionsetup{skip=1pt}
\caption{Recall in predicting AIE}
\centering
\adjustbox{max width=1\textwidth}{
\begin{tabular}{c|c|c|c}
\hline
 \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
Baseline (0) & 0.231 & 0.266 & \textit{0.355} \\\hline
Baseline (1) & 0.165 & 0.225 & 0.300 \\\hline
Baseline (2) & 0.180 & 0.288 & 0.306 \\\hline
\tool (0) & 0.284 & 0.425 & 0.470 \\\hline
\tool (1) & 0.291 & 0.358 & 0.403 \\\hline
\tool (2) & 0.333 & 0.378 & \textbf{0.489} \\\hline
\hline
Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.489} - \textit{0.355} = 0.134} \\\hline
\end{tabular}}
\label{tab:reAI}
\end{minipage}\hfill
\begin{minipage}{.33\textwidth}
\captionsetup{skip=1pt}
\caption{F1 score in predicting AIE.}
\centering
\adjustbox{max width=1\textwidth}{
\begin{tabular}{c|c|c|c}
\hline
 \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
Baseline (0) & \textit{0.256} & 0.169 & 0.163 \\\hline
Baseline (1) & 0.188 & 0.149 & 0.145 \\\hline
Baseline (2) & 0.196 & 0.183 & 0.136 \\\hline
\tool (0) & 0.276 & 0.232 & 0.182 \\\hline
\tool (1) & 0.299 & 0.195 & 0.157 \\\hline
\tool (2) & \textbf{0.347} & 0.195 & 0.179 \\\hline
\hline
Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.347} - \textit{0.256} = 0.091} \\\hline
\end{tabular}}
\label{tab:f1AI}
\end{minipage}\hfill

\par\bigskip

\begin{minipage}{.33\textwidth}
\captionsetup{skip=1pt}
\caption{Precision in predicting CCE.}
\centering
\adjustbox{max width=1\textwidth}{
\begin{tabular}{c|c|c|c}
\hline
 \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
Baseline (0) & 0.345 & 0.165 & 0.169 \\\hline
Baseline (1) & 0.328 & 0.180 & 0.135 \\\hline
Baseline (2) & \textit{0.352} & 0.198 & 0.173 \\\hline
\tool (0) & 0.362 & 0.220 & 0.170 \\\hline
\tool (1) & \textbf{0.438} & 0.244 & 0.199 \\\hline
\tool (2) & \textbf{0.438} & 0.252 & 0.193 \\\hline
\hline
Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.438} - \textit{0.387} = 0.051} \\\hline
\end{tabular}}
\label{tab:preCC}
\end{minipage}\hfill
\begin{minipage}{.33\textwidth}
\captionsetup{skip=1pt}
\caption{Recall in predicting CCE.}
\centering
\adjustbox{max width=1\textwidth}{
\begin{tabular}{c|c|c|c}
\hline
 \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
Baseline (0) & 0.270 & 0.319 & 0.467 \\\hline
Baseline (1) & 0.319 & 0.369 & 0.393 \\\hline
Baseline (2) & 0.291 & 0.371 & \textit{0.503} \\\hline
\tool (0) & 0.286 & 0.443 & 0.495 \\\hline
\tool (1) & 0.292 & 0.413 & 0.486 \\\hline
\tool (2) & 0.384 & 0.561 & \textbf{0.620} \\\hline
\hline
Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.620} - \textit{0.503} = 0.117} \\\hline
\end{tabular}}
\label{tab:reCC}
\end{minipage}\hfill
\begin{minipage}{.33\textwidth}
\captionsetup{skip=1pt}
\caption{F1 score in predicting CCE.}
\centering
\adjustbox{max width=1\textwidth}{
\begin{tabular}{c|c|c|c}
\hline
 \tabincell{c}{Methods} & Top-1 & Top-3 & Top-5  \\\hline
Baseline (0) & 0.303 & 0.217 & 0.249 \\\hline
Baseline (1) & \textit{0.323} & 0.242 & 0.201 \\\hline
Baseline (2) & 0.319 & 0.258 & 0.257 \\\hline
\tool (0) & 0.320 & 0.294 & 0.254 \\\hline
\tool (1) & 0.350 & 0.307 & 0.282 \\\hline
\tool (2) & \textbf{0.409} & 0.348 & 0.295 \\\hline
\hline
Gain & \multicolumn{3}{|l}{\hspace{1pt}\textbf{0.409} - \textit{0.323} = 0.086} \\\hline
\end{tabular}}
\label{tab:f1CC}
\end{minipage}\hfill
\end{table*}

\ignore{
\begin{table*}
\begin{minipage}{.33\textwidth}
\captionsetup{skip=1pt}
\caption{Precision in predicting all bugs.}
\centering
\adjustbox{max width=1\textwidth}{
\begin{tabular}{c|c|c|c}
\hline
 \tabincell{c}{\#Interval} & Top-1 & Top-3 & Top-5  \\\hline
1-2 & 51.1/40.2 & 29.7/23.2 & 24.0/18.1 \\\hline
3-4 & 10.0/23.1 & 8.9/12.3 & 8.7/9.2 \\\hline
5-6 & 4.3/0.0 & 2.9/6.0 & 1.7/4.8 \\\hline
>6 & 8.3/0.0 & 2.8/0.0 & 3.3/0.7 \\\hline
\end{tabular}}
\label{tab:cfgpre}
\end{minipage}
\begin{minipage}{.33\textwidth}
\captionsetup{skip=1pt}
\caption{Recall in predicting all bugs.}
\centering
\adjustbox{max width=1\textwidth}{
\begin{tabular}{c|c|c|c}
\hline
 \tabincell{c}{\#Interval} & Top-1 & Top-3 & Top-5  \\\hline
1-2 & 30.2/37.1 & 40.4/49.9 & 46.7/55.9 \\\hline
3-4 & 9.7/21.4 & 25.8/34.3 & 41.9/42.9 \\\hline
5-6 & 4.5/0.0 & 9.1/26.0 & 9.1/34.6 \\\hline
>6 & 8.3/0.0 & 8.3/0.0 & 16.7/3.3 \\\hline
\end{tabular}}
\label{tab:cfgre}
\end{minipage}
\begin{minipage}{.33\textwidth}
\captionsetup{skip=1pt}
\caption{F1 score in predicting all bugs.}
\centering
\adjustbox{max width=1\textwidth}{
\begin{tabular}{c|c|c|c}
\hline
 \tabincell{c}{\#Interval} & Top-1 & Top-3 & Top-5  \\\hline
1-2 & 37.9/38.6 & 34.2/31.7 & 31.7/27.4 \\\hline
3-4 & 9.8/22.2 & 13.2/18.1 & 14.4/15.2 \\\hline
5-6 & 4.4/NA & 4.4/9.7 & 2.9/8.4 \\\hline
>6 & 8.3/NA & 4.2/NA & 5.6/1.1 \\\hline
\end{tabular}}
\label{tab:cfgf1}
\end{minipage}

\par\bigskip

\end{table*}
}


\subsection{Performance Measurement}
We build two sets of neural bug detectors based on \tool and the baseline. Each set includes three models, each of which deals with null pointer dereference, array index out of bound and class casting bugs respectively. 

\paragraph{Evaluating models using proposal metrics} Table~\ref{tab:preNPE}--\ref{tab:f1CC} depicts the precision, recall, and F1 for all neural bug detectors. We set out to examine the impact of the depth of inlining on the performance of each bug detector. In particular, each row in a table shows the result of a neural bug detector that is trained either using the baseline model or \tool. The number in parenthesis is the depth of inlining. Specifically, 0 means no inlining, 1 inlines all methods that are invoking or invoked by the target methods, and 2 further inlines all callers and callees of each method that is inlined by 1. Exceeding the depth of 2 has costly consequences. First, most data points will have to be filtered out for overflowing the GPU memory. Moreover, a significant portion of the remaining ones would also have to be placed in a batch on its own, resulted in a dramatic increase in training time. Methods in the test set are inlined as deep as those in the training set to maintain a consistent distribution across the entire dataset. We also make certain each buggy method is only inlined once to prevent a potential date duplicate issue.
% Note that with inlining we will inevitably introduce duplicate data points. For example, if method A calls method B, which happens to be buggy, then inlining method A by depth 1 will receive the same bug labels as inlining method B by depth 1 providing that no other caller or callee of either method A or B is buggy. In other words, we may potentially recount the predictions made on the identical buggy examples. 
% % We remove the data points which include buggy methods that are already covered by 
% Concerned with the validity of our experiments, we make certain none of the buggy methods is shared among multiple data points in the test set. 
Columns in each table correspond to three prediction modes in which \tool picks 1, 3 or 5 statements to be buggy after a method is predicted to be buggy.

Overall, \tool consistently outperforms the baseline across all bug types using all proposed metrics. In particular, \tool beats the baseline by around 10\% across all bugs types in F1 score. 
% For null pointer dereference, \tool achieves far better results in all three metrics across all prediction configurations. For array index out of bound and class cast exceptions, \tool is still considerably better than the baseline despite performing marginally worse on occasion. 
Regarding the impact of the depth of inlining, we find that increasing the depth mostly but not always leads to improved performance of either \tool or the baseline. The reason is, on one hand, models will benefit from a more complete program representation thanks to the inlining. On the other hand, exceedingly large graphs hinders the generalization of GNNs, resulted in degraded performance of the neural bug detectors. 

% \begin{table*}[!t]
% \centering
% \small
% \caption{Method-level prediction results.}
% \begin{tabular}{c|ccc|ccc|ccc}
% \hline
%  \multirow{2}{*}{\tabincell{c}{Methods}} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{AIOE} & \multicolumn{3}{c}{CCE} \\
% \cline{2-10}
% & Precision & Recall & F1 & Precision & Recall & F1  & Precision & Recall & F1  \\\hline
% AST & 24.0 & 52.3 & 32.3 & 34.8 & 57.1 & 43.2 & 38.3 & 71.4 & 49.8  \\\hline
% CFG & 24.2 & 55.9 & 33.8 & 28.5 & 64.3 & 39.5 & 38.7 & 66.7 & 49.0  \\\hline
% \hline
% \tool & \textbf{30.3} & \textbf{72.1} & \textbf{42.6} & \textbf{44.7} & \textbf{85.7} & \textbf{58.7} & \textbf{41.9} & \textbf{81.0} & \textbf{55.3} \\\hline

% \end{tabular}
% \label{tab:metRes}
% \end{table*}



% \begin{figure}
% \centering
% \begin{minipage}{.45\textwidth}
%   \centering
%   \includegraphics[width=.95\linewidth]{Figures/perCmp.pdf}
%   \captionof{figure}{Average precision, recall and F1 for method-level prediction.}
%   \label{fig:perCmp}
% \end{minipage}\hfill
% \begin{minipage}{.45\textwidth}
%   \centering
%   \includegraphics[width=.95\linewidth]{Figures/largeGraph.png}
%   \captionof{figure}{F1 score of each methodology in top N\% largest graphs.}
%   \label{fig:largeGraph}
% \end{minipage}
% \end{figure}



% \begin{table}

% 	\begin{minipage}{.55\textwidth}
% 		\caption{Top-N recall for line-level prediction.}
% 		\centering
% 		\adjustbox{max width=1\textwidth}{

% 		\begin{tabular}{c|c|c|c|c|c}
% \hline
%  \tabincell{c}{Methods} & Top-N & NPE & AIOE & CCE & Avg. \\\hline
% \multirow{5}{*}{AST} & Top-1 & 37.8 & 28.6 & \textbf{66.7} & \textbf{44.4} \\\cline{2-6}
% & Top-3 & 55.0 & 35.7 & 66.7 & 52.5 \\\cline{2-6}
% & Top-5 & 64.0 & 39.3 & \textbf{81.0} & 61.4 \\\cline{2-6}
% & Top-7 & 72.1 & 42.9 & \textbf{85.7} & 66.9 \\\cline{2-6}
% & Top-10 & 80.2 & 64.3 & \textbf{95.2} & 79.9 \\\hline
% \multirow{5}{*}{CFG} & Top-1 & \textbf{47.7} & 32.1 & 52.4 & 44.1 \\\cline{2-6}
% & Top-3 & 55.9 & 46.4 & 66.7 & 56.3\\\cline{2-6}
% & Top-5 & 61.3 & 46.4 & 76.2 & 61.3 \\\cline{2-6}
% & Top-7 & 67.6 & 57.1 & 76.2 & 67.0 \\\cline{2-6}
% & Top-10 & 79.3 & 64.3 & \textbf{95.2} & 79.6 \\\hline
% \hline
% \multirow{5}{*}{\tool} & Top-1 & 44.1 & \textbf{35.7} & 47.6 & 42.5 \\\cline{2-6}
% & Top-3 & \textbf{57.7} & \textbf{50.0} & \textbf{71.4} & \textbf{59.7} \\\cline{2-6}
% & Top-5 & \textbf{67.6} & \textbf{71.4} & \textbf{81.0} & \textbf{73.3} \\\cline{2-6}
% & Top-7 & \textbf{73.0} & \textbf{75.0} & 81.0 & \textbf{76.3} \\\cline{2-6}
% & Top-10 & \textbf{82.0} & \textbf{75.0} & \textbf{95.2} & \textbf{84.1} \\\hline
% \end{tabular}}
% \label{tab:lineres}
% 	\end{minipage}\hfill
% 		\begin{minipage}{.43\textwidth}
% 		\centering
% 		\includegraphics[width=1\linewidth ]{Figures/largeGraphLine.png}
% 		\captionof{figure}{Top-3 recall in top N\% largest graphs at line-level prediction.}
%         \label{fig:largeGraphLine}
% 	\end{minipage}
% \end{table}

% \ke{line-level below}
% To completely separate the line-level prediction with the method-level 
% prediction, we train all neural bug detectors from buggy methods only. In other words, the job of line-level predictors is to locate the bugs in a known buggy method. 
%To evaluate the line-level performance, we only keep buggy methods for training and testing.
%Therefore, all data for training and testing are buggy methods with analyzed buggy lines.
%In this way, we can have a more clear performance without affected by method-level prediction results.
% Table \ref{tab:lineres} presents the top-N recall of the line-level prediction results. We choose N to be 1, 3, 5, 7, and 10 for 
% multiple prediction configurations. As before, we highlight the highest top-N recall for each methodology across all bug types. Overall, \tool outperforms the baslines in most metrics. Specifically, for array index out of bound bugs, \tool yields significantly better models than AST and CFG methods in each top-N configuration. However, the improvement \tool made over the baselines is not as significant as that in method-level prediction, especially in dealing with class cast bugs where AST method outperforms \tool in certain configurations. The last column shows average top-N recall performance among all three bug types. \tool achieves almost 60\% in top-3 and more than 70\% in top-5 recall, which is still notably better than the two other methodologies. Figure~\ref{fig:largeGraphLine} depicts the top-3 recall across the graph size. Similar to the method-level prediction, \tool shows bigger improvement over the baselines on the top 10\% largest graphs. 

% \ignore{
% As the results show, \tool is over-perform than AST method and CFG method in many cases.
% For example, for all the three metrics in array index out of bound bugs, \tool beats the two baselines with overwhelming performance.
% The average improvement in the top-N accuracy is 30.1\% and 18.0\% for AST method and CFG method when predicting the array index out of bound bug. 
% However, the performance of \tool in line-level prediction is not as good as method-level prediction results.
% AST method is beatable in some cases, such as predicting CCE bugs.
% %The performance is better for AST method.
% The last column shows average performance among the three kinds of bugs.
% The overall performance shows that \tool is better than the two baselines with around 8.3\% improvement.


% \textit{Top-N} in the second column represents that we regard \textit{N} predictions as buggy. The N we choose is 1, 3, 5, 7, and 10.
% A row with top-N means that precision, recall and F1 are evaluated when predicting \textit{N} lines as buggy and remaining lines as clean.
% In this table, we highlight the highest precision, recall and F1 of the three methods.
% We can see from the table that all metrics are the same in top-1. 
% The reason is that if a method has $N$ statements, we only predict one statement as buggy.
% If the prediction is wrong, then both FP and FN are increased by 1, which means that FP is the same as FN. 

% As the results show, \tool is over-perform than AST method and CFG method in many cases.
% For example, for all the three metrics in array index out of bound bugs, \tool beats the two baselines with overwhelming performance.
% The average improvement in the top-N accuracy is 30.1\% and 18.0\% for AST method and CFG method when predicting the array index out of bound bug. 
% However, the performance of \tool in line-level prediction is not as good as method-level prediction results.
% AST method is beatable in some cases, such as predicting CCE bugs.
% %The performance is better for AST method.
% The last column shows average performance among the three kinds of bugs.
% The overall performance shows that \tool is better than the two baselines with around 8.3\% improvement.}


% \ignore{
% From the method-level and line-level evaluation, we can find that \tool is over-perform than two baselines in method-level performance and \tool is comparable to AST method in line-level prediction.
% Additionally, note that the line-level evaluation is only focus on buggy method, which means that the combination of method-level and line-level prediction of our method is better than the two baselines.
% }

% Through our extensive evaluations of \tool in both method- and line-level predictions, we conclude that \tool's neural bug detectors are more precise in capturing the semantic buggy patterns than the two other methodologies. Compared to the CFG method, the superior performance \tool displays is entirely due to the interval-based propagation model, which demonstrates a better generalization of GGNN. As for AST methods, \tool uses a more semantic and principle graph representation to facilitate GGNN for learning deeper and more complicated semantic features.

\paragraph{Investigating models scalability}
We divide the entire test set into ten subsets, each of which consists of graphs of similar size. We then investigate how models perform on each subset starting from the smallest to the largest graphs. We fix the depth of inlining to be 2, which provides the largest variation among all graphs in terms of the size. Figure~\ref{fig:scaf} depicts the F1 score for \tool and the baseline under top-3 prediction mode (top-1 and top-5 yield similar results). Initially, \tool achieves slightly better results on the subset of small graphs; later as the size of graphs increases, \tool is significantly more resilient with its prediction than the baseline. Overall, we conclude bug detectors built out of \tool are more scalable.

\begin{figure*}
\begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{Precision in predicting NPE.}
\centering
\begin{tikzpicture}[scale=0.92]
   \begin{axis}[
    xmax=100,xmin=0,
    ymin=0,ymax=0.7,
    xlabel=\emph{Graph Size},ylabel=\emph{Top-3 F1 Score},
    xtick={0,20,40,...,100},
    ytick={0,0.1,0.20,...,0.7},
    xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}\%},
    ]
     \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(5, 0.481) (15, 0.385) (25, 0.288) (35, 0.256) (45, 0.256) (55, 0.163) (65, 0.156) (75, 0.127) (85, 0.070) (95, 0.027)};
     \addplot coordinates{(5, 0.388) (15, 0.294) (25, 0.350) (35, 0.309) (45, 0.303) (55, 0.266) (65, 0.275) (75, 0.244) (85, 0.149) (95, 0.073)};   
    \legend{\emph{Baseline},\emph{\tool}}
    \end{axis}
    \end{tikzpicture}
     ~%
    % %
    \subcaption{}
\label{fig:scaf}
\end{minipage}
\begin{minipage}{.33\textwidth}
% \captionsetup{skip=1pt}
% \caption{F1 score in predicting NPE.}
\centering
\begin{tikzpicture}[scale=0.92]
   \begin{axis}[
    xmax=120,xmin=0,
       ymin=0,ymax=0.4,
    xlabel=\emph{Training Time (Minutes)},ylabel=\emph{Average Test F1 for NPE},
    % xtick={0,4,8,...,20},
    xtick={0,30,60,90,120},
    ytick={0,0.1,0.20,...,0.4},
    xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}},
   ]
   
    %  \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(0, 0.177) (7.5, 0.171) (15, 0.165) (22.5, 0.165) (30, 0.165) (37.5, 0.141) (45, 0.193) (52.5, 0.168) (60, 0.174) (67.5, 0.168) (75, 0.153) (82.5, 0.193) (90, 0.186) (97.5, 0.180) (105, 0.156) (112.5, 0.186) (120, 0.165) (127.5, 0.162) (135, 0.199) (142.5, 0.165) (150, 0.171)};
    %  \addplot coordinates{(0, 0.245) (7.5, 0.253) (15, 0.270) (22.5, 0.291) (30, 0.304) (37.5, 0.279) (45, 0.287) (52.5, 0.300) (60, 0.291) (67.5, 0.291) (75, 0.283) (82.5, 0.274) (90, 0.296) (97.5, 0.274) (105, 0.287) (112.5, 0.287) (120, 0.287) (127.5, 0.287) (135, 0.291) (142.5, 0.287) (150, 0.283)};
     \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(0, 0.1)  (15, 0.123)  (30, 0.129) (45, 0.137)  (60, 0.169)  (75, 0.167)  (90, 0.174)  (105, 0.19)  (120, 0.191)  (135, 0.239)  (150, 0.24)};
     \addplot coordinates{(0, 0.117)  (15, 0.185)  (30, 0.204)  (45, 0.232) (60, 0.252)  (75, 0.255)  (90, 0.255)  (105, 0.256)  (120, 0.255) (135, 0.412) (150, 0.41)};
     \legend{\emph{Baseline}, \emph{\tool}}
    \end{axis}
    \end{tikzpicture}%
    ~%
\subcaption{}
\label{fig:ttf}
\end{minipage}
\begin{minipage}{.33\textwidth}
\vspace{4pt}
% \captionsetup{skip=1pt}
% \caption{Recall in predicting NPE.}
\centering
\begin{tikzpicture}[scale=0.92]
  \begin{axis}[
  % x tick label style={/pgf/number format/1000 sep=},
    ymin=0,ymax=0.7,
    xlabel=\emph{Number of First Order Intervals}, ylabel=\emph{Top-3 F1 Score},
    xtick=data,
    xticklabels={1,2,...,6,7+},
    ybar,
    bar width=6pt,
    ytick pos=left,
    xtick style={draw=none},
    xticklabel style={yshift=.75ex},
    legend image code/.code={
        \draw [#1] (0cm,-0.1cm) rectangle (0.2cm,0.25cm); },
  ]

  \addplot [black!30!white,fill=black!30!white] coordinates {
  (1, 0.257) (2, 0.215) (3, 0.183) (4, 0.173) (5, 0.116) (6, 0.115) (7, 0.074)
  };
  \addplot [black!100!white,fill=black!100!white] coordinates {
  (1, 0.352) (2, 0.288) (3, 0.259) (4, 0.291) (5, 0.102) (6, 0.159) (7, 0.107)
  };
  \legend{\emph{w/o IBPM},\emph{\tool}}
  \end{axis}
\end{tikzpicture}%
    ~%
    %
\subcaption{}
% \caption{ss}
\label{fig:intf}
\end{minipage}
\caption{Experiment results.}
\end{figure*}

% \begin{figure*}
% \centering
%   \begin{tikzpicture}[scale=0.92]
%   \begin{axis}[
%     xmax=100,xmin=0,
%       ymin=0,ymax=0.7,
%     xlabel=\emph{Graph Size},ylabel=\emph{Top-1 F1 Score},
%     xtick={0,20,40,...,100},
%     ytick={0,0.1,0.20,...,0.7},
%     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}\%},
%   ]
   
%      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(5, 0.547) (15, 0.435) (25, 0.209) (35, 0.281) (45, 0.294) (55, 0.209) (65, 0.175) (75, 0.194) (85, 0.080) (95, 0.035)};
%      \addplot coordinates{(5, 0.443) (15, 0.357) (25, 0.285) (35, 0.459) (45, 0.487) (55, 0.353) (65, 0.297) (75, 0.416) (85, 0.201) (95, 0.112)};    
%      \legend{\emph{Baseline}, \emph{\tool}}
%     \end{axis}
%     \end{tikzpicture}%
%     ~%
%     %
%     \begin{tikzpicture}[scale=0.92]
%   \begin{axis}[
%     xmax=100,xmin=0,
%     ymin=0,ymax=0.7,
%     xlabel=\emph{Graph Size},ylabel=\emph{Top-3 F1 Score},
%     xtick={0,20,40,...,100},
%     ytick={0,0.1,0.20,...,0.7},
%     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}\%},
%     ]
%      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(5, 0.481) (15, 0.385) (25, 0.288) (35, 0.256) (45, 0.256) (55, 0.163) (65, 0.156) (75, 0.127) (85, 0.070) (95, 0.027)};
%      \addplot coordinates{(5, 0.388) (15, 0.294) (25, 0.350) (35, 0.309) (45, 0.303) (55, 0.266) (65, 0.275) (75, 0.244) (85, 0.149) (95, 0.073)};   
%     \legend{\emph{Baseline},\emph{\tool}}
%     \end{axis}
%     \end{tikzpicture}%
%     ~%
%     %
%      \begin{tikzpicture}[scale=0.92]
%   \begin{axis}[
%     xmax=100,xmin=0,
%     ymin=0,ymax=0.7,
%     xlabel=\emph{Graph Size},ylabel=\emph{Top-5 F1 Score},
%     xtick={0,20,40,...,100},
%     ytick={0,0.1,0.20,...,0.70},
%     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}\%},
%     ]
    
%      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(5, 0.440) (15, 0.328) (25, 0.249) (35, 0.225) (45, 0.241) (55, 0.121) (65, 0.135) (75, 0.106) (85, 0.060) (95, 0.030)};
%      \addplot coordinates{(5, 0.343) (15, 0.280) (25, 0.337) (35, 0.304) (45, 0.302) (55, 0.228) (65, 0.202) (75, 0.207) (85, 0.115) (95, 0.069)};   
%      \legend{\emph{Baseline},\emph{\tool}}
%      \end{axis} 
%      \end{tikzpicture}
%     \caption{Investigating the scalability of all models.}
%     \label{fig:sca}
% \end{figure*}

\paragraph{Measuring training efficiency}
Since all models make instantaneous predictions (\eg around 800 examples per second), we only measure the training speed of \tool and the baseline. Again, we fix the depth of inlining to be 2, which presents the biggest challenges in training efficiency. Figure~\ref{fig:ttf} shows the \textit{test} F1 score (average across top-1, 3 and 5 prediction modes) over training time for \tool and the baseline on null pointer dereference bugs (Other two bug types are much easier to train). \tool's bug detector achieves results that are as 50\% as good as its final results under half an hour, and results that are as 95\% as good under 1 hour, while both being substantially higher than the best results of the baseline models. Our model achieves its best results around the 1 hour mark.



% Table \ref{tab:lineres} presents the top-N recall of the line-level prediction results. We choose N to be 1, 3, 5, 7, and 10 for 
% multiple prediction configurations. As before, we highlight the highest top-N recall for each methodology across all bug types. Overall, \tool outperforms the baslines in most metrics. Specifically, for array index out of bound bugs, \tool yields significantly better models than AST and CFG methods in each top-N configuration. However, the improvement \tool made over the baselines is not as significant as that in method-level prediction, especially in dealing with class cast bugs where AST method outperforms \tool in certain configurations. The last column shows average top-N recall performance among all three bug types. \tool achieves almost 60\% in top-3 and more than 70\% in top-5 recall, which is still notably better than the two other methodologies. Figure~\ref{fig:largeGraphLine} depicts the top-3 recall across the graph size. Similar to the method-level prediction, \tool shows bigger improvement over the baselines on the top 10\% largest graphs. 

% \begin{table}[!t]
% \centering
% \normalsize
% \caption{Training time.}
% \adjustbox{max width=\columnwidth}{\begin{tabular}{c|ccc|ccc|ccc}
% \hline
%  \multirow{2}{*}{\tabincell{c}{Method//\#Inline}} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{AIOE} & \multicolumn{3}{c}{CCE}\\
% \cline{2-10}
%         & 0 & 1 & 2 & 0 & 1 & 2& 0 & 1 & 2  \\\hline
% Baseline & 4 &	11.3 & 	37.8 & 0.9 &	1.9 &	6.4 & 0.7 &	1.9 &	7.5   \\\hline
% CFG & 0.9 &	1.4 &	12 &  0.2 &	0.4 &	2.2 & 0.2 &	0.3 &	2.1   \\\hline
% \hline
% \tool & 20.7 &	39.3 &	51.7 & 4.5 &	8.1 &	10.2 & 4.3 &	7.8 &	9.4  \\\hline % FP should *3?

% \end{tabular}}
% \label{tab:sats}
% \end{table}

\subsection{Contribution of IBPM}
We aim to precisely quantify IBPM's contribution to the learning capacity of the GNN. In particular, we re-implement \tool by replacing its IBPM with the standard propagation mechanism. In other words, we perform a head-to-head comparison between the two propagation mechanisms while the rest of the model architecture is held the same. Figure~\ref{fig:intf} shows how the test F1 scores of both configurations vary with the number of first order intervals in top-3 prediction mode (top-1 and top-5 yield similar results). For the same reason, the depth of inlining is fixed to be 2. Given the same number of the first order intervals, IBPM performs better than the standard propagation mechanism across the board. Apart from the apparent scalability advantage IBPM displays over the standard propagation mechanism, IBPM achieves better results even when the number of intervals is small, thanks to its exploitation of the program-specific graph characteristics.  



\subsection{Futher Evaluation of \tool}
In general, static analyzers can be classified into two categories: soundy and unsound. The former refers to tools that are sound by design but make unsound choices for utility concerns, whereas the latter is often built out of pattern matching techniques that do not concern themselves with soundness. Intending to cover both flavors, we pick soundy tools: 
Facebook Infer~\cite{calcagno2015moving,berdine2005smallfoot}, Pinpoint~\cite{shi2018pinpoint} and BugPicker, and another unsound tool: SpotBugs (the successor of FindBugs~\cite{Hovemeyer2004}).

We emphasize that our work makes no claims of advancing the theory of sound static analysis, therefore this experiment solely focuses on studying the utility of each tool in practice. 
% In other words, we present empirical evidence to demonstrate \tool's strength compared with other static analysis tools. 
We examine the performance of each checker in catching null pointer dereference bugs, which happen to be the only type of bugs all tools support.


% This section compares \tool against traditional 
% static analyzers. As a conceptual advantage, we re-emphasize 
% that creating neural bug finders based on \tool does not require the substantial amount of human-expertise that is needed to build 
% classical static analyzers. Sufficient amount of training data is 
% all \tool needs. Besides, \tool also allows an easier extension to 
% support new types of bugs compared to static analyzers. 

% To compare the actual performance between \tool and static 
% analyzers in catching real world, complex and semantic bugs, 
% we pick Facebook Infer~\cite{calcagno2015moving}, arguably the state-of-the-art static analyzer supporting Java program language. 

% We compare \tool against and Infer in catching null pointer dereference bugs, which happen to be the only type of bugs both \tool and Infer support.

% Ideally, we would like to use all bugs in our test set for the experiment, however, doing so would require a substantial amount of manual work. As for each bug in the test set, we need to pull from the repository the right version of the source code at which the bug has a presence, and subsequently analyze the report produced by each static analysis tool. 

To keep the engineering load manageable, we randomly pick 75 bugs out of seven projects from defect4j and bugs.jar, two most studied datasets in bug detection literature. Later we discover Infer does not have access to the build tools that are required to compile some of the projects in defect4j. Therefore, we show Infer's performance only on the projects it can compile. Those projects contain 58 bugs in total, namely Bug Set I.

First, we manually verify the validity, and more importantly, the location for all 75 bugs in case any bug may trigger an exception at a different location than developers' fix.
% to prevent any tool from being unfairly disadvantaged. For example, if a developer's fix does not exactly correlate to the program location where exceptions are thrown, we will manually add another buggy label to the location in addition to the point of fix committed by developers. In the end, we annotated six more buggy locations which adds up to 81 in total. 
Next, we feed the entire codebase of each project for each checker to scan. A report that points to a buggy location will be counted as a true positive, otherwise, it's a false positive. We acknowledge that a static analysis tool could have caught a real bug that is mistakenly counted as a false positive since it falls out of the 75 bugs we collected, however, the exact same issue applies to \tool, which we regrettably ignore due to resource constraint. We use \tool with depth 2 of inlining trained in the previous experiment. It is configured to run the top-1 prediction mode. We choose the most precise analysis for Pinpoint to perform. We also manually fine-tune BugPicker (\eg increase the length of the call chain or reset the timeout), but obtain the same results. We do not manage to run any other configuration for Infer and SpotBugs rather than their default set up. 

Table~\ref{tab:sats} depicts the results. Overall, we find (1) \tool achieves better precision and recall than any other evaluated tool; more importantly, (2) bugs that are found by competing tools are all caught by \tool. Besides, \tool detects another 11 bugs that are missed by the other tools.

% shows the performance of each bug finder\footnote{We also provide the details of the comparison in the supplemental material.}, and we interpret and analyze the results below.


% nitially, we collected all null pointer dereference bugs from all of our testing projects.
% Later we excluded the bugs from some of the projects that other tools do not manage to compile. For example, Infer does not have access to the build tools that are required to compile the projects in defect4j.
% \footnote{Some projects require build tools such as those provided by defects4j that Infer does not have access to.} 
% In the end we have 58 null pointer dereference bugs from Lang, Math, Flink, Closure, Wicket and Mockito, against which we show the performance of each bug finder in Table~\ref{tab:sats}. Below we interpret and analyze the results we obtain.

% \begin{itemize}%[leftmargin=*]
%     \item Each column records the number of detected bugs (denoted by TP), missed bugs (denoted by FN) and false warnings (denoted by FP) for each tool on the two bug sets. Overall, \tool achieves better precision and recall than any other evaluated tool.
%     % (we provide a breakdown for the performance of each checker on each project in the supplemental material)
%     % \item We have manually verified the validity, and more importantly the location for each of the 79 bugs to prevent any tool from being unfairly disadvantaged. For example, if a developer's fix does not exactly correlate to the program location where exceptions are thrown, we will manually add another buggy label to the location in addition to the point of fix registered by developers.
    
%     \item We use \tool with depth 2 of inlining trained in the previous experiment. It is configured to run top-1 prediction mode. We choose the most precise analysis for Pinpoint to perform. We also manually fine tune BugPicker (\eg increase the length of call chain or reset the timeout), but obtain no improvement. We do not manage to run any other configuration for Infer and SpotBugs rather than their default set up.
    
%     \item All bugs that are found by Infer and Pinpoint are also caught by \tool. In addition, \tool detects another 13 bugs that are missed by Infer and Pinpoint.
    
%     % \item In general, we found that unsound tools (\eg SpotBugs and BugPicker) produce less warnings but miss more bugs than soundy tools (\eg Infer and Pinpoint). \tool produces comparable amount of warnings to unsound tools, and catches far more bugs than any evaluated tool. 
    
% \end{itemize}

\begin{table}[!t]
\centering
\normalsize
\caption{Results of the comparison. TP, FP, FN stand for true positives, false positives and false negatives respectively.}
\adjustbox{max width=\columnwidth}{\begin{tabular}{c|ccc|ccc|cc}
\hline
 \multirow{2}{*}{\tabincell{c}{Tools}} & \multicolumn{3}{c|}{Bug Set I} & \multicolumn{3}{c|}{Remaining Set} & \multicolumn{2}{c}{Total}\\
\cline{2-9}
         & TP & FP & FN & TP & FP & FN  & Precision & Recall   \\\hline
FB Infer & 4 & 1004 & 54 & NA & NA & NA & .004 & .069    \\\hline
Pinpoint & 4 & 1524 & 54 & 3 & 1104 & 14 & .003 & .093   \\\hline
SpotBugs & 0 & 107 & 58 & 1 & 26 & 16 & .007 & .013   \\\hline
BugPicker & 0 & 79 & 58 & 0 & 0 & 17 & 0 & 0   \\\hline
\hline
\textbf{\tool} & \textbf{16} & \textbf{1655} & \textbf{42} & \textbf{5} & \textbf{521} & \textbf{12} & \textbf{.010} & \textbf{.280}  \\\hline %top-1
% \textbf{\tool} & \textbf{22} & \textbf{4414} & \textbf{33} & \textbf{8} & \textbf{1579} & \textbf{13} & \textbf{.005} & \textbf{.379}  \\\hline %top-3
%\textbf{\tool} & \textbf{25} & \textbf{136} & \textbf{33} & \textbf{6} & \textbf{34} & \textbf{11} & \textbf{.154} & \textbf{.413}  \\\hline % FP should *3?

\end{tabular}}
\label{tab:sats}
\end{table}

% On those projects, Infer reports 1008 null pointer dereference bugs in total. After manually verifying the reports according to the ground truth, we confirm that Infer detects only one of them. In comparison, \tool is able to detect 42 buggy methods with 138 warnings. With the top-3 prediction mode at the line-level, \tool achieves 71.4\% recall, in other words, by scanning three lines in each buggy method, developers are able to precisely locate 30 out of the 58 bugs.

% Worth noting we only validate Infer's report according to the existing bugs, it is possible that Infer detects potentially unknown bugs. In other words, there might have been true bugs contained in the 1008 warnings reported by Infer. However, since \tool and Infer use the same ground truth, it is equally possible that other bugs reported by \tool may also be true positives.

% Apart from the practical benefits \tool yields, we believe \tool also enjoys several conceptual advantages over the competing static analysis tools. First, given the framework \tool provides, creating a static bug finder can be simplified to solving a machine learning task. In comparison, traditional way of designing static analysis tools even the unsound ones requires substantial amount of human expertise. Besides, unlike the static analysis tools, model-based bug detectors can benefit from increasingly large datasets and powerful training regime, as a result, they will evolve and get better over time.

%The result shows that \tool is comparable to Infer in detecting NPE bugs.
%However, building a new bug detector in \tool does require expertise on static analysis or verification.
%Developers only need to collect data for the new bug and define a reasonable representation for it, which is easier than writing a program analysis tool.

We have also applied \tool to catch bugs in the wild, and obtained encouraging results. Configured with top-1 prediction mode and inline depth of 2 (we also tried 3 and 4 for smaller methods), \tool found \rBugs bugs (40 NPE and 10 AIE) in 17 projects that are among the 
most starred on GitHub. All bugs are manually verified and reported to developers, out of which \fBugs are fixed and another \cBugs are confirmed (fixes pending). Our findings show that not only does \tool significantly improve the prior works, but more importantly, \tool is a industry-strength static tool in checking real-world Java projects.

\subsection{Discussion on Limitation of \tool}
In order to gain a deeper understanding of \tool's limitation, we mainly look into the bugs \tool missed in the prior experiment. We find that when bug patterns are not local, that is, the dereference is quite distant from where a null pointer is assigned, \tool tends to struggle, in particular, it even misclassifies the method to be clean most of the time. The reason is, as one can imagine, \tool's signal gets diluted when a scattered bug pattern is overwhelmed by irrelevant statements in a program. We plan to tackle this issue with both program analysis and machine learning techniques. For data pre-processing, program slicing~\cite{Weiser1981} seems to be a promising idea. Given the location of a potential null pointer dereference (due to the null assignment or non-initialization), we can filter out statements that fall out of the slice to localize a bug pattern. On the other hand, a larger, more diverse dataset that contains a variety of bug patterns should also help, or for data augmentation, we can synthesize new programs by randomly adding dummy statements in between the assignment and dereference of null pointer for buggy methods, especially when the high-quality, large-scale public datasets are unavailable.

Another issue we discovered is \tool is less accurate when handling large programs (\ie approximately 1,000 nodes in the graph) despite the contribution IBPM makes to the underlying GNN. We find several bugs \tool missed where the bug patterns are in fact local. We believe this is due to the fundamental limitation of GNN, which requires deeper insight and understanding of the models themselves, without which, IBPM's results will be hard to improve upon in a qualitative manner.

We also briefly examine the false positives \tool emitted. For a few dozen we inspected, we find that the same issue causing \tool to miss bugs are also major sources of \tool's imprecision. In addition, \tool can be over-sensitive about the presence of null pointers, albeit we can not confirm they are never dereferenced.



% To evaluate the performance of \tool in detecting unknown bugs, we apply \tool on open-source projects. 
% For bugs reported by \tool, we manually verify them and report them to developers.
% In total, we report 193 bugs, 13 of them are confirmed, 7 of them are fixed and remainings are waiting for confirmation. 
% Specifically, we report 107 NPE bugs and 86 AIE bugs in 23 projects. 11 NPE bugs and 2 AIE bugs are confirmed. 5 NPE bugs are fixed and 2 AIE bugs are fixed.
% It is worth noting that some bugs can be grouped into one according to their root cause. For example, a method that returns null may have multiple call sites, which use the null value. AIE bugs can also be grouped in the similar way.
% The number of reported bugs is the number of bugs without group.


% \ignore{

% The section aims at evaluating the precision of infer by detecting known bugs.
% We evaluated infer on 25 projects with 58 known NPE bugs from the dataset we used.
% Infer reports 1008 null pointer dereference bugs.
% After manually verifying the reports and comparing them with the known bugs, we found that infer detects 1 of them.
% In comparison, \tool is able to detect NPE bugs with 72.1\% recall.
% \wyc{\tool detects 24 bugs base on top-3 prediction, which reports 282 warnings methods in total.
% If we use top-5 prediction, then we are able to pinpoint 28 bugs.
% }


% It is worth noting that we only validate bugs related to known bugs, there is a chance that Infer detects unknown bugs among the 1008 bug reports.
% In other words, other bugs reported by Infer may also be true positives.
% However, both two tools use the same ground truth, which means that other bugs reported by \tool may also be true positives.

% The result shows that \tool is comparable to Infer in detecting NPE bugs.
% However, building a new bug detector in \tool does require expertise on static analysis or verification.
% Developers only need to collect data for the new bug and define a reasonable representation for it, which is easier than writing a program analysis tool.
%}

% \ignore{
% \subsection{Performance on top N\% largest graphs}

% \begin{table*}[!t]
% \centering
% \small
% \caption{F1 score on top N\% largest graphs}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
%  Bug types & \multicolumn{4}{c|}{\tool} & \multicolumn{4}{c|}{CFG} & \multicolumn{4}{c|}{AST} \\
% \cline{2-13}
% & 20\% & 30\% & 40\% & 50\%  &20\% & 30\% & 40\% & 50\%  & 20\% & 30\% & 40\% & 50\% \\\hline
% NPE & 724 &  721 & 775 & 769 & 744 &  789 & 729 & 729 &  667 & 636 & 627 & 694  \\\hline
% \end{tabular}
% \label{tab:lineres}
% \end{table*}



% \begin{table*}[!t]
% \centering
% \small
% \caption{Performance on line-level prediction}
% \begin{tabular}{c|c|ccc|ccc|ccc}
% \hline
%  \multirow{2}{*}{\tabincell{c}{Methods}} & \multirow{2}{*}{Top-N} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{AIOE} & \multicolumn{3}{c}{CCE} \\
% \cline{3-11}
% &  & Precision & Recall & F1 & Precision & Recall & F1  & Precision & Recall & F1  \\\hline
% \multirow{5}{*}{AST} & Top-1 & 37.8 & 37.8 & 37.8 & 28.6 & 28.6 & 28.6 & \textbf{66.7} & \textbf{66.7} & \textbf{66.7} \\\cline{2- 11}
% & Top-3 & \textbf{22.3} & 55.0 & \textbf{31.7} & 12.7 & 35.7 & 18.7 & \textbf{26.4} & 66.7 & \textbf{37.8} \\\cline{2- 11}
% & Top-5 & \textbf{16.9} & 64.0 & \textbf{26.8} & 8.7 & 39.3 & 14.2 & \textbf{22.4} & \textbf{81.0} & \textbf{35.1} \\\cline{2- 11}
% & Top-7 & \textbf{14.7} & 72.1 & \textbf{24.4} & 6.9 & 42.9 & 11.9 & \textbf{19.4} & \textbf{85.7} & \textbf{31.6} \\\cline{2- 11}
% & Top-10 & \textbf{13.0} & 80.2 & \textbf{22.3} & 7.7 & 64.3 & 13.7 & \textbf{18.5} & \textbf{95.2} & \textbf{31.0} \\\hline
% \multirow{5}{*}{CFG} & Top-1 & \textbf{47.7} & \textbf{47.7} & \textbf{47.7} & 32.1 & 32.1 & 32.1 & 52.4 & 52.4 & 52.4 \\\cline{2- 11}
% & Top-3 & 18.6 & 55.9 & 27.9 & 15.5 & 46.4 & 23.2 & 22.2 & 66.7 & 33.3 \\\cline{2- 11}
% & Top-5 & 13.7 & 61.3 & 22.4 & 9.6 & 46.4 & 16.0 & 16.8 & 76.2 & 27.6 \\\cline{2- 11}
% & Top-7 & 11.7 & 67.6 & 19.9 & 8.7 & 57.1 & 15.2 & 13.6 & 76.2 & 23.0 \\\cline{2- 11}
% & Top-10 & 10.7 & 79.3 & 18.8 & 7.2 & 64.3 & 12.9 & 14.1 & \textbf{95.2} & 24.5 \\\hline
% \hline
% \multirow{5}{*}{\tool} & Top-1 & 44.1 & 44.1 & 44.1 & \textbf{35.7} & \textbf{35.7} & \textbf{35.7} & 47.6 & 47.6 & 47.6 \\\cline{2- 11}
% & Top-3 & 19.2 & \textbf{57.7} & 28.8 & \textbf{16.7} & \textbf{50.0} & \textbf{25.0} & 23.8 & \textbf{71.4} & 35.7 \\\cline{2- 11}
% & Top-5 & 15.1 & \textbf{67.6} & 24.7 & \textbf{14.8} & \textbf{71.4} & \textbf{24.5} & 17.9 & \textbf{81.0} & 29.3 \\\cline{2- 11}
% & Top-7 & 12.6 & \textbf{73.0} & 21.5 & \textbf{11.5} & \textbf{75.0} & \textbf{19.9} & 14.4 & 81.0 & 24.5 \\\cline{2- 11}
% & Top-10 & 11.0 & \textbf{82.0} & 19.5 & \textbf{8.4} & \textbf{75.0} & \textbf{15.1} & 14.1 & \textbf{95.2} & 24.5 \\\hline
% \end{tabular}
% \label{tab:lineresold}
% \end{table*}


% \begin{table*}[!t]
% \caption{Top-N recall for line-level prediction.}
% \centering
% \small
% \begin{tabular}{c|c|c|c|c|c}
% \hline
%  \tabincell{c}{Methods} & Top-N & NPE & AIOE & CCE & Avg. \\\hline
% \multirow{5}{*}{AST} & Top-1 & 37.8 & 28.6 & \textbf{66.7} & \textbf{44.4} \\\cline{2-6}
% & Top-3 & 55.0 & 35.7 & 66.7 & 52.5 \\\cline{2-6}
% & Top-5 & 64.0 & 39.3 & \textbf{81.0} & 61.4 \\\cline{2-6}
% & Top-7 & 72.1 & 42.9 & \textbf{85.7} & 66.9 \\\cline{2-6}
% & Top-10 & 80.2 & 64.3 & \textbf{95.2} & 79.9 \\\hline
% \multirow{5}{*}{CFG} & Top-1 & \textbf{47.7} & 32.1 & 52.4 & 44.1 \\\cline{2-6}
% & Top-3 & 55.9 & 46.4 & 66.7 & 56.3\\\cline{2-6}
% & Top-5 & 61.3 & 46.4 & 76.2 & 61.3 \\\cline{2-6}
% & Top-7 & 67.6 & 57.1 & 76.2 & 67.0 \\\cline{2-6}
% & Top-10 & 79.3 & 64.3 & \textbf{95.2} & 79.6 \\\hline
% \hline
% \multirow{5}{*}{\tool} & Top-1 & 44.1 & \textbf{35.7} & 47.6 & 42.5 \\\cline{2-6}
% & Top-3 & \textbf{57.7} & \textbf{50.0} & \textbf{71.4} & \textbf{59.7} \\\cline{2-6}
% & Top-5 & \textbf{67.6} & \textbf{71.4} & \textbf{81.0} & \textbf{73.3} \\\cline{2-6}
% & Top-7 & \textbf{73.0} & \textbf{75.0} & 81.0 & \textbf{76.3} \\\cline{2-6}
% & Top-10 & \textbf{82.0} & \textbf{75.0} & \textbf{95.2} & \textbf{84.1} \\\hline
% \end{tabular}
% \label{tab:lineres}
% \end{table*}



% \begin{figure}
% \centering
% \begin{minipage}{.45\textwidth}
%   \centering
%   \includegraphics[width=.95\linewidth]{Figures/perCmp.pdf}
%   \captionof{figure}{Method-level prediction.}
%   \label{fig:perCmp}
% \end{minipage}%
% \begin{minipage}{.45\textwidth}
%   \centering
%   \includegraphics[width=.95\linewidth]{Figures/linef1Comp.png}
%   \captionof{figure}{Top-N recall of line-level prediction.}
%   \label{fig:linef1Comp}
% \end{minipage}
% \end{figure}


% \begin{table}
% 	\begin{minipage}{.43\textwidth}
% 		\centering
% 		\includegraphics[width=1\linewidth ]{Figures/perCmp.pdf}
% 		\captionof{figure}{Average precision, recall and F1 for method-level prediction.}
%         \label{fig:perCmp}
% 	\end{minipage}\hfill
% 	\begin{minipage}{.55\textwidth}
% 		\caption{Top-N recall for line-level prediction.}
% 		\centering
% 		\adjustbox{max width=1\textwidth}{

% 		\begin{tabular}{c|c|c|c|c|c}
% \hline
%  \tabincell{c}{Methods} & Top-N & NPE & AIOE & CCE & Avg. \\\hline
% \multirow{5}{*}{AST} & Top-1 & 37.8 & 28.6 & \textbf{66.7} & \textbf{44.4} \\\cline{2-6}
% & Top-3 & 55.0 & 35.7 & 66.7 & 52.5 \\\cline{2-6}
% & Top-5 & 64.0 & 39.3 & \textbf{81.0} & 61.4 \\\cline{2-6}
% & Top-7 & 72.1 & 42.9 & \textbf{85.7} & 66.9 \\\cline{2-6}
% & Top-10 & 80.2 & 64.3 & \textbf{95.2} & 79.9 \\\hline
% \multirow{5}{*}{CFG} & Top-1 & \textbf{47.7} & 32.1 & 52.4 & 44.1 \\\cline{2-6}
% & Top-3 & 55.9 & 46.4 & 66.7 & 56.3\\\cline{2-6}
% & Top-5 & 61.3 & 46.4 & 76.2 & 61.3 \\\cline{2-6}
% & Top-7 & 67.6 & 57.1 & 76.2 & 67.0 \\\cline{2-6}
% & Top-10 & 79.3 & 64.3 & \textbf{95.2} & 79.6 \\\hline
% \hline
% \multirow{5}{*}{\tool} & Top-1 & 44.1 & \textbf{35.7} & 47.6 & 42.5 \\\cline{2-6}
% & Top-3 & \textbf{57.7} & \textbf{50.0} & \textbf{71.4} & \textbf{59.7} \\\cline{2-6}
% & Top-5 & \textbf{67.6} & \textbf{71.4} & \textbf{81.0} & \textbf{73.3} \\\cline{2-6}
% & Top-7 & \textbf{73.0} & \textbf{75.0} & 81.0 & \textbf{76.3} \\\cline{2-6}
% & Top-10 & \textbf{82.0} & \textbf{75.0} & \textbf{95.2} & \textbf{84.1} \\\hline
% \end{tabular}}
% \label{tab:lineres}
% 	\end{minipage}
% \end{table}


% }

\ignore{

\begin{figure*}
\centering
\begin{tikzpicture}[scale=0.92]
  \begin{axis}[
  % x tick label style={/pgf/number format/1000 sep=},
    ymin=0,ymax=0.7,
    xlabel=\emph{Number of First Order Intervals}, ylabel=\emph{Top-1 F1 Score},
    xtick=data,
    xticklabels={1,2,...,6,7+},
    ybar,
    bar width=6pt,
    legend image code/.code={
        \draw [#1] (0cm,-0.1cm) rectangle (0.2cm,0.25cm); },
  ]

  \addplot [black!30!white,fill=black!30!white] coordinates {
  (1, 0.297) (2, 0.220) (3, 0.202) (4, 0.213) (5, 0.058) (6, 0.095) (7, 0.044) 
  };
  \addplot [black!100!white,fill=black!100!white] coordinates {
  (1, 0.358) (2, 0.310) (3, 0.233) (4, 0.397) (5, 0.076) (6, 0.154) (7, 0.213)
  };
  \legend{\emph{w/o IBPM},\emph{\tool}}
  \end{axis}
\end{tikzpicture}%
    ~%
    %
\begin{tikzpicture}[scale=0.92]
  \begin{axis}[
  % x tick label style={/pgf/number format/1000 sep=},
    ymin=0,ymax=0.7,
    xlabel=\emph{Number of First Order Intervals}, ylabel=\emph{Top-3 F1 Score},
    xtick=data,
    xticklabels={1,2,...,6,7+},
    ybar,
    bar width=6pt,
    legend image code/.code={
        \draw [#1] (0cm,-0.1cm) rectangle (0.2cm,0.25cm); },
  ]

  \addplot [black!30!white,fill=black!30!white] coordinates {
  (1, 0.257) (2, 0.215) (3, 0.183) (4, 0.173) (5, 0.116) (6, 0.115) (7, 0.074) 
  };
  \addplot [black!100!white,fill=black!100!white] coordinates {
  (1, 0.352) (2, 0.288) (3, 0.259) (4, 0.291) (5, 0.102) (6, 0.159) (7, 0.107)
  };
  \legend{\emph{w/o IBPM},\emph{\tool}}
  \end{axis}
\end{tikzpicture}%
    ~%
    %
\begin{tikzpicture}[scale=0.92]
  \begin{axis}[
  % x tick label style={/pgf/number format/1000 sep=},
    ymin=0,ymax=0.7,
    xlabel=\emph{Number of First Order Intervals}, ylabel=\emph{Top-5 F1 Score},
    xtick={1,2,...,7},
    xticklabels={1,2,...,6,7+},
    ybar,
    bar width=6pt,
    legend image code/.code={
        \draw [#1] (0cm,-0.1cm) rectangle (0.2cm,0.25cm); },
  ]

  \addplot [black!30!white,fill=black!30!white] coordinates {
  (1, 0.215) (2, 0.182) (3, 0.136) (4, 0.138) (5, 0.090) (6, 0.114) (7, 0.048) 
  };
  \addplot [black!100!white,fill=black!100!white] coordinates {
  (1, 0.326) (2, 0.269) (3, 0.228) (4, 0.219) (5, 0.099) (6, 0.163) (7, 0.071)
  };
  \legend{\emph{w/o IBPM},\emph{\tool}}
  \end{axis}
\end{tikzpicture}
    \caption{Comparing IBPM against the standard propagation. \wyc{(11+ represent graphs with more than 11 intervals.)}}
    \label{fig:pm}
     
\end{figure*}


% \begin{figure*}
% \centering
%   \begin{tikzpicture}[scale=0.92]
%   \begin{axis}[
%     xmax=20,xmin=0,
%       ymin=0,ymax=0.7,
%     xlabel=\emph{Training Time (Minutes)},ylabel=\emph{F1 Score for NPE},
%     xtick={0,4,8,...,20},
%     ytick={0,0.1,0.20,...,0.7},
%     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}},
%   ]
   
%      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{(0, 0.177) (1, 0.171) (2, 0.165) (3, 0.165) (4, 0.165) (5, 0.141) (6, 0.193) (7, 0.168) (8, 0.174) (9, 0.168) (10, 0.153) (11, 0.193) (12, 0.186) (13, 0.180) (14, 0.156) (15, 0.186) (16, 0.165) (17, 0.162) (18, 0.199) (19, 0.165) (20, 0.171)};
%      \addplot coordinates{(0, 0.245) (1, 0.253) (2, 0.270) (3, 0.291) (4, 0.304) (5, 0.279) (6, 0.287) (7, 0.300) (8, 0.291) (9, 0.291) (10, 0.283) (11, 0.274) (12, 0.296) (13, 0.274) (14, 0.287) (15, 0.287) (16, 0.287) (17, 0.287) (18, 0.291) (19, 0.287) (20, 0.283)};    
%      \legend{\emph{Baseline}, \emph{\tool}}
%     \end{axis}
%     \end{tikzpicture}%
%     ~%
%     %
%     \begin{tikzpicture}[scale=0.92]
%   \begin{axis}[
%     xmax=7,xmin=0,
%     ymin=0,ymax=0.7,
%     xlabel=\emph{Training Time (Minutes)},ylabel=\emph{F1 Score for AIOE},
%     xtick={0,1,2,...,7},
%     ytick={0,0.1,0.20,...,0.7},
%     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}},
%     ]
%      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{ (0, 0.176) (1, 0.196) (2, 0.098) (3, 0.157) (4, 0.196) (5, 0.176) (6, 0.137) (7, 0.157) (8, 0.118) (9, 0.137) (10, 0.157) (11, 0.157) (12, 0.157) (13, 0.098)};
%      \addplot coordinates{ (0, 0.256) (1, 0.256) (2, 0.320) (3, 0.288) (4, 0.256) (5, 0.288) (6, 0.320) (7, 0.288)};   
%     \legend{\emph{Baseline},\emph{\tool}}
%     \end{axis}
%     \end{tikzpicture}%
%     ~%
%     %
%      \begin{tikzpicture}[scale=0.92]
%   \begin{axis}[
%     xmax=10,xmin=0,
%     ymin=0,ymax=0.7,
%     xlabel=\emph{Training Time (Minutes)},ylabel=\emph{F1 Score for CCE},
%     xtick={0,1,2,...,10},
%     ytick={0,0.1,0.20,...,0.70},
%     xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}},
%     ]
%      \addplot+ [mark=pentagon*,mark size=2.5pt,every mark/.append style={}] coordinates{ (0, 0.319) (1, 0.223) (2, 0.191) (3, 0.223) (4, 0.287) (5, 0.255) (6, 0.255) (7, 0.191) (8, 0.255) (9, 0.319) (10, 0.191) (11, 0.191)};
%      \addplot coordinates{(0, 0.223) (1, 0.260) (2, 0.335) (3, 0.335) (4, 0.297) (5, 0.335) (6, 0.409) (7, 0.372) (8, 0.372) (9, 0.297) (10, 0.335) (11, 0.372) (12, 0.260)};   
%      \legend{\emph{Baseline},\emph{\tool}}
%      \end{axis} 
%      \end{tikzpicture}
%     \caption{Training time.}
%     \label{fig:tt}
     
% \end{figure*}
}

==> GGNN_paper-(submission)/Sections/Implementation.tex <==
% !TeX root = ../ggnn.tex

\section{Implementation}\label{sec:impl}
%Using GGNNs for sets of large, diverse graphs requires some engineering effort, as efficient batching is hard in the presence of diverse shapes.  An important observation is that large graphs are normally very sparse, and thus a representation of edges as an adjacency list would usually be advantageous to reduce memory consumption. In our case, this can be easily implemented using a sparse tensor representation, allowing large batch sizes that exploit the parallelism of modern GPUs efficiently. 
%A second key insight is to represent a batch of graphs as one large graph with many disconnected components. This just requires appropriate pre-processing to make node identities unique. As this makes batch construction somewhat CPU-intensive, we found it useful to prepare minibatches on a separate thread. Our TensorFlow (Abadi et al., 2016) implementation scales to 55 graphs per second during training and 219 graphs per second during test-time using a single NVidia GeForce GTX Titan X with graphs having on average 2,228 (median 936) nodes and 8,350 (median 3,274) edges and 8 GGNN unrolling iterations, all 20 edge types (forward and backward edges for 10 original edge types) and the size of the hidden layer set to 64. The number of types of edges in the GGNN contributes proportionally to the running time. For example, a GGNN run for our ablation study using only the two most common edge types (NextToken, Child) achieves 105 graphs/second during training and 419 graphs/second at test time with the same hyperparameters. Our (generic) implementation of GGNNs is available at https://github.com/Microsoft/ gated-graph-neural-network-samples, using a simpler demonstration task.

 we run the state-of-the-art clone detector, DECKARD \cite{4222572}, to pick a non-buggy method that is syntactically closest to each buggy method we collect.
 
 
The code extraction, construction of control flow graph and intervals are implemented based on Spoon~\cite{pawlak:hal-01169705}, which is an open-source library for Java source code transformation and analysis.

All neural bug detectors are implemented in Tensorflow. All RNNs built in the model have 1 recurrent layer with 100 hidden units. We adopt random initialization for weight initialization. Each token in the vocabulary is embedded into a 100-dimensional vector. We train the neural bug detectors using the Adam optimizer~\cite{kingma2014adam}. All experiments are performed on a 3.7GHz i7-8700K machine with 32GB RAM and NVIDIA GTX 1080 GPU.


==> GGNN_paper-(submission)/Sections/Interval.tex <==
\section{Interval-Based Propagation Mechanism}
\label{sec:ibpm}

In this section, we present the Interval-Based Propagation Mechanism (IBPM), a new protocol that regulates how nodes exchange messages with their peers in a graph. In particular, we highlight the conceptual advantages IBPM enjoys over the existing propagation mechanism.

\subsection{IBPM's Algorithm for Graph Propagation}
\label{subsec:IBPM}

We discuss two major issues existing works that apply GNN in program analysis suffer from. 

Even though GNN has shown its generality by succeeding in a variety of problem domains (\eg scene graph generation~\cite{8099813}, traffic prediction~\cite{li2017diffusion}, recommendation system~\cite{Ying:2018}, \etc), it can benefit from specializations designed to address the uniqueness of each problem setting, especially when dealing with programs, a fundamentally different data structure. However, prior works made little adjustment to accommodate such program-specific graph characteristics, resulted in a potential loss of model precision. Besides, scalability challenges can also hinder the generalization of GNN. That is when a graph has a large diameter; information has to be propagated over long distance, therefore, message exchange between nodes that are far apart becomes difficult. 

IBPM is designed specifically to tackle the aforementioned weaknesses of GNN. To start with, programs are represented by their control flow graphs. More distinctively, propagation is only allowed on a subgraph defined by an interval. Since iteration statements (\ie loops) often determines the formation of intervals (because loop back edge \eg node 7 to node 2 in Figure~\ref{fig:interval} cuts off the loop header into a new interval), IBPM, in essence, attends to such loop structures when propagating on a control-flow graph. To enable the message-exchange between nodes that are far apart, IBPM switches onto a higher order graph, as such, involving more nodes to communicate within the same interval. On the other hand, by reducing the order of graph, IBPM restores the location propagation, and eventually recovers the node embeddings on the original control flow graph. 
% To elevate the propagation from local to global mode, we increase the order of control flow graphs to enable the message exchange among nodes across the entire graph. 
Below we use the program in Figure~\ref{fig:ibpm}, a function that computes the starting indices of the substring \texttt{s1} in string \texttt{s2}, and its control-flow graph in Figure~\ref{fig:interval} to explain how IBPM works.

\lstset{style=mystyle}
\begin{figure*}
        \centering
        \begin{tikzpicture}
        \matrix[matrix of nodes, 
        nodes={anchor=center},
        column sep=-1em,
        row sep = -.5em]{%
        {%
        \setlength{\fboxsep}{1.5pt}%
        \setlength{\fboxrule}{.5pt}%
        \fbox{\hspace{3pt}\includegraphics[width=0.28\textwidth]{Figures/intervals1.png}\hspace{6.1pt}}%
        }%
            &
            \thinspace\thinspace%\enspace
            \includegraphics[width=0.03\textwidth]{Figures/Picture1.png}
            &\thinspace\thinspace%\enspace
            {%
                \setlength{\fboxsep}{2.6pt}%
                \setlength{\fboxrule}{.5pt}%
                \fbox{\hspace{3.5pt}\includegraphics[width=0.28\textwidth]{Figures/intervals2.png}\hspace{5.2pt}}%
             }            
             &
            \thinspace\thinspace%\enspace
            \includegraphics[width=0.03\textwidth]{Figures/Picture1.png}
            \thinspace
            &
            {%
                \setlength{\fboxsep}{5pt}%
                \setlength{\fboxrule}{.5pt}%
                \fbox{\hspace{1.5pt}\includegraphics[width=0.28\textwidth]{Figures/intervals3.png}\hspace{2pt}}%
             }
             \\
            \begin{minipage}[t][8ex][t]{0.28\textwidth}
            \subcaption{Propagation among node 3, 4, 5 and 6 on the first order graph.\label{fig:fog}}
            \end{minipage}
            &&
            \begin{minipage}[t][8ex][t]{0.3\textwidth}
            \subcaption{Propagation among node 2, 7 and 8 on the second order graph.\label{fig:sog}}
            \end{minipage}%
            &&
            \begin{minipage}[t][8ex][t]{0.3\textwidth}
            \subcaption{Propagation among node 1 and 9 on the third order graph.\label{fig:tog}}
            % \quad\quad\quad\quad\quad\quad\bigupArrow
            \end{minipage}%
            \\    
            \vspace{-1cm}
            \begin{minipage}[t]{0.28\textwidth}
            	\lstinputlisting[linewidth=5.1cm,xleftmargin=-0.4em,xrightmargin=0em,framexleftmargin=0em]{Codes/IBPM1.java}
            \end{minipage}
            &
            \thinspace\thinspace
            \includegraphics[width=0.03\textwidth]{Figures/arrowd.png}
            &
            \begin{minipage}[t]{0.28\textwidth}
            	\lstinputlisting[linewidth=5.4cm,xleftmargin=0.55em,xrightmargin=0em,framexleftmargin=0em]{Codes/IBPM2.java}
            \end{minipage}
            &
            %\enspace\thinspace
            \includegraphics[width=0.03\textwidth]{Figures/arrowd.png}
            &
            \begin{minipage}[t]{0.28\textwidth}
            	\lstinputlisting[linewidth=5.3cm,xleftmargin=0.15em,xrightmargin=0em,framexleftmargin=0em]{Codes/IBPM3.java}
            \end{minipage}
            \\
            \begin{minipage}[t][7ex][t]{0.28\textwidth}
            \subcaption{Illustration of IBPM on the first order graph using example program.\label{fig:tran1}}
            % \quad\quad\quad\quad\quad\quad\bigdownArrow
            \end{minipage}
            &&
            \begin{minipage}[t][7ex][t]{0.28\textwidth}
            \subcaption{Illustration of IBPM on the second order graph using example program.\label{fig:tran2}}
            \end{minipage}%
            &&
            \begin{minipage}[t][7ex][t]{0.28\textwidth}
            \subcaption{Illustration of IBPM on the third order graph using example program.\label{fig:tran3}}
            \end{minipage}%
            \\%[4pt]
        };
        \end{tikzpicture}
        \caption{Interval-Based Propagation Mechanism.\label{fig:ibpm}}
    \end{figure*}

Depicted in Figure~\ref{fig:fog}, IBPM starts with the first order graph (\ie the original control flow graph). As explained earlier, we restrict communication among nodes within the same interval. Consequently, node 3, 4, 5 and 6 will freely pass messages to the neighbors along their directed edges. On the contrary, node 1 and 2, which are alone in their respective intervals, will not contact any other node in the graph. Such propagation that occurs internal to an interval is carried out in the same manner as the standard propagation (Equation~\ref{equ:h}). Figure~\ref{fig:tran1} highlights the part of the example program that corresponds to the only active interval in the current step of IBPM. Apparently, IBPM focuses on learning from the inner loop while leaving the rest of the program unattended. 

We then move onto the second order graph as shown in Figure~\ref{fig:sog}. Recall how a second order graph is derived. We compute a new node (\ie node 8) to replace the only active interval on the first order graph (\ie node 3, 4, 5 and 6). Equation~\ref{equ:merge} defines how to initialize node 8 or any other node that is created when IBPM transitions from lower-order to higher-order graphs.
\begin{equation}\label{equ:merge}
\mu^{(0)}_{w} = \sum_{\mathclap{v \in I^{i}(h)}} \alpha_{v}\mu^{(l)}_{v}
\end{equation}

where $w$ denotes the node created out of the interval $I^{i}(h)$ and $\alpha_{v}$ is defined by 
\begin{equation}\label{equ:weight}
\alpha_{v} = \frac{exp\,(\mu^{(l)}_{v})}{\sum\limits_{\mathclap{v \in I^{i}(h)}} exp\,(\mu^{(l)}_{v})}         
\end{equation}

% \sum_{\mathclap{v \in I^{i}(h)}} exp(\mu^{(l)}_{v})

Due to the same restriction IBPM imposes, propagation on the second order graph now covers node 2, 7 and 8. Because node 8 can be deemed as a proxy of node 3-6, this propagation, in essence, covers all but node 1 on the first order graph. In other words, even though propagation is always performed within each interval, increasing the order of a graph implicitly expands the region of an interval, therefore facilitating more nodes to communicate. For visualization, Figure~\ref{fig:tran2} highlights the part of the program---the nested loop structure---IBPM attends to at the current step.
% represented by the only active interval on the second order graph in Figure~\ref{fig:tran2}. Apparently, IBPM gradually transitions from local to global mode by covering the entire nested loop structure. 

Figure~\ref{fig:tog} shows the third step of IBPM, where propagation spans across the entire graph. Upon completion of the message-exchange between node 1 and 9, IBPM transitions back to the lower order graphs; interval nodes will be split back into the multitude of nodes from which they formed (\eg node 9 to node 2, 7 and 8; node 8 to node 3-6). Equation below defines how to compute the initial embeddings for a node that is split from an interval. $\mu_{w}$ and $\alpha_{v}$ denote the same meaning in Equation~\ref{equ:merge}.
\begin{equation*}\label{equ:split}
\mu^{(0)}_{v} = \alpha_{v}\mu^{(l)}_{w}
\end{equation*}

Eventually, the node embeddings on the original control flow graph will be recovered. Worth mentioning recurring local propagation on the lower order graphs improves the accuracy of node embeddings by incorporating the previously accumulated global graph knowledge on the higher order graphs. In return, more precise modeling of the subgraphs also benefits the further global propagation across the entire graph. As the transitioning between local and global mode repeats, node embeddings will continue to be refined to reflect the properties of a graph.

\subsection{Comparing IBPM to Standard Propagation}
% In this section, we explain in details why IBPM is advantageous over the standard propagation mechanism. 

\paragraph{\textbf{Structured Propagation}}
As described in Section~\ref{subsec:IBPM}, IBPM works with a graph hierarchy, where each level attends to distinct, important code constructs in a program, such as the loops illustrated in Figure~\ref{fig:tran1} and~\ref{fig:tran2}. This is in stark contrast with the standard propagation mechanism, where program structure is largely ignored and messages spread across the entire graph. Intuitively, we believe by utilizing the program constructs to regulate the message exchange, IBPM improves the precision of GNN in learning program properties.

\paragraph{\textbf{Scalable Propagation}}
We prove in theory IBPM also enjoys scalability advantage over the standard propagation mechanism. By scalability, we mean the number of messages that have been passed in total until the graph is sufficiently propagated. Since determining the threshold of sufficient propagation is beyond the scope of this paper, we make reasonable approximations to assist our proof. For simplicity, we assume directed, connected graphs which consist of distinct nodes and homogeneous edges, and synchronous message passing scheme in all definitions, theorems, and proofs.  

\begin{definition}{(Distance)}
\label{def:dis}
Given two nodes $v_{i}$ and $v_{j}$ on a graph $\mathcal{G}$, their distance, denoted by $\theta(v_{i},v_{j})$, is the length of the shortest path from $v_{i}$ to $v_{j}$ on $\mathcal{G}$.
% that consists of the least number of edges.
\end{definition}

\begin{definition}{(Diameter)}
\label{def:dia}
The diameter of a graph $\mathcal{G}$, $\pi(\mathcal{G})$, is the longest distance between any two nodes on $\mathcal{G}$. Assuming $\mathcal{V}$ is the set of nodes on $\mathcal{G}$.
\end{definition}
\begin{equation*}
\pi(\mathcal{G}) = \!\!\!\maxx_{v_{i},v_{j} \in \mathcal{V}} \! \! \!  \theta(v_{i},v_{j})        
\end{equation*}

\noindent
We define the point of sufficient propagation as follows.

\begin{definition}{(Fixed Point)}
\label{def:fp}
Given a graph $\mathcal{G}\! =\! (\mathcal{V}, \mathcal{E})$, associate each node $v \in \mathcal{V}$ with a set $\sigma_{v}$, which is initialized to contain the node itself, denoted by $\sigma_{v}^{0} = \{v\}$. After the $l$-th round of message passing, $\sigma_{v}^{l}$ is updated to $\bigcup_{u \in \mathcal{N}(v)} \sigma_{u}^{l-1}$, where $\mathcal{N}(v)$ refers to the neighbouring nodes of $v$. The propagation is said to reach the fixed point on $\mathcal{G}$ after $l$-th round of message passing iff (1) $\forall l^{\prime}\geq l,\, \forall v \in \mathcal{V},\, \sigma_{v}^{l} = \sigma_{v}^{l^{\prime}}$; and (2) $\nexists l^{\prime}<l,\, \forall l^{\prime\prime}\geq l^{\prime},\, \forall v \in \mathcal{V},\, \sigma_{v}^{l^{\prime}} = \sigma_{v}^{l^{\prime\prime}}$.
\end{definition}

% \theoremstyle{definition}
% \begin{assumption}{(Distinctiveness)} \label{assume:dis}
% Assume, without the loss of generality, that nodes on a graph $\mathcal{G}\! =\! (\mathcal{V}, \mathcal{E})$ are distinct. Formally, $\nexists v_{i} \in \mathcal{V} ,\nexists v_{j} \in \mathcal{V}, v_{i} \ne v_{j} \wedge \sigma_{v_{i}}^0 \cap \sigma_{v_{j}}^0 \neq \emptyset$.
% \end{assumption}\ke{why is this a reasonable assumption}
% \begin{assume}[Distinctiveness]
% Hereinafter, we assume, without the loss of generality, that nodes on $\mathcal{G}$ are distinct. Formally, $\nexists v_{i} \in \mathcal{V} ,\nexists v_{j} \in \mathcal{V}, v_{i} \ne v_{j} \wedge \sigma_{v_{i}}^0 \cap \sigma_{v_{j}}^0 \neq \emptyset$.
% \end{assume}

% Hereinafter, we assume, without the loss of generality, that nodes on $\mathcal{G}$ are distinct. Formally, $\nexists v_{i} \in \mathcal{V} ,\nexists v_{j} \in \mathcal{V}, v_{i} \ne v_{j} \wedge \sigma_{v_{i}}^0 \cap \sigma_{v_{j}}^0 \neq \emptyset$.

\begin{theorem}[Distance Measure]
\label{the:dm}
Given two nodes $v_{i}$ and $v_{j}$ on a graph (hereinafter assuming all edges are of unit length), if $\sigma_{v_{j}}$ contains $v_{i}$ only after the $l$-th round of message passing, that is $\,\,\forall l^{\prime}<l,\, v_{i} \notin \sigma_{v_{j}}^{l^{\prime}}$ and $\, \forall l^{\prime}\geq l,\, v_{i} \in \sigma_{v_{j}}^{l^{\prime}}$, then $\theta(v_{i},v_{j}) = l$.
\end{theorem}

\begin{proof}
Assume otherwise \st $\theta(v_{i},v_{j}) = l^{\prime} \wedge l \neq l^{\prime}$. Synchronous message passing system in essence enumerates all possible paths between any two nodes on the graph. In particular, all paths of length $l$ will be enumerated in $l$-th round of message passing. If $\theta(v_{i},v_{j}) = l^{\prime}$, then $l^{\prime}$ rounds would have been needed, after which $\sigma_{v_{j}}$ contains $v_{i}$, which contradicts the assumption $\sigma_{v_{j}}$ contains $v_{i}$ after the $l$-th round of message passing.
\end{proof}

\begin{theorem}[Scalability Measure]
\label{the:sm}
Given a graph $\mathcal{G}\! =\! (\mathcal{V}, \mathcal{E})$, the number of messages that have been sent by all nodes in $\mathcal{V}$ until the propagation reaches fixed point on $\mathcal{G}$ equals to $\pi(\mathcal{G})\, * \lvert \mathcal{E} \rvert$.
\end{theorem}

\begin{proof}
Because synchronous message passing system has $\lvert \mathcal{E} \rvert$ message sent in each round on directed graphs. So it suffices to prove that $\pi(\mathcal{G})$ rounds of message passing are needed until propagation reaches the fixed point. Assume otherwise, reaching the fixed point on $\mathcal{G}$ takes $l^{\prime}$ rounds:

(a)  $l^{\prime} > \pi(\mathcal{G})$. This indicates $\exists v_{i} \in \mathcal{V}, \, \exists v_{j} \in \mathcal{V}, \, \forall l^{\prime\prime}<l^{\prime},\, v_{i} \notin \sigma_{v_{j}}^{l^{\prime\prime}} \wedge v_{i} \in \sigma_{v_{j}}^{l^{\prime}}$. According to Theorem~\ref{the:dm}, then $\theta(v_{i},v_{j}) = l^{\prime}$. Since $l^{\prime} > \pi(\mathcal{G})$, therefore contradicting the Definition~\ref{def:dia}. 

(b) $l^{\prime} < \pi(\mathcal{G})$. This indicates $\nexists v_{i} \in \mathcal{V}, \nexists v_{j} \in \mathcal{V}, \nexists l^{\prime\prime} > l^{\prime}, \forall l^{\prime\prime\prime}<l^{\prime\prime}, v_{i} \notin \sigma_{v_{j}}^{l^{\prime\prime\prime}} \wedge v_{i} \in \sigma_{v_{j}}^{l^{\prime\prime}}$. According to Theorem~\ref{the:dm}, then $\nexists v_{i} \in \mathcal{V}, \nexists v_{j} \in \mathcal{V}, \nexists l^{\prime\prime} > l^{\prime}, \theta(v_{i},v_{j}) = l^{\prime\prime}$, and therefore $l^{\prime} \geq \pi(\mathcal{G})$, which contradicts the assumption $l^{\prime} < \pi(\mathcal{G})$.
% As explained above, synchronous message passing system enumerates all paths of length $l$ in $l$-th round of message passing. This indicates $\exists v_{i} \in \mathcal{V}, \, \exists v_{j} \in \mathcal{V}, \, \theta(v_{j},v_{i})=\pi(\mathcal{G}) \wedge v_{j} \notin \sigma_{v_{i}}^{l^{\prime}}$, therefore contradicting the Definition~\ref{def:fp}.
\end{proof}

% We modify Definition~\ref{def:fp} to fit IBPM. 
\noindent
Similarly, we define the saturation point of IBPM.

\begin{definition}{(Fixed Point for IBPM)}
\label{def:fpI}
Given the first order graph $\mathcal{S}^1$, and successively derived higher order graphs, $\mathcal{S}^2,\mathcal{S}^3,...,\mathcal{S}^n$ ($\mathcal{S}^n$ represents the highest order graph), propagation transitions from $\mathcal{S}^i$ to $\mathcal{S}^{i+1}$ (or $\mathcal{S}^{i-1}$) only after the fixed point on all intervals in $\mathcal{S}^i$ has been reached (according to the Definition~\ref{def:fp}). In addition, $\sigma_{v^{i+1}}^{0}$ of a new node $v^{i+1}$ on $\mathcal{S}^{i+1}$ is initialized to $\bigcup_{u \in I^{i}(v)} \sigma_{u}^{l}$, where $I^{i}(v)$ denotes the interval from which $v^{i+1}$ is created, and $l=\pi(I^{i}(v))$. As for a new node $v^{i-1}$ on $\mathcal{S}^{i-1}$, $\sigma_{v^{i-1}}^{0}$ is initialized to $\{v^{i-1}\}$. The whole process is said to reach fixed point iff the propagation successively transitions from $\mathcal{S}^{1}$ to $\mathcal{S}^{n}$ and back to $\mathcal{S}^{1}$, on which subsequent propagation also reaches fixed point.
\end{definition}%$l^{u}$ denotes the number of rounds after which the propagation reaches fixed point on $I^{i}(v)$

\begin{theorem}[Scalability Measure for IBPM]
\label{the:smI}
Given $\mathcal{S}^1,\mathcal{S}^2$, $...,\mathcal{S}^n$ and their respective member intervals $I^1(h_{1}^{1}),...,I^1(h_{\,\rule{.4pt}{1.2ex} \mathcal{S}^{1} \rule{.4pt}{1.2ex}}^{1})$; $I^2(h_{1}^{2}),...,I^2(h_{\,\rule{.4pt}{1.2ex} \mathcal{S}^{2} \rule{.4pt}{1.2ex}}^{2})$; $I^n(h_{1}^n),...,I^n(h_{\,\rule{.4pt}{1.2ex} \mathcal{S}^{n} \rule{.4pt}{1.2ex}}^{n})$, the number of messages that have been sent until IBPM reaches fixed point equals to 
\begin{equation}\label{equ:ibpmsca}
\bigg( \sum_{j=1}^{n-2} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} 2 * \pi(I^{j}(h^{j}_{i})) * \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert \bigg) + \pi(\mathcal{S}^{n-1}) * \lvert \mathcal{E}_{\mathcal{S}^{n-1}} \rvert
\end{equation}

\noindent if $\mathcal{S}^{n}$ is a single node, otherwise
\begin{equation*}
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\bigg( \sum_{j=1}^{n-1} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} 2 * \pi(I^{j}(h^{j}_{i})) * \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert \bigg)  + \pi(\mathcal{S}^{n}) * \lvert \mathcal{E}_{\mathcal{S}^{n}} \rvert
\end{equation*}
\noindent $\mathcal{E}_{g}$ denotes the set of edges in $g$ in both formulas.

% on $\mathcal{S}^1$, $\mathcal{S}^2$,...,\,$\mathcal{S}^n$ equals to $\sum_{j=1}^{n-2} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} 2 * \pi(I^{j}(h^{j}_{i})) * \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert + \pi(\mathcal{S}^{n-1}) * \lvert \mathcal{E}_{\mathcal{S}^{n-1}} \rvert$ if $\lvert \mathcal{E}_{\mathcal{S}^{n}}\rvert = 0$, where $\mathcal{E}_{g}$ denotes the edge set of $g$, otherwise $\sum_{j=1}^{n-1} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} 2 * \pi(I^{j}(h^{j}_{i})) * \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert + \pi(\mathcal{S}^{n}) * \lvert \mathcal{E}_{\mathcal{S}^{n}} \rvert$.
\end{theorem}
% 
\begin{proof}
Break IBPM into sub-propagation on each interval at each order of graph. Therefore, the number of messages sent in total can be computed by summing up the messages sent during each sub-propagation. Since all assumptions still hold,
% $\forall t \in [1,n], \nexists v_{i} \in \mathcal{V}_{\mathcal{S}^{t}}, \nexists v_{j} \in \mathcal{V}_{\mathcal{S}^{t}}, \sigma_{v_{i}}^{0} \cap \sigma_{v_{j}}^{0} \neq \emptyset$ ($\mathcal{V}_{\mathcal{S}^{t}}$ denotes the set of nodes on $\mathcal{S}^{t}$), 
Theorem~\ref{the:sm} can be applied to derive the proof.
\end{proof}

Below we compare the scalability of two propagation mechanism. First, we consider the case where $\mathcal{S}^{n}$ is a single node. Add another $\pi(\mathcal{S}^{n-1}) * \lvert \mathcal{E}_{\mathcal{S}^{n-1}} \rvert$ to Equation~\ref{equ:ibpmsca} leads to:
\begin{equation} \label{equ:deri1}
\setlength{\jot}{1pt} 
\begin{split}
&\!\!\!\!\!\bigg( \sum_{j=1}^{n-2} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} 2 * \pi(I^{j}(h^{j}_{i})) * \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert \bigg) + \pi(\mathcal{S}^{n-1}) * \lvert \mathcal{E}_{\mathcal{S}^{n-1}} \rvert < \\
&\!\!\!\!\!\bigg( \sum_{j=1}^{n-2} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} 2 * \pi(I^{j}(h^{j}_{i})) * \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert \bigg)  + 2 * \pi(\mathcal{S}^{n-1}) * \lvert \mathcal{E}_{\mathcal{S}^{n-1}} \rvert
\end{split}
\end{equation}

Absorb $2 * \pi(\mathcal{S}^{n-1}) * \lvert \mathcal{E}_{\mathcal{S}^{n-1}} \rvert$ into the sum at the right hand side of Equation~\ref{equ:deri1} gives
\begin{equation} \label{equ:deri2}
\setlength{\jot}{1pt} 
\begin{split}
\!\!\!\!\!&\bigg( \sum_{j=1}^{n-2} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} 2 * \pi(I^{j}(h^{j}_{i})) * \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert \bigg) + \pi(\mathcal{S}^{n-1}) * \lvert \mathcal{E}_{\mathcal{S}^{n-1}} \rvert < \\
\!\!\!\!\!&\sum_{j=1}^{n-1} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} 2 * \pi(I^{j}(h^{j}_{i})) * \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert
\end{split}
\end{equation}

To simply, assume 
% \begin{equation} \label{equ:deri3}
%      \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall j \in [1,n-1], \forall i \in [1,\lvert \mathcal{S}^{j} \rvert], \pi(I^{j}(h^{j}_{i}))=\tau
% \end{equation}
\[
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall j \in [1,n-1], \forall i \in [1,\lvert \mathcal{S}^{j} \rvert], \pi(I^{j}(h^{j}_{i}))=\tau 
\]

then
\begin{equation}\label{equ:deri3}
\!\!\!\!\!\sum_{j=1}^{n-1} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} 2 * \pi(I^{j}(h^{j}_{i})) * \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert
=
2 * \tau * \sum_{j=1}^{n-1} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert    
\end{equation}
% \[
% \!\!\!\!\!\!\!\!\!\!\!\sum_{j=1}^{n-1} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} 2 * \pi(I^{j}(h^{j}_{i})) * \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert
% =
% 2 * \tau * \sum_{j=1}^{n-1} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert
% \]

Because $\sum_{j=1}^{n-1} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert \leq \lvert \mathcal{E} \rvert$. In particular, the equivalence establishes when none of the intervals at any order of graph that has multiple exit edges to the same external node. So we derive

\begin{equation} \label{equ:deri4}
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!2 * \tau * \sum_{j=1}^{n-1} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert
\leq
2 * \tau * \lvert \mathcal{E} \rvert
\end{equation}

Linking Equation~\ref{equ:deri1}-\ref{equ:deri4}, we derive 

\begin{equation*}
\setlength{\jot}{2pt} 
\begin{split}
\!\!\!\!\!\!\!\!\!&\bigg( \sum_{j=1}^{n-2} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} 2 * \pi(I^{j}(h^{j}_{i})) * \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert \bigg) + \pi(\mathcal{S}^{n-1}) * \lvert \mathcal{E}_{\mathcal{S}^{n-1}} \rvert < \\
\!\!\!\!\!\!\!\!\!&2\tau * \lvert \mathcal{E} \rvert
\end{split}
\end{equation*}
% \[ 
% \sum_{j=1}^{n-2} \sum_{i=1}^{\lvert \mathcal{S}^{j} \! \rvert} 2 * \pi(I^{j}(h^{j}_{i})) * \lvert \mathcal{E}_{I^{j}(h^{j}_{i})} \rvert + \pi(\mathcal{S}^{n-1}) * \lvert \mathcal{E}_{\mathcal{S}^{n-1}} \rvert 
% <
% 2\tau * \lvert \mathcal{E} \rvert
% \]
Essentially, we have estimated an upper bound of the scalability measure for IBPM: $2\tau * \lvert \mathcal{E} \rvert$. The same upper bound can also be derived for the other case where $\mathcal{S}^{n}$ is not a single node. Comparing with Theorem~\ref{the:sm}'s result: $\pi(\mathcal{G}) * \lvert \mathcal{E} \rvert$, IBPM is more scalable than the standard propagation mechanism since the diameter of an interval is generally small (\ie around 2 on control flow graphs according to our large-scale evaluation). When the size of a graph increases, the size of an interval mostly stays as a constant, therefore IBPM outperforms the standard propagation by an even wider margin. Overall, using sensible approximations, we have proved IBPM is superior to the standard propagation in the scalability regard.









% propagation always happens at the level of intervals as the order graph increases/decreases, the propagation transitions from local to global naturally

% enables the nodes to be communicated thoroughly and efficiently across the entire graph, ultimately help GNN to converge.

% it recovers the lower order graph step by step. Worth mentioning the subsequent local propagation conducted at the level of intervals will be influenced by the global knowledge previously gained from the highest order of graph. 

==> GGNN_paper-(submission)/Sections/Introduction.tex <==
% !TeX root = ../ggnn.tex

\section{Introduction}\label{sec:Intro}

Static analysis is an effective technique to catch bugs early when they are cheap to fix.
% Static analysis is an important method for finding software defects. It's performed early in the development cycle to catch bugs as quickly as they appear, paving the way for easy fixes. 
Unlike dynamic analysis, static analysis reasons about every path in a program, offering formal guarantees for its run-time behavior. As an evidence of their increasing maturity and popularity, many static analyzers have been adopted by major tech companies to prevent bugs leaked to their production code. Examples include Google's Tricorder~\citep{Sadowski2015}, Facebook's Getafix~\citep{scott2019getafix} and Zoncolan, and Microsoft's Visual Studio IntelliCode.
% Examples include Microsoft's SLAM~\cite{Ball2002} Google's Error Prone~\cite{6392098}, Facebook's Infer~\cite{calcagno2015moving}, Coverity~\cite{Bessey2010} and Astr\'ee~\cite{Blanchet}.

Despite the significant progress, static analyzers suffer from several well-known issues. One, in particular, is the high false positive rate which tends to overshadow true positives and hurt usability. The reason for this phenomenon is well-known: all nontrivial program properties are mathematically
undecidable, meaning that automated reasoning of software generally must involve approximation. 
% grow larger, static analyzers choose to over approximate the program semantics to alleviate the scalability challenges, 
% which inevitably introduces imprecision (\eg errors flagged by static analyzers do not occur in reality). 
On the other hand, problems of false negatives also need to be dealt with. Recently,~\citet{Habib2018} investigated how effective the state-of-the-art static analyzers are in handling a set of real-world bugs. Habib~\etal show more than 90\% of the bugs are missed, exposing the severity of false negatives.

To tackle the aforementioned weaknesses, this paper explores an alternative approach to create static bug checkers---neural bug detection. Our observation is bug patterns exist even for those targeted by static analyzers. Therefore, machine learning techniques offer a viable solution. The challenge though is how to design a model that is effective in catching such bug patterns, which are non-trivial and can even be quite complex. Although Graph Neural Networks (GNN) have seen success across many program analysis tasks~\cite{li2015gated,allamanis2017learning,si2018learning}, they have been utilized only to catch specialized, relatively syntactic bugs in variable naming~\cite{allamanis2017learning}, hence limited impact. To elevate GNN's capability to a sufficient extent for detecting semantic bugs, we invent a novel, efficient propagation mechanism based on graph intervals. Our insight is specializing GNN to exploit the program-specific graph characteristics enhances their capacity of learning complex programming patterns. Specifically, our propagation mechanism forces GNN to attend to certain code constructs to extract deep, semantic program features. Moreover, our propagation mechanism operates on hierarchical graphs to alleviate the scalability issues GNN often encounters when learning from larger graphs.


We realize our approach into a framework, called \tool, that is general (\ie language-agnostic), and extensible (\ie not restricted to certain bug types). \tool performs inter-procedural analysis for bug finding. The framework first automatically scrapes training data across multiple project corpus, creating a large set of buggy and clean code examples; then trains a model to differentiate between these two; and finally uses the trained model for detecting bugs in previously unseen code. We present three neural bug detectors based on \tool targeting null pointer dereference, array index out of bound and class cast exceptions. Figure~\ref{fig:1}-\ref{fig:3} depict three real bugs (from the dataset introduced by~\citet{ye2014learning} and~\citet{just2014defects4j}) that are caught by our neural bug detectors. 
% Besides, we include the details of our further investigation in Figure~\ref{fig:b},~\ref{fig:d} and~\ref{fig:f}.
% In addition, we further probe \tool in an attempt to disclose its reasoning strategy for detecting each bug. Figure~\ref{fig:exa} describes in details the action we undertake and the results we obtain. 
In principle, extending \tool to create new bug detectors only requires the bug type information as the entire workflow will be automatically performed by \tool.
% a training data generator that extracts buggy code examples from a given code corpus, since the rest will be automatically performed by \tool. 
In theory, compared to the soundy static analysis tools~\cite{livshits2015defense}, our learner-based bug detectors are inherently unsound, 
% due to the nature of our methodology
however, their strength lies in their far lower cost of design (\ie no human expertise is required), 
% offers compelling benefits, among which the most prominent is a relatively static analysis tools, 
and comparable or even superior performance in practice.



\begin{figure}
    \centering
    \adjustbox{max width=.98\columnwidth}{
	\lstset{style=mystyle}
	\lstinputlisting[numbers=left,linewidth=8.5cm,framexleftmargin=8pt]{Codes/npe.java}}
	\caption{A null pointer dereference bug (bugs-dot-jar\_MNG-5613\_bef7fac6). The presence of the exception handling routine at line 9-10 indicates the function at line 4 may throw an exception, in which case the value of \texttt{projectDependencyGraph} is likely to be null; subsequently, a null pointer dereference will be triggered at line 7.}
    \label{fig:1}
\end{figure}

\begin{figure}
    \centering
    \adjustbox{max width=.98\columnwidth}{
	\lstset{style=mystyle}
	\lstinputlisting[numbers=left,linewidth=8.3cm,framexleftmargin=8pt]{Codes/index.java}}
	\caption{An array index out of bound bug (eclipse.jdt.ui-2f5e78c). Since the pre-incrementor at line 14 increments the value of \texttt{i} right before accessing the array \texttt{buffer}, an array index out of bound exception will be triggered in the iteration where \texttt{i} equals to \texttt{length}-1.}
    \label{fig:2}
\end{figure}

\begin{figure}
    \centering
    \adjustbox{max width=.98\columnwidth}{
	\lstset{style=mystyle}
	\lstinputlisting[numbers=left,linewidth=8.3cm,framexleftmargin=8pt]{Codes/cast.java}}
	\caption{An class cast bug (eclipse.jdt.ui-c0e0634). If \texttt{isInterface} (line 6) is evaluated to false, it's possible \texttt{parentType} is not an instance of \texttt{TypeDeclaration}, in which case a class cast exception will be triggered at line 11.}
    \label{fig:3}
\end{figure}
	

Our approach significantly differs from almost all related work in the literature~\cite{wang2016automatically,pradel2018deepbugs,allamanis2017learning}. Specifically, we consider deep and semantic bugs that are proven to be hard even for state-of-the-art static analyzers instead of shallow and syntactic bugs targeted by other works~\cite{wang2016automatically,allamanis2017learning,pradel2018deepbugs}. 
% In addition, our neural bug detectors are trained exclusively on the real world programs, which help them to be
% effective against complicated bugs in unseen code. 
% data set containing exclusively real programs written by developers. The quality of our training data helps \tool to create powerful static bug checkers that are 
Additionally, \tool pinpoints a bug in a program to a line instead of predicting an entire file to be buggy or not~\cite{wang2016automatically}.

We evaluate \tool by training its three instantiations on 30,000 methods extracted from hundreds of Java projects and detecting bugs in 1,700 methods from a different set of 13 Java projects. %28,344 files and searching bugs in another 73 projects containing 88,162 
In total, our corpus amounts to 1,047,296 lines. We find that all neural bug detectors are effective with each achieving above 35\% precision and 45\% recall. 

% We evaluate \tool by training its three instantiations on six Java projects consisting of 28,344 files and searching bugs in another 73 projects containing 88,162 Java files. In total our corpus amounts to 7,547,096 lines. We find that our neural bug detectors are effective, achieving above 38.9\% precision, 79.6\% recall and 52.2\% F1 score.
% In particular, when predicting at the level of methods, the three models yield on average 38.9\% precision, 79.6\% recall and 52.2\% F1 score, even at the level of lines, three models still achieve 73.3\% recall. 
% We also find out the neural bug detectors perform equally well in the within- and cross-project prediction. This finding indicates that bugs of the same kind display similar characteristics despite being authored by different developers. 
To further demonstrate the utility of \tool, we compare our neural bug detector with several static analysis tools (\eg Facebook's Infer~\cite{calcagno2015moving,berdine2005smallfoot}, Pinpoint~\cite{shi2018pinpoint}, \etc). Our comparison focuses on the performance of each checker in catching null pointer dereference bugs, the only kind of bugs that can be handled by all tools. Results show that our neural bug detector catches more bugs and produces less spurious warnings than any evaluated static analyzer. We have also applied our neural bug detectors to 17 popular projects on GitHub and discovered 50 new bugs, among which 9 have been fixed and 3 have been confirmed (fixes pending).

We make the following contributions:
\begin{itemize}
    \item We propose a deep neural network based methodology for building static bug checkers. Specifically, we utilize GNN to train a classifier for differentiating buggy code from correct code.
    \item  We propose a novel interval-based propagation model that significantly enhances the capacity of GNN in learning programming patterns.
    \item We design and implement a framework to streamline the creation of neural bug detectors
    % including automatic data preparation and model training. 
    The framework is open-sourced at \url{https://github.com/anonymoustool/NeurSA}.
    \item We publish our data set at \url{https://figshare.com/articles/datasets_tar_gz/8796677} for the three neural bug detectors we built based on \tool to aid the future research activity.
    \item We present the evaluation results showing our neural bug detectors are highly precise in detecting the semantic bugs in real-world programs and outperform many flagship static analysis tools including Infer in catching null pointer dereference bugs. 
\end{itemize}














==> GGNN_paper-(submission)/Sections/Methodology.tex <==
% !TeX root = ../NeurSA.tex

\section{Methodology}\label{sec:Meth}

This section presents three neural bug detectors we created based on \tool framework. The bug detectors address a diverse set of programming mistakes: null pointer dereference bugs, array index out of bound bugs, and class casting bugs. 

\subsection{Null Pointer Exception}

The first neural bug detector addresses null pointer exception (NPE for short), which is caused by dereferencing null pointer. The main challenge for static analyzers to catch them is to precisely analyze the points-to relations, which also can scale to large programs~\cite{shi2018pinpoint}. We made the following adjustments to our graph encoding to deal with the null pointer dereference bugs. 

First, given a method call, we explicitly inject its return type and the types of its arguments. Second, We add an entry of $\mathit{NULL}$ to the vocabulary. Finally, we perform value flow analysis~\cite{shi2018pinpoint, sui2012static} to extract the data dependency among variables, in particular, we introduce a unique type of edge, which describes the value flow for pointers exclusively. Since the backbone of our graph is a variant of control flow graph, all the dependency edges are added between statement nodes (containing the dependent variables) rather than the variable itself.  

\ignore{
To this end, we devise a novel representation of $\textit{NULL}$ and pointers. Our statement representation has incorporated with the type information.
However, it misses $\textit{NULL}$ information and the propagation along control flow graph.
To address null pointer exception, we design an approach extracts the following information:

\begin{itemize}
    \item The type information of callee is placed before (or after) the callee if it is a return type(or function arguments).
    \item The explicit vocabulary of $\mathit{NULL}$. One way of avoid null pointer exception is by adding pointer checks, ensure that a pointer is not null.
    \item The data dependence of a pointer, which tracks data flow of a pointer.
\end{itemize}

The node embedding for NPE is in form of $(..., \tau_{ret}, NI_{callee}, \tau_{arg1}, \tau_{arg2},...)$ where $\tau_{ret}$ is the type information of return value, $NI_{callee}$ is the node index.
We additionally add an entry of $\mathit{NULL}$ to the vocabulary.
Then, to leverage data dependence of a pointer, we introduce value flow graph \cite{shi2018pinpoint, sui2012static}.
Value flow analysis provides data dependency information to identify identifications for null pointer dereference.
Based on value flow graph, we introduce a new kind of edge from value flow for pointers.
Specifically, for each pointer, we analyze its data dependency graph.
Then for each edge in the graph, we locate the corresponding start node $v_s$ and end node $v_d$ in the interval graph and add a new edge from $v_s$ to $v_d$.}

\subsection{Array Index Out of Bound Exception}
Array index out of bound exception (AIOE for short) occurs when the index of an array falls out of the range [0,$n$-1] ($n$ is the length of the array). The main challenge of statically analyzing this bug is to precisely determine the array bound and the index value at compile time\cite{gao2016carraybound, gao2016bovinspector}. To address this challenge, we attempted the following. 

Given an array declaration, we inject the type and the length of the array into our graph encoding. Whenever an array is accessed, we also add the type of the index variable to the mix. Finally we connect the value flow edges between statements that contain array declarations and array access operations.

\ignore{
\begin{itemize}
    \item For each array, we incorporate the array and its size. Note that we abstract variables as type information, we insert a new field at the end of the type information, indicating the length of an array.
    \item The value of an array index. When accessing an array by index, explicitly highlight the array accessing by grouping the array and the index.
    \item The data dependence of an array to tracks data flow.
\end{itemize}


The node embedding for the definition of array index out of bound is in form of $(..., \tau_{array}, \tau_{length},...)$ where $\tau_{array}$ is the type information of return value, $\tau_{length}$ is an integer or variable that indicates length of the array.
For each array access point, the encoding is in form of $(..., \tau_{array}, \tau_{length},\tau_{index},...)$ where $\tau_{index}$ is the type information of the index.
Finally, we add value flow edges from the definition of an array to the use of the array.}
  
\subsection{Class Cast Exception}
Class cast exception (CCE for short) is thrown when the object is cast to a subclass of which it is not an instance. The challenge lies in analyzing the type of a variable, determining whether there is an inherent relation between the variable that is being cast and the target type the variable is cast to. To deal with the challenge, we take the following actions.

Given a cast operation, we explicitly encode the type of the variable to be cast, providing an opportunity for GGNN to check the compatibility between its actual type and target type to be cast to. In addition, we also add the value flow edges connecting the cast operation to all statements that contain other variables the variable depends on.

\ignore{
\begin{itemize}
    \item For the target type, we also extract the type information instead of only analyzing type information of variable.
    \item The data dependence of an array to tracks data flow.
\end{itemize}

The node embedding for type cast operation is in form of $(..., \tau_{cast\_type}, \tau_{var},...)$ where $cast\_type$ is the target type of cast operation and $var$ is the variable that to be cast.
The data dependence tracks variable type by adding value flow edges.
Note that this bug highly depends on the type of a variable and thus it is important to track its type.}




==> GGNN_paper-(submission)/Sections/Preliminary.tex <==
\section{Preliminary}\label{sec:Pre}

First, we revisit the definition of connected, directed graphs. Then we give a brief overview of interval~\cite{Allen:1970:CFA:800028.808479} and GNN~\cite{gori2005new}, which our work builds on.

\subsection{Graph}
A graph $\mathcal{G}\! =\! (\mathcal{V}, \mathcal{E})$ consists of a set of nodes $\mathcal{V} \!= \!\{v_1, ..., v_m\}$, and a list of directed edge sets $\mathcal{E} = (\mathcal{E}_1, . . . , \mathcal{E}_K)$ where $K$ is the total number of edge types and $\mathcal{E}_k$ is a set of edges of type $k$. $E(v_s, v_d, k), k\in(1,...,K)$ denotes an edge of type $k$ directed from node $v_s$ to node $v_d$. For graphs with only one edge type, $E$ is represented as $(v_s, v_d)$.

The immediate successors of a node $v_i$ (denoted as $\textit{post}\,(v_i)$) are all of the nodes $v_j$ for which $(v_i, v_j)$ is an edge in $\mathcal{E}$. The immediate predecessors of node $v_j$  (denoted as $\textit{pre}\,(v_j)$) are all of the nodes $v_i$ for which $(v_i, v_j)$ is an edge in $\mathcal{E}$. 

A path is an ordered sequence of nodes $(v_j,..., v_k)$ and their connecting edges, in which each $v_i$ $\in$ $\textit{pre}\,(v_{i+1})$ for $i \in (j,...,k-1)$. A closed path is a path in which the first and last nodes are the same. The successors of a node $v_i$ (denoted as $\textit{post}\,^{*}(v_i)$) are all of the nodes $v_j$ for which there exists a path from $v_i$ to $v_j$. The predecessors of a node $v_j$  (denoted as $\textit{pre}\,^{*}(v_j)$) are all of the nodes $v_i$ for which there exists a path from $v_i$ to $v_j$.


\subsection{Interval}
% subsection 1: Intervals 
% formalization follow (https://amturing.acm.org/p137-allen.pdf) to define graph, path, closed path, intervals

%Given a graph, we construct intervals based on the following definition \cite{allen1976program}:

Introduced by~\citet{Allen:1970:CFA:800028.808479},
%Given a node \textit{h} (stands for head node), 
an interval \textit{I(h)} is the maximal,
single entry subgraph in which \textit{h} is the only entry node
and all closed paths contain \textit{h}. The unique
interval node \textit{h} is called the interval head or simply the
header node. An interval can be expressed in terms of
the nodes in it: $I(h) = \{v_l, v_2, ... ,v_m\}. $

By selecting the proper set of header nodes, a graph can be partitioned into a set of disjoint intervals. An algorithm for such a partition is shown in Algorithm \ref{alg:intervals}. The key is to add to an interval a node only if all of whose immediate predecessors are already in the interval (Line \ref{li:w2} to \ref{li:s2}). The intuition is such nodes when added to an interval keep the original header node as the single entry of an interval. To find a header node to form another interval, a node is picked that is not a member of any existing intervals although it must have a (not all) immediate predecessor being a member of the interval that is just computed (Line \ref{li:w3} to \ref{li:s3}). We repeat the computation until reaching the fixed-point where all nodes are members of an interval.
 
%Note that for an interval $I(h)$,  it adds nodes whose all immediate predecessors are already in $I(h)$ (at line \ref{li:w2} to \ref{li:s2})
%After constructing $I(h)$, we add all nodes to $H$ if they meet the following condition: they are not already in $H$ and are not in $I(h)$ but have immediate predecessors in $I(h)$ (at lines \ref{li:w3} to \ref{li:s3}).
%Last, add $I(h)$ to $\mathcal{S}$ and repeat the procedure until $H$ is empty.



\begin{algorithm}[tbp]
\small
\caption{Finding intervals for a given graph} 
% \newline
% \textbf{Input}: Graph $\mathcal{G}$, Node set $\mathcal{V}$ \newline
% \textbf{Output}: Interval set $\mathcal{S}$
% }
\label{alg:intervals}
\raggedright
\KwIn {Graph $\mathcal{G}$, Node set $\mathcal{V}$}
\KwOut {Interval set $\mathcal{S}$}
// $v_0$ is the unique entry node for the graph

H = \{$v_0$\}\;
\While{$H \neq \emptyset$}
{
        // remove next $h$ from $H$
        
        h = H.pop()\;
        I(h) = \{h\}\;
        // only nodes that are neither in the current interval nor any other interval will be considered 
        
        
        \While{$\{v \in \mathcal{V} \,| \, v \notin I(h) \wedge \nexists s (s \in \mathcal{S} \wedge v \in s) \wedge  pre(v) \subseteq I(h)\} \neq \emptyset$\label{li:w2}}  
        {
           I(h) = I(h) $\cup$ \{ v \}\; \label{li:s2}
        }
        // find next headers
        
        \While{$\{v \in \mathcal{V}  \,| \, \nexists s_{1} (s_{1} \in \mathcal{S} \wedge v \in s_{1}) \, \wedge\!$ $\exists m_{1}, m_{2}$ $(m_{1}$ $\in$ $pre(v)$ $\wedge$ $m_{2} \in pre(v) \wedge m_{1} \in I(h) \wedge m_{2} \notin I(h)) \} \neq \emptyset \; \; \;$ \label{li:w3}}
%        $\exists v \in \mathcal{V}$ such that $v \notin H$ and 
%        $v \notin I(h)$ and   
%            $\exists m \in imme\_pred(v)$ such that $m \in I(h)$ \label{li:w3}}
        {
            H = H $\cup$ \{ v \}\; \label{li:s3}
        }
        $\mathcal{S}$ = $\mathcal{S}$ $\cup$ I(h)\;
}
\end{algorithm}

The intervals on the original graph 
are called the first order intervals denoted by 
$I^1(h)$, and the graph from which they were derived 
is called first order graph (also called the set 
of first order intervals) $\mathcal{S}^1$ \st 
$I^1(h) \in \mathcal{S}^1$. By making each first order 
interval into a node and each interval exit edge into 
an edge, the second order graph can be derived, from 
which the second order intervals can also be defined. 
The procedure can be repeated to derive successively 
higher order graphs until the n-th order graph consists 
of a single node\footnote{Certain graphs can't be reduced to single nodes.}. Figure~\ref{fig:interval} illustrates 
such a sequence of derived graphs. 

%As we can see that the result graph may also be reducible, thus, we refer $\mathcal{S}^i$ as the i-th order of graph. 
%For example, $I^1(h) \in \mathcal{S}^1$ means that the interval $I^1(h)$ is an element of the first order graph.
%Figure \ref{fig:interval} shows four interval graphs.
%For example, $G^1$ is the original graph, four intervals below $G^1$ are intervals computed based on $G^1$.
%Then, we construct $G^2$ according to $\{I^1(h), h \in \{1,2,3,7\}\}$ and repeat the way of constructing intervals.
%Finally, there is only one interval in $G^3$, which means that $G^4$ is only one node.

% \begin{figure}[t]
% %\centering
% \small
% \begin{lstlisting}[language=Java,showstringspaces=false,numbers=none, framexleftmargin=0pt]
% public int substringIndices(String s1, String s2, 
%     int maxTry){
%   int M = s1.length(); 
%   int N = s2.length();  
%   int i = 0, j = 0, res = 0, pos = 0;
%   do { 
%     if (pos != maxTry) {
%       do {
%         log("Begin at index: " + i);
%         if (s2.charAt(i + j) != s1.charAt(j)) {
%           res = -1;
%           log("Unequal at: " + j);
%         }
%         else
%           log("Equal at: " + j);
%         j++;
%       } while( j < M );
%     }
%     log("Found at: " + res);
%     i++;
%     res = i;
%     j = 0;
%   } while (i <= N - M)
%   return res;
% }

% \end{lstlisting}

% \vspace*{-5pt}
% \caption{\label{exp1} \textbf{\small Our motivating example}}
% \normalsize
% %\vspace*{-5ex}
% \end{figure}

\begin{figure}[tbp]
\centering
  \includegraphics[width=1\linewidth]{Figures/intervalsB.png}
  \caption{n-th order intervals and graphs. The set of intervals on $\mathcal{S}^1$ are $I^1(1)$=\{1\}, $I^1(2)$=\{2\}, $I^1(3)$=\{3,4,5,6\}, $I^1(7)$=\{7\}. $I^2(1)$=\{1\} and $I^2(2)$=\{2,7,8\} are the second order intervals. $I^3(1)$=\{1,9\} and $I^4(10)$=\{10\} are the only intervals on $\mathcal{S}^3$ and $\mathcal{S}^4$ respectively.}
  \label{fig:interval}
\end{figure}

% subsection 2: GGNN 
% describe how it works give some functions follow (https://www.seas.upenn.edu/~xsi/data/nips18.pdf)
\subsection{Graph Neural Network}
Graph Neural Networks (GNN)~\cite{scarselli2008graph,gori2005new} is a specialized machine learning model designed to learn from graph data.

We extend the definition of a graph to include $\mathcal{M}$ (\ie $G = (\mathcal{V}, \mathcal{E}, \mathcal{M})$). $\mathcal{M}$ is a set of vectors (or embeddings) $\{\mu_{v_1}, ..., \mu_{v_m}\}$, where each $\mu_{v} \in \mathbb{R}^d$ denotes the embedding of a node $v$ in the graph. GNN updates node embeddings via a propagation model. The simplest yet most popular is synchronous message passing systems~\cite{attiya2004distributed} introduced in distributed computing theory. Specifically, the inference is executed as a sequence of rounds: in each round, every node first sends messages to all of its neighbors, and then update its embedding by aggregating all incoming messages.
\begin{equation}
\mu^{(l+1)}_{v} = h(\{\mu^{(l)}_{u}\}_{u \in \mathcal{N}^{k}(v), k \in \{1,2,...,K\}}) \label{equ:h}
\end{equation}

$\mathcal{N}^{k}{(v)}$ denotes the neighbours that are connected to $v$ with edge type $k$, \ie, $\mathcal{N}^{k}{(v)} = \{u|(u,v,k) \in \mathcal{E}\} \cup \{u|(v,u,k) \in \mathcal{E}\} $. $h(\cdot)$ denotes the aggregation function. We repeat the propagation for $L$ steps to update $\mu_{v}$ to $\mu^{(L)}_{v}, \forall v \in \mathcal{V}$. 
%After $L$ steps, we use the state vectors from the last time step as the final node representations.

Some GNNs~\cite{si2018learning} compute a separate node embedding \wrt an edge type (\ie $\mu^{(l+1), k}_{v}$ in Equation~\ref{equ:type}) before aggregating them into a final embedding (\ie $\mu^{(l+1)}_{v}$ in Equation~\ref{equ:sum}).
\begin{align}
\mu^{(l+1), k}_{v} &= \phi_1(\sum_{\mathclap{u \in \mathcal{N}^{k}{(v)}}} \mathbf{W_1} \mu_u^{(l)}), \forall k \in \{1,2,...,K\} \label{equ:type}\\
\mu^{(l+1)}_{v} &= \phi_2(\mathbf{W_2}[ \mu_v^{(l), 1}, \mu_v^{(l), 2}, ..., \mu_v^{(l), K}]) \label{equ:sum}
% \mu^{(0)}_{v} &= \mathbf{W_1}\mu_{v} \label{equ:ini}
\end{align}

$\mathbf{W_1}$ and $\mathbf{W_2}$ are variables to be learned, and $\phi_1$ and $\phi_2$ are some nonlinear activation functions.

To further improve the model capacity,~\citet{li2015gated} proposed Gated Graph Neural Network (GGNN). Their major contribution is a new instantiation of $h(\cdot)$ (Equation~\ref{equ:h}) with Gated Recurrent Units~\cite{cho2014properties}. The following equations describe how GGNN works:
\begin{align}
%\tilde{m}_v^l &= \sum_{\mathclap{u \in \mathcal{N}^{k}{(v)}}} f(\mu_{u}^{(l)}) \label{equ:mes1}\\
%\tilde{m}_v^l &= \mathop{\sum \sum }_{k \in \mathcal{T}\  u \in \mathcal{N}^{k}{(v)}} f(\mu_{u}^{(l)}) \text{, where }\mathcal{T}\text{ is }\{1, 2, ..., K\} \label{equ:mes1}\\
\tilde{m}_v^l &= \sum_{\mathclap{u \in \mathcal{N}{(v)}}} f(\mu_{u}^{(l)}) \label{equ:mes1}\\
%\mu^{(l+1), k}_{v} &= GRU(\tilde{m}_v^l, \mu^{(l)}_{v})\label{equ:mes2}
\mu^{(l+1)}_{v} &= GRU(\tilde{m}_v^l, \mu^{(l)}_{v})\label{equ:mes2}
\end{align}

To update the embedding of node $v$, Equation~\ref{equ:mes1} computes a message $\tilde{m}_v^l$ using $f(\cdot)$ (\eg a linear function) from the embeddings of its neighboring nodes $\mathcal{N}{(v)}$. Next a $GRU$ takes $\tilde{m}_v^l$ and $\mu^{(l)}_{v}$---the current embedding of node $v$---to compute the new embedding, $\mu^{(l+1)}_{v}$ (Equation~\ref{equ:mes2}).
%Then, $GRU$ takes the aggregated message $\tilde{m}_v^l$ of node $v$ and the current state $\mu^{(l)}_{v}$ of node $v$ to compute the next representation of $v$.

% Similarly, the propagation will be repeated for a fixed number of time steps. In the end, we use the embeddings from the last time step as the final node representations.

==> GGNN_paper-(submission)/Sections/Problem.tex <==
% !TeX root = ../ggnn.tex

\section{Software defects}\label{sec:problem}
\subsection{Null pointer exception}

\begin{figure}[t]
%\centering
\small
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
public SortedKeyValueIterator<Key,Value> deepCopy(IteratorEnvironment env) {
    ...
    // rowMatcher may be null
    result.rowMatcher = rowMatcher.pattern().matcher("");
    ...
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\vspace*{-5pt}
\caption{\label{NPE} NPE example (from bugs-dot-jar\_ACCUMULO-189)}
\normalsize
%\vspace*{-5ex}
\end{figure}

\subsection{Array index out-of-bound}



\subsection{Class cast exception}

\begin{figure}[t]
%\centering
\small
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
    ...
    } else if (target instanceof FilterProcessor) {
        // FilterDefinition is so precise that it results in class cast exception
        // The patch changes it to its parent class ExpressionNode.
        answer = new ManagedFilter(context, (FilterProcessor) target,
        (FilterDefinition) definition);
    ...
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\vspace*{-5pt}
\caption{\label{CCE} Class cast exception (from bugs-dot-jar\_CAMEL-9672)}
\normalsize
%\vspace*{-5ex}
\end{figure}




==> GGNN_paper-(submission)/Sections/Relatedwork.tex <==
% !TeX root = ../ggnn.tex

\section{Related Work}\label{sec:related}

% \paragraph{\textbf{Language Models for Programs}}
% The recent success in machine learning has lead to a strong interest in applying machine learning techniques to learn program representations.
% %One major research direction is to model programs for machine learning.
% ~\citet{hindle2012naturalness} leverage an n-gram language model to show that source code is highly repetitive. 
% %\citet{bhoopchand2016learning} model the code as a sequence of tokens to capture long-range dependencies. 
% other works~\cite{maddison2014structured, bielik2016phog, Alon:2018:GPR:3192366.3192412,Alon:2019:CLD:3302515.3290353} model the code structure based on ASTs. 
% %Alon et al. \cite{Alon:2018:GPR:3192366.3192412} 
% %learn from paths through ASTs to produce general representations
% %of programs; in \cite{Alon:2019:CLD:3302515.3290353} they expand upon this general representation by leveraging attention mechanisms.
% %However, the two methods cannot
% %represent unseen relations.
% %To improve it, they propose word2seq \cite{alon2018code2seq}, which can represent and use any syntactic path in any unseen example by representing AST paths node-by-node using LSTMs. Further, it decodes
% %the output sequence step-by-step while attending over the input paths, and can thus generate unseen
% %sequences, compared to code2vec \cite{Alon:2019:CLD:3302515.3290353}, which has a closed vocabulary.
% \citet{henkel2018code} use abstractions of traces obtained from symbolic execution of a program as a representation for learning program embeddings. Wang~\etal proposed another line of works in learning program semantics from executions~\cite{wang2017dynamic,wang2019learning}; of late they show combining symbolic and concrete executions could be an even more promising approach in learning precise and efficient program embeddings~\cite{wang2019hybrid}.


\paragraph{\textbf{Machine Learning for Defect Prediction}}
Utilizing machine learning techniques for software defect prediction is another rapidly growing research field. So far the literature has been focusing on detecting simpler bugs that are syntactic in nature. 
%is used for detecting some easier bugs in programs at the beginning, \eg, name-based bugs.
%Name-based bug detection relates to existing learning-based approaches that consider identifiers.
%Raychev et al. propose a prediction engine called JSNice for predicting (syntactic) names of identifiers and predicting (semantic) type annotations of variables \cite{raychev2015predicting}.
%They also propose a complementary tool of JSNice, called AUTONYM, to address the problem of recovering meaningful identifiers from minified code, using conditional random fields and statistical machine translation, respectively\cite{vasilescu2017recovering}. 
%Another approach summarizes code into descriptive names that can serve, \eg, as method names \cite{allamanis2017learning}.
\ignore{
Choi et al. train a memory network model \cite{} for predicting buffer overruns in programming language analysis\cite{Choi2017bufferoverrun}. 
Their work can only work on buffer overrun prediction since they generate dataset by only focusing on buffer related functions}
%Li~\etal proposed a deep learning-based vulnerability detector VulDeePecker~\cite{ndssLiZXO0WDZ18VulDeePecker} 
%, in which they use code gadgets to represent programs and then generate vectors for learning \cite{ndssLiZXO0WDZ18VulDeePecker}. 
%Their model learns from positive and negative examples, but the examples are manually created and labeled.
\citet{wang2016automatically} leverages deep belief network to learn program representations for defect prediction. Their model predicts an entire file to be buggy or not. \citet{pradel2018deepbugs} present Deepbugs, a framework to detect name-based bugs in binary operation. Another line of works targets variable misuse bugs~\cite{allamanis2017learning,vaswani2017attention}, in which developers use wrong variables, and models are required to predict the ones that should have been used. Clearly, \tool significantly differs from all of them as it locates complex semantic bugs.

% \tool deals with semantic bugs that are general and complex. As a more specialized effort, some prior works also attempted to detect vulnerabilities in programs. \citet{Choi2017bufferoverrun} trains a memory network model for predicting buffer overruns. \citet{ndssLiZXO0WDZ18VulDeePecker} proposed a deep learning-based vulnerability detector VulDeePecker. A drawback is their model relies on examples that are manually created, whereas, \tool only considers real-world programs. 
% and is equipped with the infrastructure to collect data automatically.
%learns from positive and negative examples, but the examples are manually created and labeled.
%Their work can only work on buffer overrun prediction since they generate dataset by only focusing on buffer related functions}
%Li~\etal proposed a deep learning-based vulnerability detector VulDeePecker~\cite{ndssLiZXO0WDZ18VulDeePecker} 
%, in which they use code gadgets to represent programs and then generate vectors for learning \cite{ndssLiZXO0WDZ18VulDeePecker}. 
%Their model learns from positive and negative examples, but the examples are manually created and labeled.

%They use dedicated word embedding for each kind of name-based bugs, in order to form semantic features from methods, and they use learn-bug detectors to conduct bug detection.
%However, dedicated code representation for each bug requires additional effort to design and implement. 
%In contrast, we focus on deep and semantic bugs rather than name-based bugs.

\paragraph{\textbf{Static Bug Finding}}
In principle, static analysis models all executions of a program in order to provide the soundness guarantee. However, perfectly sound static analysis tools almost never exist; concessions that sacrifice the soundness guarantee have to be made to ensure the usability of static analyzers. Several years ago, a new term---soundiness~\cite{livshits2015defense}---is brought forward aiming to clarify the level of approximation adopted in the analysis. Below we survey several flagship static analyzers.

SLAM~\cite{Ball2002}, BLAST~\cite{Henzinger2002}, and SATABS~\cite{Clarke2004} adopt abstract
refinement for static bug checking. CBMC~\cite{Clarke2003,Clarke2004} performs bounded model checking. Saturn~\cite{Xie2005,Dillig2008} is another program analysis system, which uses the combination of summaries and constraints to achieve both high scalability and precision. Compass~\cite{Dillig2011} performs bottom-up, summary-based heap analysis for the verification of real C and C++ programs.

Compared with static analysis tools, we believe \tool yields several conceptual advantages. First, with \tool, creating a static bug finder can be simplified to solving a machine learning task. In comparison, the traditional way of designing static analyzers even the unsound ones requires a substantial amount of human expertise. Besides, unlike the static analysis tools, model-based bug detectors can benefit from increasingly large datasets and powerful training regime, as a result, they will evolve and get better over time.


% Recent works focus on the paradox - a highly precise analysis limits its scalability and an imprecise one seriously hurts its precision or recall. 
% Pinpoint~\cite{shi2018pinpoint} and SMOKE~\cite{fan2019smoke} present two kinds of techniques to resolve the paradox.

% \citet{shi2018pinpoint} propose function-level summary to decompose the cost of high-precision points-to analysis by precisely discovering local data dependency. Then it leverages the function summary when conducting the expensive inter-procedural analysis. SMOKE~\cite{fan2019smoke} adopts a staged approach to design an analysis of high precision, while being able to scale to large programs. In the first stage, instead of using a uniform precise analysis for all paths, it uses a scalable but imprecise analysis. In the second stage, it leverages a more precise analysis to verify the feasibility of those candidates. Facebook Infer~\cite{calcagno2015moving, calcagno2009compositional, berdine2005smallfoot} combines techniques like separation logic~\cite{berdine2005smallfoot} and bi-abduction~\cite{calcagno2009compositional}. Separation logic is a kind of mathematical logic which facilitates reasoning about mutations to computer memory. It enables scalability by breaking reasoning into chunks corresponding to local operations on memory, and then composing the reasoning chunks together. Bi-abduction is a form of logical inference for separation logic which automates the key ideas about local reasoning.



==> GGNN_paper-(submission)/Sections/Tables.tex <==

\begin{table*}[!t]
\centering
\small
\caption{Performance on  alternative node representations in \tool}
\begin{tabular}{c|ccc|ccc|ccc}
\hline
\multirow{2}{*}{\tabincell{c}{Bug types}} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{Array} & \multicolumn{3}{c}{CCE}\\
\cline{2-10}
& Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall & F1 \\\hline
\tabincell{c}{Characteristic\\vectors}&  00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\\hline
\tabincell{c}{RNN-based\\encoding } & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0  \\\hline
\tabincell{c}{Transformer-based\\encoding } & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\\hline 

\end{tabular}
\label{tab:alter}
\end{table*}



\begin{table*}[!t]
\centering
\small
\caption{Performance on method-level prediction}
\begin{tabular}{c|ccc|ccc|ccc}
\hline
 \multirow{2}{*}{\tabincell{c}{Bug types}} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{Array} & \multicolumn{3}{c}{CCE} \\
\cline{2-10}
& Precision & Recall & F1 & Precision & Recall & F1  & Precision & Recall & F1  \\\hline
\tool & 65.6 & \textbf{72.1} & \textbf{68.7} &  \textbf{70.7} & 52.3 & 60.1 &70.1 &  48.6 & 57.4 \\\hline
AST & 77.4 & \textbf{85.7} & \textbf{81.4} &  \textbf{84.2} & 57.1 & 68.1 &  69.2 & 64.3 & 66.7  \\\hline
CFG & 77.3 & \textbf{81.0} & \textbf{79.1} &  78.9 & 71.4 & 75.0 &   \textbf{82.4} & 66.7 & 73.7  \\\hline

\end{tabular}
\label{tab:metRes}
\end{table*}



\begin{table*}[!t]
\centering
\small
\caption{Performance on line-level prediction}
\begin{tabular}{c|c|ccc|ccc|ccc}
\hline
 \multirow{2}{*}{\tabincell{c}{Bug types}} & \multirow{2}{*}{Top-N} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{Array} & \multicolumn{3}{c}{CCE} \\
\cline{3-11}
&  & Precision & Recall & F1 & Precision & Recall & F1  & Precision & Recall & F1  \\\hline
\multirow{5}{*}{\tool} & Top-1 & 44.1 & 44.1 & 44.1 & 37.8 & 37.8 & 37.8 & \textbf{47.7} & \textbf{47.7} & \textbf{47.7} \\\cline{2-11}
& Top-3 & 19.2 & \textbf{57.7} & 28.8 & \textbf{22.3} & 55.0 & \textbf{31.7} & 18.6 & 55.9 & 27.9 \\\cline{2-11}
& Top-5 & 15.1 & \textbf{67.6} & 24.7 & \textbf{16.9} & 64.0 & \textbf{26.8} & 13.7 & 61.3 & 22.4 \\\cline{2-11}
& Top-7 & 12.6 & \textbf{73.0} & 21.5 & \textbf{14.7} & 72.1 & \textbf{24.4} & 11.7 & 67.6 & 19.9 \\\cline{2-11}
& Top-10 & 11.0 & \textbf{82.0} & 19.5 & \textbf{13.0} & 80.2 & \textbf{22.3} & 10.7 & 79.3 & 18.8  \\\hline
\multirow{5}{*}{AST} & Top-1 & \textbf{35.7} & \textbf{35.7} & \textbf{35.7} & 28.6 & 28.6 & 28.6 & 32.1 & 32.1 & 32.1 \\\cline{2-11}
& Top-3 & \textbf{16.7} & \textbf{50.0} & \textbf{25.0} & 12.7 & 35.7 & 18.7 & 15.5 & 46.4 & 23.2 \\\cline{2-11}
& Top-5 & \textbf{14.8} & \textbf{71.4} & \textbf{24.5} & 8.7 & 39.3 & 14.2 & 9.6 & 46.4 & 16.0 \\\cline{2-11}
& Top-7 & \textbf{11.5} & \textbf{75.0} & \textbf{19.9} & 6.9 & 42.9 & 11.9 & 8.7 & 57.1 & 15.2 \\\cline{2-11}
& Top-10 & \textbf{8.4} & \textbf{75.0} & \textbf{15.1} & 7.7 & 64.3 & 13.7 & 7.2 & 64.3 & 12.9  \\\hline
\multirow{5}{*}{CFG} & Top-1 & 47.6 & 47.6 & 47.6 & \textbf{66.7} & \textbf{66.7} & \textbf{66.7} & 52.4 & 52.4 & 52.4 \\\cline{2-11}
& Top-3 & 23.8 & \textbf{71.4} & 35.7 & \textbf{26.4} & 66.7 & \textbf{37.8} & 22.2 & 66.7 & 33.3 \\\cline{2-11}
& Top-5 & 17.9 & \textbf{81.0} & 29.3 & \textbf{22.4} & \textbf{81.0} & \textbf{35.1} & 16.8 & 76.2 & 27.6 \\\cline{2-11}
& Top-7 & 14.4 & 81.0 & 24.5 & \textbf{19.4} & \textbf{85.7} & \textbf{31.6} & 13.6 & 76.2 & 23.0 \\\cline{2-11}
& Top-10 & 14.1 & \textbf{95.2} & 24.5 & \textbf{18.5} & \textbf{95.2} & \textbf{31.0} & 14.1 & \textbf{95.2} & 24.5  \\\hline

\end{tabular}
\label{tab:lineres}
\end{table*}


==> GGNN_paper-(submission)/commands.tex <==
\usepackage{xspace}
\usepackage{multirow}
\usepackage{algorithmic}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{pgffor} % \foreach \java in  {NPE, Array, CCE}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{enumitem}
\usepackage{caption}
\usepackage{pgfplots}
\pgfplotsset{
    compat=1.4,
    small,
    legend style={
        at={(0.99,0.99)},
        anchor=north east,
        font=\bfseries,
    },
    label style={font=\sffamily\small\bfseries}
}%




\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\usepackage{mdframed}
\usepackage{xcolor}
\usepackage{adjustbox}
\usepackage{listings}
   \lstdefinestyle{mystyle}{
      % backgroundcolor=\color{backcolour},   
      frame=single,
      framexleftmargin=0pt,
      commentstyle=\color{green},
      keywordstyle=\color{blue}\bfseries,
      numberstyle=\tiny\color{gray},
      stringstyle=\color{purple},
      basicstyle=\scriptsize\ttfamily\bfseries,
      breakatwhitespace=false,         
      breaklines=false,                 
      captionpos=b,                    
      keepspaces=true,     
    %   xleftmargin=0em,
    %   xrightmargin=0em,
      numbers=none,                    
      numbersep=4pt,                  
      showspaces=false,                
      showstringspaces=false,
      showtabs=false,                  
      tabsize=2,
      language=Java,
    %   moredelim=**[is][\underbar]{_}{_},
      escapechar=\%
      % moredelim=**[is][\btHL]{`}{`},
      % moredelim=**[is][{\btHL[fill=red!40]}]{@}{@},%,draw=red,dashed,thick  
   }
   \lstset{style=mystyle}
\usepackage{pifont}
\usepackage{tikz}
\usetikzlibrary{matrix}
\usepackage{bm}
\usepackage{flushend}

\definecolor{light-gray}{gray}{0.80}

\newcommand*{\bigrightArrow}{|[yshift=-2]| \color{green}{\scalebox{2.4}[3.6]{\ding{225}}}}
\newcommand*{\bigleftArrow}{ \color{green}{\rotatebox[origin=c]{180}{\scalebox{2.4}[3.6]{\ding{225}}}}}


\newcommand*{\bigdoubleArrow}{\color{gray}{\rotatebox[origin=c]{90}{\scalebox{1.5}[2.2]{$\bm{\Updownarrow}$}}}}

\newcommand{\tool}{\textsc{NeurSA}\xspace}

%\newcommand{\tool}{\textsc{GUARD}\xspace}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}


\newcommand{\ke}[1]{{\color{purple} \sf KE: #1}}

\newcommand{\gfj}[1]{{\color{blue} \sf GFJ: #1}}
\newcommand{\wyc}[1]{{\color{red} \sf #1}}
\newcommand{\ignore}[1]{\iffalse #1 \fi}

\usepackage{rotating}

% English
\newcommand{\cf}{\hbox{\emph{cf.}}\xspace}
\newcommand{\deletia}{\ldots [deletia] \ldots}
\newcommand{\etal}{\hbox{\emph{et al.}}\xspace}
\newcommand{\eg}{\hbox{\emph{e.g.}}\xspace}
\newcommand{\ie}{\hbox{\emph{i.e.}}\xspace}
\newcommand{\scil}{\hbox{\emph{sc.}}\xspace} 
\newcommand{\st}{\hbox{\emph{s.t.}}\xspace}
\newcommand{\wrt}{\hbox{\emph{w.r.t.}}\xspace}
\newcommand{\etc}{\hbox{\emph{etc.}}\xspace}
\newcommand{\viz}{\hbox{\emph{viz.}}\xspace}
\newcommand{\vv}{\hbox{\emph{vice versa}}\xspace}

%\theoremstyle{definition}
%\newtheorem{definition}{Definition}[section]



\definecolor{OliveGreen}{rgb}{0,0.6,0}

\lstset{basicstyle=\ttfamily,numbers=left,numberstyle=\tiny,keywordstyle=\color{blue!70},
commentstyle=\color{OliveGreen},
rulesepcolor=\color{red!20!green!20!blue!20}
% escapeinside=``,xleftmargin=2em,xrightmargin=2em, aboveskip=1em
}

\lstset{escapeinside={(*@}{@*)}}


\DeclareMathOperator*{\maxx}{max}

% \theoremstyle{definition}
% \newtheorem{assumption}[theorem]{Assumption}

\newcommand{\rBugs}{50\xspace}
\newcommand{\cBugs}{3\xspace}
\newcommand{\fBugs}{7\xspace}


==> Sections/Append.tex <==
\subsection{Irreducible Graph }

Figure \ref{fig:irredGraph} shows examples of graphs that can not be reduced to a single node.

\begin{figure}[htb!]
\centering
  \includegraphics[width=.25\linewidth]{Figures/non-reduce.pdf}
  \caption{Examples of irreducible graph.}
  \label{fig:irredGraph}
\end{figure}


\subsection{Examples of Array Index Out of Bound bugs and Class Cast Exceptions}

Figure \ref{fig:CCEExamples} and \ref{fig:AIOOBExamples} show examples of the array index out of bound and class casting bugs.
Note that even though there are lots of these kinds of bugs, the pattern of them are less than null pointer dereference bugs.


\begin{figure*}
\begin{subfigure}[htb!]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Casting PC to ChildClass raises CCE.
public void manipulate(ParentClass PC) {
    ChildClass CC = (ChildClass) PC;
}
    
public void foo() {
    ParentClass PC = new ParentClass();
    manipulate(PC);
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:CCEa} A typical pattern of CCE.}
\end{subfigure}

\begin{subfigure}[b]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Extracted from bugs-dot-jar_LOG4J2-104
static {
    ...
    // url.returnLines() returns objects not in XML format
    props.loadFromXML(url.returnLines());
    ...
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:CCEb} CCE caused by different class.}
\end{subfigure}


\begin{subfigure}[b]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Extracted from bugs-dot-jar_CAMEL-9672
public Object getManagedObjectForProcessor(CamelContext context, 
                                        Processor processor,
                                        ProcessorDefinition<?> definition, 
                                        Route route) {     
    ...
    } else if (target instanceof FilterProcessor) {
        // FilterDefinition is so precise that it results in CCE
        // The repair patch changes it to its parent class ExpressionNode.
        answer = new ManagedFilter(context, (FilterProcessor) target,
        (FilterDefinition) definition);
    ...
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:CCEc} CCE caused by class inherent.}
\end{subfigure}


\begin{subfigure}[b]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Extracted from eclipse.jdt.ui-096ab8f
private ITypeBinding getDestinationBinding() throws JavaModelException {
    ...
    // None of the two class cast operations are safe.
    return (ITypeBinding)((SimpleName)node).resolveBinding();
    // Fixed codes
    if (!(node instanceof SimpleName)) return null;
    IBinding binding= ((SimpleName)node).resolveBinding();
    if (!(binding instanceof ITypeBinding)) return null;
    return (ITypeBinding)binding;
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:CCEd} CCE caused by multiple class cast operations.}
\end{subfigure}
\caption{Illustrative examples of the CCE bugs.}
\label{fig:CCEExamples}
\end{figure*}


\begin{figure*}[t]
%\centering
\begin{subfigure}[b]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Extracted from eclipse.platform.ui-fa4aec8
public void restoreState(IDialogSettings dialogSettings) {
    ...
    priorities[i] = Integer.parseInt(priority);
    ...
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:array1} A typical pattern of AIOE.}
\end{subfigure}


\begin{subfigure}[b]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Extracted from bugs-dot-jar_LOG4J2-811
public void logMessage(final String fqcn, final Level level, 
    final Marker marker, final Messagemsg,
    final Throwable throwable) {
    ...
    // the length of params can be zero.
    if (... && params != null && params[params.length - 1] instanceof Throwable) {
        t = (Throwable) params[params.length - 1];
    } 
    ...
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:array2} AIOE caused by zero length array.}
\end{subfigure}


\begin{subfigure}[b]{1\textwidth}
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
// Extracted from tomcat-3f4a241
public void addFilterMapBefore(FilterMap filterMap) {
    ...
    // The 4-th argument should be filterMaps.length - (filterMapInsertPoint + 1)
    System.arraycopy(filterMaps, filterMapInsertPoint, results,
    filterMaps.length - filterMapInsertPoint + 1,
    ...
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\caption{\label{fig:array3} AIOE caused by miscalculate starting position in destination array.}
\end{subfigure}

\caption{Illustrative examples of AIOE.}
\label{fig:AIOOBExamples}
\end{figure*}

\clearpage

\subsection{Other Pertinent Information of Evaluated Projects}

Table \ref{tab:numOfBugs} shows the number of bugs and buggy methods in our evaluated projects. The number outside (inside) of the parenthesis is the number of bugs (buggy methods). Note that developer may fix multiple methods for a single bug so the number of buggy method and bugs may differ.

\begin{table*}[htbp!]
\centering
\small
\caption{Number of bugs of evaluated projects}
\begin{tabular}{c|ccc}
\hline
  \multirow{2}{*}{\tabincell{c}{Projects}} &  \multicolumn{3}{c}{Number of bugs (buggy methods)} \\
\cline{2-4}
& \tabincell{c}{NPE} & \tabincell{c}{AIOE} & \tabincell{c}{CCE} \\\hline
Lang &  5 (7) & 3 (5) & 1 (2)  \\\hline
Closure & 2 (18) & 0 (0) & 0 (0)  \\\hline
Chart & 4 (17) & 1 (7) & 0 (0)  \\\hline
Mockito & 7 (14) & 2 (5)  & 5 (23)  \\\hline
Math & 10 (16)  & 8 (17) & 2  (3) \\\hline
Accumulo & 5 (6)  & 0 (0) & 0 (0)  \\\hline
Camel & 8 (17) & 1 (1) & 1 (1)  \\\hline
Flink & 6 (13) & 0 (0) & 0 (0)  \\\hline
Jackrabbit-oak & 7 (23) & 1 (1) & 1 (1)  \\\hline
Log4j2 & 16 (29) & 1 (1) & 1  (2) \\\hline
Maven & 3 (6) & 0 (0) & 0 (0)  \\\hline
Wicket & 6 (7) & 1 (1) & 3 (8)  \\\hline
Birt & 165 (678) & 19 (129) & 39 (154)  \\\hline
JDT UI & 332  (897) & 39 (63) &  47 (156) \\\hline
SWT & 105  (276) & 40 (136) & 7  (26)  \\\hline
Platform UI & 389  (920) & 27 (72) & 60  (194) \\\hline
Aspectj & 72  (151) & 9 (14) &  9  (19) \\\hline
Tomcat & 44  (111) & 6  (18)& 12  (28) \\\hline
\hline
Total & 1186 (3206) & 143 (470) & 188 (617)  \\\hline
\end{tabular}
\label{tab:numOfBugs}
\end{table*}









\ignore{

\begin{table*}[!t]
\centering
\small
\caption{Projects used in the evaluation.}
\begin{tabular}{c|c|c|ccc}
\hline
 \multirow{2}{*}{Dataset} & \multirow{2}{*}{Projects} & \multirow{2}{*}{Description}&  \multicolumn{3}{c}{\#Methods} \\
\cline{4-6}
& & &\tabincell{c}{NPE} & \tabincell{c}{Array} & \tabincell{c}{\tabincell{c}{CCE}} \\\hline
\multirow{13}{*}{Test} &Lang & Java lang library & 486 & 225 & 174  \\\cline{2-6}
&Closure & A JavaScript checker and optimizer. & 46 & 0 & 0  \\\cline{2-6}
&Chart & Java chart library & 504 & 20 & 0  \\\cline{2-6}
&Mockito & Mocking framework for unit tests & 209 & 22 & 94  \\\cline{2-6}
&Math & Mathematics and statistics components & 188 & 284 & 31  \\\cline{2-6} % 121+67, 139+145, 31
&Accumulo & Key/value store & 69 & 0 & 0  \\\cline{2-6}
&Camel & Enterprise integration framework & 653 & 98 & 12  \\\cline{2-6}
&Flink & System for data analytics in clusters & 141 & 0 & 0  \\\cline{2-6}
&Jackrabbit-oak & hierarchical content repository & 289 & 34 & 24  \\\cline{2-6}
&Log4j2 & Logging library for Java & 187 & 9 & 2  \\\cline{2-6}
&Maven & Project management and comprehension tool & 50 & 0 & 0  \\\cline{2-6}
&Wicket & Web application framework & 98 & 42 & 30  \\\hline
\hline
\multicolumn{3}{r|}{Total}& 2920 (173) & 734 (38) & 365 (40)  \\\hline % (num) is the number of buggy methods
\hline
\multirow{6}{*}{Training}&Birt & Data visualizations platform & 1356 & 258 & 308  \\\cline{2-6}
&JDT UI & User interface for the Java IDE & 1794 & 126 & 312 \\\cline{2-6}
&SWT & Eclipse Platform project repository & 552 & 272 & 52  \\\cline{2-6}
&Platform UI & User interface and help components of Eclipse & 1840 & 144 & 388  \\\cline{2-6}
&AspectJ & An aspect-oriented programming extension & 302 & 28 &  38 \\\cline{2-6}
&Tomcat & Web server and servlet container & 222 & 36 & 56  \\\hline
\hline
\multicolumn{3}{r|}{Total}& 6066 (3033) & 864 (432) & 1154(577)  \\\hline
\end{tabular}
\label{tab:methodres}
\end{table*}
}



==> Sections/Discussion.tex <==
% !TeX root = ../ggnn.tex

\section{Limitation}\label{sec:discussion}
% This section discusses the limitation of \tool, and several other related subject matters.

% \subsection{Limitation}
We also discovered several issues that prevented \tool from being more effective. One, in particular, is the scalability. \tool is notably less accurate when handling larger programs despite the contribution IBPM makes to the underlying GNN. Naturally, steady advances in deep learning research would keep pushing the limit of model capacity. As a result, solutions in the specific application domains would continue to get better. In addition, we conjecture that better program representation that enables deep learning models to fulfill their potential may exist and worth exploring. Most importantly, we believe fundamental research aiming to explain why GNN can learn to analyze programs is necessary. Without a deeper understanding of GNNs, IBPM's results will be hard to improve upon.

% Even though IBPM significantly improves GNN's scalability, \tool tends to mishandle large programs. Steady advances in the deep learning community would keep pushing the limit of model capacity. As a result, solutions in the specific application domains would continue to get better. In addition, we conjecture that better program representation that enables deep learning models to fulfill their potential may exist and worth exploring. Most importantly, we believe fundamental research aiming to explain why GNN can learn to analyze programs is necessary. Specifically, how is the message-passing protocol, a seemingly effective technique on a general-purpose graph structure, even a sensible approach for any graph representation of a program? Answers to those questions help to diagnose the cause of GNN's shortcomings and stimulate future research. 

\tool is also limited by the availability of high-quality, large-scale datasets. Even with the synthetic buggy code injected into our dataset, it is not nearly at the same scale as other machine learning datasets (\eg ImageNet~\cite{russakovsky2015imagenet}). Considering the size and complexity of programs, it is fair to argue dataset of programs should be even larger for sufficiently training a quality model. 
% The difficulty though is the tremendous human effort that is needed to assemble such a dataset even with the abundant, freely accessible repositories of source code. Because automating this process involves other manual work such as identifying buggy code snippets, analyzing their root causes, collecting the corresponding fixes, \etc Examples like BugSwarm~\cite{tomassi2019bugswarm} have made great strides, however, we have found it to be significantly more noisy than defect4j and bugs.jar, two manually analyzed datasets.
% in our experiments. 

When applying \tool to catch bugs in the wild, we find \tool could have been a more useful bug-finding tool if it can provide justification to the developers as to why a particular code snippet is predicted to be buggy. We believe this issue can be promptly addressed by incorporating the ideas from a long line of works in the explainability of machine learning models~\cite{guidotti2019survey}. At the very least, \tool can highlight the regions of programs that have the most influence on its predictions, a technique researchers developed to explain why an image is predicted in a certain category.

% \subsection{Dealing with Noise}
% % \ignore{\gfj{As discussed in \cite{kim2011dealing}, recent studies have discovered that data so collected contain noises because current defect collection practices are based on optional bug fix keywords or bug report links in change logs. Automatically collected defect data based on the change logs could include noises.}}

% Recent studies~\cite{kim2011dealing} have discovered that the datasets used for training bug detectors can be noisy. We discuss two potential sources that could introduce noise in our datasets. 

% First, bugs types can be mislabeled (\eg null pointer dereference can be labeled as an array index out of bound). As explained in Section~\ref{subsec:over}, we determine the type of a bug by matching key words in the bug report. Even though the correctness can not be guaranteed, it is fair to disregard mislabeling as a serious issue. Because the nature of the three types of bugs we deal with is very different. Unless developer made a mistake in describing the bug in the report, the way we determine a bug type should be reliable. 

% Second, identifying a buggy method based upon the code patches is unsound. It is entirely possible for developers to commit quick hack around instead of fixes that address the root cause of the bug. However, since our datasets are well-studied in the literature, noise caused by imprecise fixes should be minimal. For the manually checked bugs, 79 in total, we only tweaked one bug location, which signals the quality of our datasets.

% % To confirm our hypothesis, we randomly pick 100 bugs in our datasets for manual inspection, and we find that all of them have not only the correct labels of bug types but also the correct locations in the method. 

% % \ignore{
% % \wyc{To further avoid noisy data, we use defects4j and bugs.jar as the ground truth (\ie, testing dataset) because they are widely used datasets. 
% % In contrast, the training dataset extends the dataset provided by \citet{ye2014learning}, which might be more noise and thus is not suitable to be the ground truth.}

% % We found that there is only one exception.
% % The case is that the code snippet contains a comment about NPE bug, which is identified as an NPE bug in \tool.
% % From the result we can claim that the noise in our datasets is small enough to be used in evaluation.}

% Finally, even though the noise is inevitable, our neural bug detectors beat the baseline on a level playing field.

% % \ignore{It is an unsound way and thus may miss related bugs.
% % However, it barely collects wrong bugs because if a bug report mentions some exception such as \textit{NullPointerException}, it probabily related to the null pointer bug.
% % The second kind is from imprecise patch analysis, \ie, identification of buggy methods and buggy lines.
% % There would be many incorrect/redundant buggy methods if we did not ignore some buggy irrelevant operations, new blank lines in a method for example.}

% % \subsection{Data Sufficiency}


% % \begin{figure}[htb!]
% % \captionsetup{justification=centering}
% % \begin{subfigure}{.4\textwidth}
% % \centering
% %   \includegraphics[width=\linewidth]{Figures/dataSizePerf.png}
% %   \caption{F1 score on NPE bugs.}
% %   \label{fig:dataSizePerfNPE}
% % \end{subfigure}
% % \par\bigskip
% % \begin{subfigure}{.4\textwidth}
% % \centering
% %   \includegraphics[width=\linewidth]{Figures/dataSizePerfArray.png}
% %   \caption{F1 score on AIOE bugs.}
% %   \label{fig:dataSizePerfArray}
% % \end{subfigure}
% % \par\bigskip
% % \begin{subfigure}{.4\textwidth}
% % \centering
% %   \includegraphics[width=\linewidth]{Figures/dataSizePerfCCE.png}
% %   \caption{F1 score on CCE bugs.}
% %   \label{fig:dataSizePerfCCE}
% % \end{subfigure}
% % \caption{How F1 varies as training data increase.}
% % \label{fig:dataSizePerf}  
% % \end{figure}

% % In this experiment, we examine the sufficiency of our training data. Specifically, starting from 10\% of the original training data, we gradually increase the percentage to investigate the performance trend for the three sets of neural bug detectors built by \tool and two other baselines. The testing data is kept intact for this experiment.
% % %\wyc{WY: updated to the three bug dataset instead of one}
% % %We measure the data sufficiency for all the three kinds of datasets we used.
% % %TODO: add results.
% % %The result in Fig. \ref{fig:dataSizePerf} shows the line chart of F1 score in different percentage of our dataset.
% % Figure~\ref{fig:dataSizePerf} shows how the F1 scores change as the percentage of the original training data increases. 
% % %is $N$ and Y-axis is the F1 score.
% % %$N$ ranges from 10 to 100, denoting that we use 10\% to 100\% of dataset for training.
% % Figure~\ref{fig:dataSizePerfNPE} shows the three competing models in catching null pointer dereference bugs. Three models show similar convergence. That is when reaching 80\% all three models show little improvements onward. Even at 50\%, their performances do not change by a big margin. 
% % %In fact, the performance becomes close to each other when there is more than 50\% of dataset.
% % Compared to the two baselines, the model built based on \tool requires less training data to converge. Overall, we conclude our data set is sufficient for training detectors of null pointer dereference bugs.
% % %Therefore, the number of bugs is enough for our evaluation.

% % %Note that it is the F1 score on NPE dataset, which is the largest dataset among the three bug datasets we used.
% % %The other two datasets include 14.4\% and 22.4\% of NPE dataset.

% % Figure~\ref{fig:dataSizePerfArray} and~\ref{fig:dataSizePerfCCE} shows 
% % the performance trend of the other two classes of bug detectors. Compared to the null pointer dereference bug detectors, all array index out of bound bug detectors display a smoother convergence, indicating the lower complexity in learning the semantic patterns of array index out of bound bugs. Similarly, class casting bugs detectors also seem to require less amount of training data to generalize compared to the null pointer dereference bugs. According to our manual inspection, the reason is that the patterns of null pointer dereference bugs are significantly more diverse than those of the other two bug types. To some degree, it also explains null pointer dereference bugs are harder to prevent, which tend to occur more frequently than other types of bugs in software development. 
% % % We list several examples of null pointer dereference bugs in Figure~\ref{fig:NPEs} we encountered in our dataset. 

% % Overall, we demonstrate in this experiment, the training data for all three sets of bug detectors are sufficient. Bug detectors instantiated from \tool tend to converge early with higher precision.
% % \ignore{
% % The bug in Figure~\ref{fig:npe1} is caused by calling a null pointer because \texttt{context.getManager()} may return $\mathit{NULL}$.
% % Fig. \ref{fig:npe2} misses an additional check to avoid \texttt{null == null} while Fig. \ref{fig:npe3} introduces an NPE by splitting empty data.
% % Fig. \ref{fig:npe4} shows an NPE caused by insufficient checks because \texttt{failureDetector} itself can be $\mathit{NULL}$.
% % Therefore, we should check \texttt{failureDetector} first and then check whether \texttt{failureDetector.get()} is success.}





% % \ignore{
% % The performance of the two datasets is similar to the NPE dataset,
% % the reason is that different kinds of bugs require various training data.
% % For example, the pattern in class cast exception is more clear because almost every buggy lines have type cast operations.
% % Similarly, array index out of bound exception has a pattern in the form of $array[index]$, which is also more clear comparing to null pointer dereference bugs.
% % However, the pattern of NPE bug is various and depends on how to use a pointer.
% % This is also the reason why the number of NPE bugs is significantly larger than the other two.
% % For instance, examples in Fig. \ref{fig:NPEs} are found when we inspect the NPE dataset.
% % The bug in Fig. \ref{fig:npe1} is caused by calling a null pointer because \texttt{context.getManager()} may return $\mathit{NULL}$.
% % Fig. \ref{fig:npe2} misses an additional check to avoid \texttt{null == null} while Fig. \ref{fig:npe3} introduces an NPE by splitting empty data.
% % Fig. \ref{fig:npe4} shows an NPE caused by insufficient checks because \texttt{failureDetector} itself can be $\mathit{NULL}$.
% % Therefore, we should check \texttt{failureDetector} first and then check whether \texttt{failureDetector.get()} is success.}




% % \begin{figure*}[htbp!]
% % %\centering
% % \ignore{
% % \begin{subfigure}[b]{1\textwidth}
% % \begin{mdframed}[roundcorner=5pt]
% % \scriptsize
% % \begin{lstlisting}[language=C++,showstringspaces=false]
% % ...
% % scriptContext.getContext().setApplicationClassLoader(
% %     getApplicationClassLoader());
% % ...
% % \end{lstlisting}
% % \vspace*{-4pt}
% % \end{mdframed}
% % \caption{\label{fig:npe1} NPE caused by calling a null pointer.}
% % \end{subfigure}
% % }



% % \begin{subfigure}[b]{1\textwidth}
% % \begin{mdframed}[roundcorner=5pt]
% % \scriptsize
% % \begin{lstlisting}[language=C++,showstringspaces=false]
% % // Extracted from tomcat-e14afee
% % public void list(HttpServletRequest request,
% %                 HttpServletResponse response,
% %                 String message) throws IOException {
% %     ...               
% %     // context.getManager() may return null.
% %     args[11] = new Integer(context.getManager().getMaxInactiveInterval()/60);
% %     ...
% % }
% % \end{lstlisting}
% % \vspace*{-4pt}
% % \end{mdframed}
% % \caption{\label{fig:npe1} NPE caused by missing check. }
% % \end{subfigure}


% % \begin{subfigure}[b]{1\textwidth}
% % \begin{mdframed}[roundcorner=5pt]
% % \scriptsize
% % \begin{lstlisting}[language=C++,showstringspaces=false]
% % // Extracted from bugs-dot-jar_FLINK-1167
% % public void setNextPartialSolution(OptimizerNode nextPartialSolution,
% %                                 OptimizerNodeterminationCriterion) {
% %     ...
% %     if (nextWorkset == worksetNode) {
% %         PactConnection noOpConn = new PactConnection(nextWorkset, noop);
% %         ...
% %     }
% %     ...
% % }
% % \end{lstlisting}
% % \vspace*{-4pt}
% % \end{mdframed}
% % \caption{\label{fig:npe2} NPE caused by comparing two $\mathit{NULL}$s.}
% % \end{subfigure}


% % \begin{subfigure}[b]{1\textwidth}
% % \begin{mdframed}[roundcorner=5pt]
% % \scriptsize
% % \begin{lstlisting}[language=C++,showstringspaces=false]
% % // Extracted from bugs-dot-jar_FLINK-1922
% % public InputSplit getNextInputSplit() {
% %     ...
% %     byte[] serializedData = nextInputSplit.splitData();
% %     deserializeObject(serializedData);
% %     ...
% % }
% % \end{lstlisting}
% % \vspace*{-4pt}
% % \end{mdframed}
% % \caption{\label{fig:npe3} NPE caused by splitting empty data of Byte class. }
% % \end{subfigure}




% % \begin{subfigure}[b]{1\textwidth}
% % \begin{mdframed}[roundcorner=5pt]
% % \scriptsize
% % \begin{lstlisting}[language=C++,showstringspaces=false]
% % // Extracted from tomcat-eb9f94e
% % protected void sendPing() {
% %     ...
% %     // Variable failureDetector itself can be null. 
% %     if (failureDetector.get() != null) {
% %         ...
% %     }
% %     ...
% % }
% % \end{lstlisting}
% % \vspace*{-4pt}
% % \end{mdframed}
% % \caption{\label{fig:npe4} NPE caused by insufficient check that misses the object. }
% % \end{subfigure}


% % \begin{subfigure}[b]{1\textwidth}
% % \begin{mdframed}[roundcorner=5pt]
% % \scriptsize
% % \begin{lstlisting}[language=C++,showstringspaces=false]
% % // Extracted from eclipse.platform.ui-6102a2f
% % private boolean isStatusLine(Control ctrl) {
% %     ...
% %     // element.getElementId() can also return null.
% %     if (element != null
% %         && element.getElementId().equals("org.eclipse.ui.StatusLine"))
% %         return true;
% %     return false;
% % }
% % \end{lstlisting}
% % \vspace*{-4pt}
% % \end{mdframed}
% % \caption{\label{fig:npe5} NPE caused by insufficient check that misses the return value of a method. }
% % \end{subfigure}

% % \caption{Illustrative examples of a variety of the NPE bugs.}
% % \label{fig:NPEs}
% % \end{figure*}



% \subsection{Dataset Selection}
% We pick datasets that are widely studied in the literature~\cite{just2014defects4j,saha2018bugs,ye2014learning}. Given their generality and representativeness, we believe \tool's performance is likely to transfer to many other projects. 
% % \ignore{The examined projects in this work have a large variance
% % in average buggy rates. We have tried our best to make our dataset general and representative. However, it is still possible that these projects are not generalizable enough to represent all software projects. Given projects that are not included in the 18 projects, our proposed approach might generate better or worse results. \tool is only evaluated on open source Java projects. Its performance on closed source software and projects written in other languages is unknown.}

% \subsection{Bug Selection}
% %The examined bugs in this work are highly depend on the number of bug reports in the dataset.
% We have analyzed all kinds of Java runtime exceptions in our dataset, and show their distributions in Figure~\ref{fig:numOfBugs}. We chose null pointer dereference, array index out of bound and class casting bugs to create neural bug detectors because they are among the highest occurrence of bugs in the codebases. We did not use illegal argument exceptions despite having enough data. The reason is vast majority of the bugs can be caught by a simple type checker on the argument of the caller and the parameter of the callee. Other bugs like out of assertion error are short of data for building bug detectors despite their important roles in ensuring software quality. 

% % \ignore{even though it is important to detect whether an assertion can be violated or not.
% % There are many bugs that are also as important as NPE bugs, but the number of bugs are only tens, such as stack overflow bugs.}

% \begin{figure}
% \centering
%   \includegraphics[width=\linewidth]{Figures/numOfBugs.pdf}
%   \caption{Bug distributions of our dataset.}
%   \label{fig:numOfBugs}
% \end{figure}

% \subsection{Generalizing to Other Programming Languages}
% \tool is a general framework across different programming languages. In particular, generalizing to another language only requires a new extractor that constructs the graph representation for programs in the new language, the rest of the workflow is language-agnostic.
% % \subsection{Limitation}
% % We pick datasets that are widely studied in the literature~\cite{just2014defects4j,saha2018bugs,ye2014learning}. Given their generality and representativeness, we believe \tool's performance is likely to transfer to many other projects. 

==> Sections/Implementation.tex <==
% !TeX root = ../ggnn.tex

\section{Implementation}\label{sec:impl}
%Using GGNNs for sets of large, diverse graphs requires some engineering effort, as efficient batching is hard in the presence of diverse shapes.  An important observation is that large graphs are normally very sparse, and thus a representation of edges as an adjacency list would usually be advantageous to reduce memory consumption. In our case, this can be easily implemented using a sparse tensor representation, allowing large batch sizes that exploit the parallelism of modern GPUs efficiently. 
%A second key insight is to represent a batch of graphs as one large graph with many disconnected components. This just requires appropriate pre-processing to make node identities unique. As this makes batch construction somewhat CPU-intensive, we found it useful to prepare minibatches on a separate thread. Our TensorFlow (Abadi et al., 2016) implementation scales to 55 graphs per second during training and 219 graphs per second during test-time using a single NVidia GeForce GTX Titan X with graphs having on average 2,228 (median 936) nodes and 8,350 (median 3,274) edges and 8 GGNN unrolling iterations, all 20 edge types (forward and backward edges for 10 original edge types) and the size of the hidden layer set to 64. The number of types of edges in the GGNN contributes proportionally to the running time. For example, a GGNN run for our ablation study using only the two most common edge types (NextToken, Child) achieves 105 graphs/second during training and 419 graphs/second at test time with the same hyperparameters. Our (generic) implementation of GGNNs is available at https://github.com/Microsoft/ gated-graph-neural-network-samples, using a simpler demonstration task.

 we run the state-of-the-art clone detector, DECKARD \cite{4222572}, to pick a non-buggy method that is syntactically closest to each buggy method we collect.
 
 
The code extraction, construction of control flow graph and intervals are implemented based on Spoon~\cite{pawlak:hal-01169705}, which is an open-source library for Java source code transformation and analysis.

All neural bug detectors are implemented in Tensorflow. All RNNs built in the model have 1 recurrent layer with 100 hidden units. We adopt random initialization for weight initialization. Each token in the vocabulary is embedded into a 100-dimensional vector. We train the neural bug detectors using the Adam optimizer~\cite{kingma2014adam}. All experiments are performed on a 3.7GHz i7-8700K machine with 32GB RAM and NVIDIA GTX 1080 GPU.


==> Sections/Methodology.tex <==
% !TeX root = ../NeurSA.tex

\section{Methodology}\label{sec:Meth}

This section presents three neural bug detectors we created based on \tool framework. The bug detectors address a diverse set of programming mistakes: null pointer dereference bugs, array index out of bound bugs, and class casting bugs. 

\subsection{Null Pointer Exception}

The first neural bug detector addresses null pointer exception (NPE for short), which is caused by dereferencing null pointer. The main challenge for static analyzers to catch them is to precisely analyze the points-to relations, which also can scale to large programs~\cite{shi2018pinpoint}. We made the following adjustments to our graph encoding to deal with the null pointer dereference bugs. 

First, given a method call, we explicitly inject its return type and the types of its arguments. Second, We add an entry of $\mathit{NULL}$ to the vocabulary. Finally, we perform value flow analysis~\cite{shi2018pinpoint, sui2012static} to extract the data dependency among variables, in particular, we introduce a unique type of edge, which describes the value flow for pointers exclusively. Since the backbone of our graph is a variant of control flow graph, all the dependency edges are added between statement nodes (containing the dependent variables) rather than the variable itself.  

\ignore{
To this end, we devise a novel representation of $\textit{NULL}$ and pointers. Our statement representation has incorporated with the type information.
However, it misses $\textit{NULL}$ information and the propagation along control flow graph.
To address null pointer exception, we design an approach extracts the following information:

\begin{itemize}
    \item The type information of callee is placed before (or after) the callee if it is a return type(or function arguments).
    \item The explicit vocabulary of $\mathit{NULL}$. One way of avoid null pointer exception is by adding pointer checks, ensure that a pointer is not null.
    \item The data dependence of a pointer, which tracks data flow of a pointer.
\end{itemize}

The node embedding for NPE is in form of $(..., \tau_{ret}, NI_{callee}, \tau_{arg1}, \tau_{arg2},...)$ where $\tau_{ret}$ is the type information of return value, $NI_{callee}$ is the node index.
We additionally add an entry of $\mathit{NULL}$ to the vocabulary.
Then, to leverage data dependence of a pointer, we introduce value flow graph \cite{shi2018pinpoint, sui2012static}.
Value flow analysis provides data dependency information to identify identifications for null pointer dereference.
Based on value flow graph, we introduce a new kind of edge from value flow for pointers.
Specifically, for each pointer, we analyze its data dependency graph.
Then for each edge in the graph, we locate the corresponding start node $v_s$ and end node $v_d$ in the interval graph and add a new edge from $v_s$ to $v_d$.}

\subsection{Array Index Out of Bound Exception}
Array index out of bound exception (AIOE for short) occurs when the index of an array falls out of the range [0,$n$-1] ($n$ is the length of the array). The main challenge of statically analyzing this bug is to precisely determine the array bound and the index value at compile time\cite{gao2016carraybound, gao2016bovinspector}. To address this challenge, we attempted the following. 

Given an array declaration, we inject the type and the length of the array into our graph encoding. Whenever an array is accessed, we also add the type of the index variable to the mix. Finally we connect the value flow edges between statements that contain array declarations and array access operations.

\ignore{
\begin{itemize}
    \item For each array, we incorporate the array and its size. Note that we abstract variables as type information, we insert a new field at the end of the type information, indicating the length of an array.
    \item The value of an array index. When accessing an array by index, explicitly highlight the array accessing by grouping the array and the index.
    \item The data dependence of an array to tracks data flow.
\end{itemize}


The node embedding for the definition of array index out of bound is in form of $(..., \tau_{array}, \tau_{length},...)$ where $\tau_{array}$ is the type information of return value, $\tau_{length}$ is an integer or variable that indicates length of the array.
For each array access point, the encoding is in form of $(..., \tau_{array}, \tau_{length},\tau_{index},...)$ where $\tau_{index}$ is the type information of the index.
Finally, we add value flow edges from the definition of an array to the use of the array.}
  
\subsection{Class Cast Exception}
Class cast exception (CCE for short) is thrown when the object is cast to a subclass of which it is not an instance. The challenge lies in analyzing the type of a variable, determining whether there is an inherent relation between the variable that is being cast and the target type the variable is cast to. To deal with the challenge, we take the following actions.

Given a cast operation, we explicitly encode the type of the variable to be cast, providing an opportunity for GGNN to check the compatibility between its actual type and target type to be cast to. In addition, we also add the value flow edges connecting the cast operation to all statements that contain other variables the variable depends on.

\ignore{
\begin{itemize}
    \item For the target type, we also extract the type information instead of only analyzing type information of variable.
    \item The data dependence of an array to tracks data flow.
\end{itemize}

The node embedding for type cast operation is in form of $(..., \tau_{cast\_type}, \tau_{var},...)$ where $cast\_type$ is the target type of cast operation and $var$ is the variable that to be cast.
The data dependence tracks variable type by adding value flow edges.
Note that this bug highly depends on the type of a variable and thus it is important to track its type.}




==> Sections/Problem.tex <==
% !TeX root = ../ggnn.tex

\section{Software defects}\label{sec:problem}
\subsection{Null pointer exception}

\begin{figure}[t]
%\centering
\small
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
public SortedKeyValueIterator<Key,Value> deepCopy(IteratorEnvironment env) {
    ...
    // rowMatcher may be null
    result.rowMatcher = rowMatcher.pattern().matcher("");
    ...
}
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\vspace*{-5pt}
\caption{\label{NPE} NPE example (from bugs-dot-jar\_ACCUMULO-189)}
\normalsize
%\vspace*{-5ex}
\end{figure}

\subsection{Array index out-of-bound}



\subsection{Class cast exception}

\begin{figure}[t]
%\centering
\small
\begin{mdframed}[roundcorner=5pt]
\scriptsize
\begin{lstlisting}[language=C++,showstringspaces=false]
    ...
    } else if (target instanceof FilterProcessor) {
        // FilterDefinition is so precise that it results in class cast exception
        // The patch changes it to its parent class ExpressionNode.
        answer = new ManagedFilter(context, (FilterProcessor) target,
        (FilterDefinition) definition);
    ...
\end{lstlisting}
\vspace*{-4pt}
\end{mdframed}
\vspace*{-5pt}
\caption{\label{CCE} Class cast exception (from bugs-dot-jar\_CAMEL-9672)}
\normalsize
%\vspace*{-5ex}
\end{figure}




==> Sections/Tables.tex <==

\begin{table*}[!t]
\centering
\small
\caption{Performance on  alternative node representations in \tool}
\begin{tabular}{c|ccc|ccc|ccc}
\hline
\multirow{2}{*}{\tabincell{c}{Bug types}} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{Array} & \multicolumn{3}{c}{CCE}\\
\cline{2-10}
& Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall & F1 \\\hline
\tabincell{c}{Characteristic\\vectors}&  00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\\hline
\tabincell{c}{RNN-based\\encoding } & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0  \\\hline
\tabincell{c}{Transformer-based\\encoding } & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\\hline 

\end{tabular}
\label{tab:alter}
\end{table*}



\begin{table*}[!t]
\centering
\small
\caption{Performance on method-level prediction}
\begin{tabular}{c|ccc|ccc|ccc}
\hline
 \multirow{2}{*}{\tabincell{c}{Bug types}} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{Array} & \multicolumn{3}{c}{CCE} \\
\cline{2-10}
& Precision & Recall & F1 & Precision & Recall & F1  & Precision & Recall & F1  \\\hline
\tool & 65.6 & \textbf{72.1} & \textbf{68.7} &  \textbf{70.7} & 52.3 & 60.1 &70.1 &  48.6 & 57.4 \\\hline
AST & 77.4 & \textbf{85.7} & \textbf{81.4} &  \textbf{84.2} & 57.1 & 68.1 &  69.2 & 64.3 & 66.7  \\\hline
CFG & 77.3 & \textbf{81.0} & \textbf{79.1} &  78.9 & 71.4 & 75.0 &   \textbf{82.4} & 66.7 & 73.7  \\\hline

\end{tabular}
\label{tab:metRes}
\end{table*}



\begin{table*}[!t]
\centering
\small
\caption{Performance on line-level prediction}
\begin{tabular}{c|c|ccc|ccc|ccc}
\hline
 \multirow{2}{*}{\tabincell{c}{Bug types}} & \multirow{2}{*}{Top-N} & \multicolumn{3}{c|}{NPE} & \multicolumn{3}{c|}{Array} & \multicolumn{3}{c}{CCE} \\
\cline{3-11}
&  & Precision & Recall & F1 & Precision & Recall & F1  & Precision & Recall & F1  \\\hline
\multirow{5}{*}{\tool} & Top-1 & 44.1 & 44.1 & 44.1 & 37.8 & 37.8 & 37.8 & \textbf{47.7} & \textbf{47.7} & \textbf{47.7} \\\cline{2-11}
& Top-3 & 19.2 & \textbf{57.7} & 28.8 & \textbf{22.3} & 55.0 & \textbf{31.7} & 18.6 & 55.9 & 27.9 \\\cline{2-11}
& Top-5 & 15.1 & \textbf{67.6} & 24.7 & \textbf{16.9} & 64.0 & \textbf{26.8} & 13.7 & 61.3 & 22.4 \\\cline{2-11}
& Top-7 & 12.6 & \textbf{73.0} & 21.5 & \textbf{14.7} & 72.1 & \textbf{24.4} & 11.7 & 67.6 & 19.9 \\\cline{2-11}
& Top-10 & 11.0 & \textbf{82.0} & 19.5 & \textbf{13.0} & 80.2 & \textbf{22.3} & 10.7 & 79.3 & 18.8  \\\hline
\multirow{5}{*}{AST} & Top-1 & \textbf{35.7} & \textbf{35.7} & \textbf{35.7} & 28.6 & 28.6 & 28.6 & 32.1 & 32.1 & 32.1 \\\cline{2-11}
& Top-3 & \textbf{16.7} & \textbf{50.0} & \textbf{25.0} & 12.7 & 35.7 & 18.7 & 15.5 & 46.4 & 23.2 \\\cline{2-11}
& Top-5 & \textbf{14.8} & \textbf{71.4} & \textbf{24.5} & 8.7 & 39.3 & 14.2 & 9.6 & 46.4 & 16.0 \\\cline{2-11}
& Top-7 & \textbf{11.5} & \textbf{75.0} & \textbf{19.9} & 6.9 & 42.9 & 11.9 & 8.7 & 57.1 & 15.2 \\\cline{2-11}
& Top-10 & \textbf{8.4} & \textbf{75.0} & \textbf{15.1} & 7.7 & 64.3 & 13.7 & 7.2 & 64.3 & 12.9  \\\hline
\multirow{5}{*}{CFG} & Top-1 & 47.6 & 47.6 & 47.6 & \textbf{66.7} & \textbf{66.7} & \textbf{66.7} & 52.4 & 52.4 & 52.4 \\\cline{2-11}
& Top-3 & 23.8 & \textbf{71.4} & 35.7 & \textbf{26.4} & 66.7 & \textbf{37.8} & 22.2 & 66.7 & 33.3 \\\cline{2-11}
& Top-5 & 17.9 & \textbf{81.0} & 29.3 & \textbf{22.4} & \textbf{81.0} & \textbf{35.1} & 16.8 & 76.2 & 27.6 \\\cline{2-11}
& Top-7 & 14.4 & 81.0 & 24.5 & \textbf{19.4} & \textbf{85.7} & \textbf{31.6} & 13.6 & 76.2 & 23.0 \\\cline{2-11}
& Top-10 & 14.1 & \textbf{95.2} & 24.5 & \textbf{18.5} & \textbf{95.2} & \textbf{31.0} & 14.1 & \textbf{95.2} & 24.5  \\\hline

\end{tabular}
\label{tab:lineres}
\end{table*}

